A Spectral Analysis of Dot-product Kernels

We present eigenvalue decay estimates of integral operators associated with compositional dot-product kernels. The estimates improve on previous ones established for power series kernels on spheres. This allows us to obtain the volumes of balls in the corresponding reproducing kernel Hilbert spaces. We discuss the consequences on statistical estimation with compositional dot product kernels and highlight interesting trade-offs between the approximation error and the statistical error depending on the number of compositions and the smoothness of the kernels.

==> sections/broader-impact.tex <==
\section*{Broader Impact}
This work does not present any foreseeable societal consequence.

==> sections/section1-neurips.tex <==
\section{Introduction}
% \todo{change Proposition ect with Prop. Sec. ect + add notations}
Dot product kernels are important tools to tackle signal or image data in machine learning, statistical estimation, and computational mathematics~\cite{steinwart2008support,MR1837879,MR2131724,zbMATH01602327}. Signal and image data is commonly normalized to lie on a sphere for signal denoising or image classification for instance~\cite{DBLP:journals/ftcgv/MairalBP14}.  The spectrum of eigenvalues of an integral operator associated with a simple dot product kernel such as the Gaussian kernel was first presented in~\cite{smola2001regularization} and explored further in a series of papers~\cite{NIPS2009_3628,zwicknagl2009power,azevedo2014sharp}. 

Recently new dot product kernels have appeared in relation to the theoretical analysis of deep networks \textit{e.g.}in~\cite{mairal2014convolutional, daniely2016toward, bach2017breaking, song2018mean}. A striking feature of recent works is the variety of applications of dot product kernels. In~\cite{mairal2014convolutional,daniely2016toward}, kernel deep networks are proposed using multi-layer kernels. In~\cite{bach2017breaking}, dot product kernels are used to analyze single hidden-layer neural networks in the realizable case. In~\cite{song2018mean}, dot product kernels arise within in an asymptotic mean-field analysis of neural networks. 

We present tight estimates of eigenvalue decay for integral operators associated with dot product kernels of the form
\begin{align}
\label{eq:kernel-gene-form}
K_{N}(x,x'):=f_N\circ...\circ f_1(\langle x,x'\rangle_{\mathbb{R}^d})
\end{align}
when the functions $(f_i)_{i=1}^N$ satisfy regularity conditions on $[-1,1]$. The eigenvalue decay estimates we obtain are of independent interest, as they generalize previous fundamental results on Mercer decompositions and eigenvalue estimates of dot product kernels~\cite{zwicknagl2009power,azevedo2014sharp}. Central to the analysis are spherical harmonics, a family of special functions arising as eigenfunctions of integral operators associated with simple dot product kernels. We also show how we can approach the statistical analysis of a multi-layer perceptron using a reproducing kernel Hilbert space associated with a dot product kernel of this form. As a result, we obtain statistical bounds for multi-layer perceptrons that encompass both the unrealizable case and the realizable case. 

The analysis also yields a characterization of the universality of dot product kernels. The universality of a kernel is a key property which guarantees Bayes-consistency~\cite{steinwart2008support}. We show that the universality can be related to regularity conditions of the functions $(f_i)_{i=1}^N$ on $[-1,1]$. The analysis suggests that, 
as the number of composition grows, the statistical rate remains basically the same, while the set of target functions that can be approximated gets larger.  We believe the results can contribute to develop a better understanding of the impact of a compositional structure on statistical performance.

\paragraph{Related work}
We give here a brief overview of related works. We point to the Supplement for more detailed discussions. 

\textit{Dot product kernels.} In the seminal paper~\cite{smola2001regularization}, initial estimates of eigenvalue decay for simple dot product kernels, corresponding to $N=1$ in our framework, have been presented. Tight estimates for power series kernels were then obtained in~\cite{zwicknagl2009power,azevedo2014sharp} in a particular regime. We extend these tight estimates to a broader range of regimes. In other words, we have obtained a complete characterization of the eigenvalue decay of power series kernels. The results we present also apply to recent kernel-based alternatives to deep networks such as~ \cite{shankar2020neural}. 

\textit{Single hidden-layer neural networks.} In~\cite{bach2017breaking}, single-hidden layer neural networks with input data normalized on the sphere are analyzed via reproducing kernel Hilbert spaces of kernels on spheres.
 %The eigenvalue decay regime of the integral operator associated with the kernel on sphere considered satisfies a polynomial eigenvalue decay regime. 
 We extend the work of~\cite{bach2017breaking} in that we analyze neural networks with more than one hidden layer in various eigenvalue decay regimes including the geometric and super-geometric ones which were not considered in~\cite{bach2017breaking}. Moreover, in contrast to~\cite{bach2017breaking} in which the learning problem is assumed to be realizable, \textit{i.e.} the target function is assumed to live in the function space, we work under less stringent source condition assumptions to derive statistical convergence rates. 

\textit{Special class of neural networks.} In~\cite{savarese:etal:2019,ongie:etal:2020}, the authors focus on the realizable case, \textit{i.e.} when the target function $f_{\rho}$ lives in the function space used to learn, and characterize the norm required to realize such functions using a network, with a single-hidden layer, with an infinite width, and a ReLU activation. Their viewpoint is diametrically opposed to ours, the proof techniques as well, since we do not assume that the target function is realizable, nor do we assume that the layers have infinite width, and consider multi-layer networks instead of a single-hidden layer ones. The two viewpoints can therefore be seen as complementary. 

\textit{Multi-layer neural networks with smooth activation functions.} In \cite{zhang2016l1}, multi-layer neural networks with smooth activation functions are analyzed via reproducing kernel Hilbert spaces. The family of kernels we consider in~Prop.~\ref{prop:RKHS-MLP} generalizes the one studied in~\cite{zhang2016l1} 
%and the RKHS norm hence the generalization bounds for the multi-layer neural network obtained in~\cite{zhang2016l1} is less tight the one we have
as our kernels are adaptive to the nonlinear functions involved in the construction of the network. In~\cite{suzuki2018fast}, excess risk bounds for multi-layer perceptrons are presented. While integral operators and eigendecay arise in the analysis, no estimate of eigendecay are obtained, whereas this is one of our main contributions in this paper. The tight estimates we obtain result in estimates of effective dimension or degrees-of-freedom of multi-layer perceptrons. 


\paragraph{Paper outline.} After introducing the framework and the notations in Sec. 2, we show in Sec. 3 that the function space associated with deep networks can be embedded into an adaptive RKHS associated to a kernel of the form~(\ref{eq:kernel-gene-form}). We exhibit a control of the eigenvalue decay associated with these compositional kernels in two regimes. In Sec. 4, we show an application of the eigenvalue decay estimates to the statistical analysis of multi-layer perceptrons. 

==> sections/section1.tex <==
\section{Introduction}
Multi-layer perceptrons have been an important family of machine learning methods, whose history alternates between periods of wide popularity and periods of fading interest \cite{rosenblatt1958perceptron, Minsky:Papert:1987, duda1973pattern}. Described in a mathematical language, a multi-layer perceptron is the iterated composition of parameterized affine maps and nonlinear maps, ultimately composed with a prediction map either for the purpose of predicting a scalar value as in curve fitting or regression, or a binary label as in supervised classification. As the number of layers or network depth grows, the parameterized map resulting from this iterated composition may change in terms of smoothness properties. 

However the impact of network depth on the regularity of the resulting deep network function is, quite surprisingly, still not fully understood, in particular for multi-layer perceptrons. Consider the setting, where the number of datapoints is finite, the number of hidden layers is finite, and the number of weights per layers is finite. We would like to understand, in the case of least-squares regression through with regularized empirical risk minimization for instance \cite{Lin_2020,marteau2019beyond,blanchard2018optimal,steinwart2008support,caponnetto2007optimal,smale2007learning}, how fast does the learned function converge to the target function as the network depth grows and the sample size grows. 

Understanding the relative scaling of the sample size and the network depth can be related to the detailed study of the spectrum of the integral operator associated with a reproducing kernel related to the network architecture. This reproducing kernel may or may not be universal, hence Bayes-consistency may or may not be satisfied. Yet, as we show in this paper, the universality and Bayes-consistency is guaranteed for wide array of situations.


The integral operator is compact, self-adjoint and admits a spectral decomposition. The rate of eigenvalue decay directly controls the convergence rate of the learned function. In this work, we obtain a tight control of the rate of eigenvalue decay for several regimes depending on the nonlinear maps involved in the construction of the network. From this control, we establish high-probability bounds on the learned function and provide guidance on the effect of the depth for such networks, depending on the sample size. Moreover the results obtained extends previous results related to the Mercer decomposition of dot product kernels on spheres \cite{azevedo2014sharp}.

Reproducing kernels are powerful tools which have been used to analyze deep networks in various ways. Recent works used reproducing kernels to build equivalent instantaneous approximations of deep networks during the training process, blending algorithmic and statistical considerations in the analysis. Although remarkable progress has been made in recent years, the understanding of training processes of deep networks is still limited. Many results are qualitative in spirit and various seemingly incompatible interpretations have been proposed and subject to discussion \cite{jacot2018neural,song2018mean,chizat2019lazy}.

We adopt here a nonparametric learning approach~\cite{gkkw:2002,steinwart2008support}, with the modest goal to uncover the interplay of regularity controlled by the network depth and the sample size, with the expectation to obtain high-probability bounds on the learned function explicitly involving the eigenvalue decay of the integral operator. We shall not assume that the target function belongs to the function spaces used for learning. We believe such results are important steps to shed light on the role of network depth on statistical performance. We present here results of this kind for multi-layer perceptrons.
\medbreak
This work makes the following contributions.
\begin{itemize}
    \item In Sections 3, we present general convergence rates for regularized least-squares regression with kernel-based methods, improving upon known convergence rates in the near geometric regime of eigenvalue decay of integral operators. 
    \item In Section 4, we consider deep networks of multi-layer perceptron type and show how to approach them through reproducing kernel Hilbert spaces and associated integral operators. We obtain tight controls of the eigenvalue decay of the integral operator in two regimes, geometric and super-geometric. 
    
    \item In section 5 we obtain the learning rates associated to multi-layer perceptrons in two regimes of eigenvalue decay of the integral operators, geometric and super-geometric, matching known minimax optimal rates in nonparametric least-squares regression. We show increasing the network depth allows to increase the target function space without sacrificing the convergence rate. 
\end{itemize}
We round off the paper with  illustrations of the relationship between the eigenvalue decay and the network depth.



==> sections/section2-neurips.tex <==
\section{Dot Product Kernels and their Spectral Decompositions}

Kernels on spheres are ubiquitous in machine learning, statistical estimation, and computational mathematics~\cite{smola2001regularization,steinwart2008support,MR1837879,MR2131724,zbMATH01602327}.
Simple kernels on spheres date back to the seminal works on reproducing kernels by Sch\"{o}nberg~\cite{MR5922}. Examples of simple kernels on spheres include homogeneous polynomial kernels, inhomogeneous polynomial kernels, and Vovk's polynomial kernels~\cite{smola2001regularization,steinwart2008support}.
%It would be nice to add here the refs for Shawe-Taylor and Cristianini book and Schoelkopf-Smola book 
The analysis of a dot product kernel on the sphere hinges upon a Taylor-like expansion which then allows one to obtain a spectral decomposition, on the one hand, and a Mercer decomposition, on the other hand. 

\paragraph{Dot product kernel on the sphere.} 
Let $d\geq 2$ and $S^{d-1}$ be the unit sphere of $\mathbb{R}^d$. A kernel of the form
\begin{align}
\label{eq:dot-product-kernel}
    K(x,y)=\sum_{m\geq 0}  b_m (\langle x,y\rangle)^{m}\text{,\quad} x,y\in S^{d-1}
\end{align}
in which $(b_m)_{m\geq 0}$ is an absolutely summable sequence of real numbers is called a \emph{dot product kernel on the sphere} $S^{d-1}$~\cite{zwicknagl2009power}. Note that the construction we describe below could be extended to dot product kernels in Hilbert spaces~\cite{MR5922}. If $b_m\geq 0$ for every $m\geq 0$, then $K$ is a \emph{continuous positive semi-definite kernel} on the sphere $S^{d-1}$~\cite{pinkus2004strictly}. 

\paragraph{Integral operator.}
Let $L_2^{d\sigma_{d-1}}(S^{d-1})$ be the space of (real) square-integrable functions on the sphere $S^{d-1}$ endowed with its induced Lebesgue measure $d\sigma_{d-1}$ and $|S^{d-1}|$ the surface area of $S^{d-1}$.
Given a positive semi-definite kernel $K$ on $S^{d-1}$, we define the integral operator on $L_2^{d\sigma_{d-1}}(S^{d-1})$ associated 
$$\begin{array}{ccccc}
T_{K} & : &  L_2^{ d\sigma_{d-1}}(S^{d-1}) & \to &  L_2^{ d\sigma_{d-1}}(S^{d-1})\\
 & & f &\to & \int_{S^{d-1}} K(x,\cdot)f(x)d\sigma_{d-1}(x)
\end{array}$$
As soon as $\int_{S^{d-1}} K(x,x)d\sigma_{d-1}(x)$ is finite, $T_K$ is well defined, self-adjoint, positive semi-definite and trace-class~\cite{smale2007learning,steinwart2008support}. 

Denote $H$ the Reproducing Kernel Hilbert Space (RKHS) associated to $K$. The spectral theorem for compact operators~\cite{MR1335452} tells us for an at most countable index set $I$, we have a positive, decreasing sequence $(\lambda_i)_{i\in I} \in \ell_1(I)$ and a family $(e_i)_{i\in I} \subset H$, such that $(\lambda_i^{1/2} e_i)_{i\in I}$ is an orthonormal system in $H$ while $(e_i)_{i\in I}$ is an orthonormal system in $L_2^{d\sigma_{d-1}}(S^{d-1})$ with
\begin{align*}
T_{K} &=\sum_{i\in I}\lambda_i\langle ., e_i\rangle_{L_2^{d\sigma_{d-1}}(S^{d-1})} e_i
\end{align*}
The system of eigenfunctions of $T_{K}$ is particularly interesting, yet often unknown analytically, except for special classes of kernels. Our class of kernels is one of them. 
\medbreak


\paragraph{Spherical harmonics.}
Let $P_{m}(d)$ be the space of homogeneous polynomials of degree $m$ in $d$ variables with real coefficients and $\mathcal{H}_{m}(d)$ be the space of harmonics polynomials defined by 
 \begin{align*}\mathcal{H}_m(d):=\{P\in P_{m}(d)| \Delta P=0\}
  \end{align*}
   where $\Delta \cdot = \sum\limits_{i=1}^d\frac{\partial^2\cdot}{\partial x_i^2} $ is the Laplace operator on $\mathbb{R}^d$~\cite{MR2131724}.  Moreover define
 $H_{m}(S^{d-1})$ the space of real spherical harmonics of degree $m$ defined as the set of restrictions of harmonic polynomials in $\mathcal{H}_{m}(d)$ to $S^{d-1}$. Let also $L_2^{d\sigma_{d-1}}(S^{d-1})$ be the space of (real) square-integrable functions on the sphere $S^{d-1}$ endowed with its induced Lebesgue measure $d\sigma_{d-1}$ and $|S^{d-1}|$ the surface area of $S^{d-1}$. $L_2^{d\sigma_{d-1}}(S^{d-1})$ endowed with its natural inner product is a separable Hilbert space and the family of spaces $(H_m(S^{d-1}))_{m\geq 0}$, yields a direct sum decomposition~\cite{frye2012spherical} that reads as
 \begin{align}
 L_2^{d\sigma_{d-1}}(S^{d-1})=\bigoplus_{m\geq 0}H_m(S^{d-1})
 \end{align}
 which means that the summands are closed and pairwise orthogonal.
 Moreover, each $H_m(S^{d-1})$ has a finite dimension $\alpha_{m,d}$ with $\alpha_{0,d}=1$, $\alpha_{1,d}=d$ and for $m\geq 2$
 \begin{align*}
 \alpha_{m,d}=\dbinom{d-1+m}{m}-\dbinom{d-1+m-2}{m-2}
 \end{align*}
 Therefore for all $m\geq 0$, given any orthonormal basis of $H_m(S^{d-1})$, $(Y_{m}^1,...,Y_{m}^{\alpha_{m,d}})$, we can build an Hilbertian basis of $L_2^{d\sigma_{d-1}}(S^{d-1})$ by concatenating these orthonormal bases. Let us denote in the following $(Y_{m}^{l_m})_{m,l_m}$ such an Hilbertian basis of $L_2^{d\sigma_{d-1}}(S^{d-1})$.
 

\paragraph{Mercer decomposition.}
In~\cite{azevedo2014sharp}, a Mercer decomposition is given for a dot product kernel on the sphere of the form~(\ref{eq:dot-product-kernel}). Indeed each spherical harmonics of degree $m$, $Y_{m}\in H_{m}(S^{d-1})$, is an eigenfunction of $T_{K}$ with associated eigenvalue given by the formula
% The eigenvalues of $T_{K}$ are exactly the set $\{\lambda_m\text{: }m\geq 0\}$ where $\lambda_m$ is defined as
\begin{align}
\label{eq:formula_eigen-notions}
\lambda_{m}=&\frac{|S^{d-2}|\Gamma((d-1)/2)}{2^{m+1}}\\
&\sum_{s\geq 0}b_{2s+m}\frac{(2s+m)!}{(2s)!}\frac{\Gamma(s+1/2)}{\Gamma(s+m+d/2)} 
\end{align}
The decay of eigenvalues (or eigendecay) is central to the understanding of a kernel. Moreover we need to take into account the \emph{eigenvalue multiplicities} in order to control of the eigendecay. A control of eigendecay is usually out of reach except for specific kernels on specific domains; see~\cite{steinwart2008support} for a survey. Indeed upper bounding or lower bounding can quickly result in such loose bounds that they are trivial bounds. A careful control of eigenvalues and their multiplicities is essential. 


\paragraph{Eigendecay regimes.}
We distinguish three regimes of decay of eigenvalues: polynomial, geometric, and super-geometric. Polynomial decay corresponds to a rate proportional to $m^{-q}$ with $q>0$; geometric decay proportional to $\exp(-\alpha m^q)$ with $\alpha>0$ and $q>0$; super-geometric decay faster to geometric decay. We shall see that multi-layer perceptrons (\ref{eq:formula_eigen-notions}) relate to geometric and super-geometric decays. In Table \ref{table:1}, we give an overview of several kernels along with their eigendecays from the literature~\cite{bach2017breaking,bach2017equivalence,blanchard2008finite}, as well as the two type of kernels we consider in this paper.
 

  %%%
\begin{table*}[ht]
\centering
\begin{tabular}{lcc}
Kernel & Space & Rate \\ 
\hline
\vspace{0.25cm}
$K(x,x'):=\exp(-b(x-x')^2)$ & $[0,1]$  & $(b/(a+b))^{m}$,$\quad a,b>0$ \\
\vspace{0.25cm}
$K(x,x'):=\nu_0+\sum_{m>0}\nu_m \cos(2\pi m(x-x'))$ & $[0,1]$&  $m^{-2s}$,$\quad s\in\mathbb{N}^{*}$\\
\vspace{0.25cm}
$K(x,x'):=\mathbb{E}_{v\sim\sigma_{d-1}}(v^T x)^s_{+}(v^T x)^s_{+}$ &$S^{d-1}$  & $m^{-1-1/(d-1)-2s/(d-1)}$, $\quad s\in\mathbb{N}$\\
\vspace{0.25cm}
$K_1$ & $S^{d-1}$ &  $m^{- \gamma m^{1/(d-1)}}$, $\quad\gamma>0$ \\
\vspace{0.25cm}
$K_2$ & $S^{d-1}$  & $e^{-\gamma m^{\frac{1}{d-1}}}$,$\quad\gamma>0$ 
\end{tabular}
\caption{Comparison of eigendecay rates for different kernels. $K_1$ and $K_2$ are kernels associated with MLPs in super-geometric and geometric regime resp.\label{table:1}}
\end{table*}
%%%
\textbf{Embedding a Multi-layer Perceptron in an RKHS.}
The mapping defined by a multi-layer perceptron (MLP) can be embedded into an appropriate RKHS with respect to the nonlinear activations involved in the network architecture. Moreover the \emph{kernel induced by an MLP is a dot product kernel} of the form~(\ref{eq:dot-product-kernel})
% \begin{align}
% \label{eq:dot-product-kernel}
%     K(x,y)= \sum_{m\geq 0}  b_m (\langle x,y\rangle)^{m}\text{,\quad} x,y\in \mathcal{X}
% \end{align}
where $(b_m)_{m\geq 0}$ is completely determined by the non linear activation functions $(\sigma_i)_{i=1}^N$ involved in the network. When $\mathcal{X}$ happens to be the unit sphere $S^{d-1}$ of $\mathbb{R}^d$ with $d\geq 2$, we can actually describe the eigenspectrum of the associated integral operator.


We refer to here as a multi-layer perceptron a fully-connected deep neural network~\cite{shalevshwartz2014}. We give below useful definitions for our construction in the next sections. 
Let $\mathcal{X}$ be a subset of $\mathbb{R}^d$, $N$ be the number of hidden layers, $\sigma_1,...,\sigma_N$ real-valued functions defined on $\mathbb{R}$ be the activation functions at each layer and $m_1,...,m_N$ be the width of each layer. Set $m_0:=d$ and $m_{N+1}:=1$. Then, any function defined by a multi-layer perceptron (MLP) is parameterized by weight matrices $(W^k)_{k=1}^{N+1}$ where each $W^k\in\mathbb{R}^{m_{k-1}m_{k}}$ and can be recovered as follows. Let $x\in\mathcal{X}$, define $\mathcal{N}^0(x):=x$ and for $k\in\{1,\dots,N\}$,  denote
$W^k:=(w_1^k,...,w_{m_{k}}^k)$ where for all  $j\in[|1,m_k|]$ $w_j^k\in\mathbb{R}^{m_{k-1}}$. Then, for all $k\in\{1,...,N\}$, define the $k^{\text{th}}$ layer as
$$\mathcal{N}^{k}(x):=(\sigma_k(\langle \mathcal{N}^{k-1}(x),w_1^k \rangle), ...,\sigma_k(\langle \mathcal{N}^{k-1}(x),w_{m_k}^k \rangle))$$

We obtain $\mathcal{N}(x)=\langle \mathcal{N}^N(x),W^{N+1}\rangle_{\mathbb{R}^{m_N}}$.
We shall denote $\mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N,(m_i)_{i=1}^N}$ the function space defined by all functions $\mathcal{N}$ defined as above on $\mathcal{X}$ for any choice of $(W^k)_{k=1}^{N+1}$. We shall also consider the union space
$$\mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N}:=\bigcup_{(m_1,...,m_N)\in\mathbb{N_{*}}^N} \mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N,(m_i)_{i=1}^N} .$$



==> sections/section2.tex <==
\section{Basic Notions and Notations}

\textbf{Multi-layer Perceptrons.} Let us first introduce the network of interest. Here we consider a fully-connected deep neural network. We shall refer to it as a multi-layer perceptron (MLP).
Let $\mathcal{X}$ be a subset of ${R}^d$, $N$ be the number of hidden layers, $\sigma_1,...,\sigma_N$ real-valued functions defined on $\mathbb{R}$ be the activation functions at each layer and $m_1,...,m_N$ be the width of each layer. Set $m_0:=d$ and $m_{N+1}:=1$. Then, any function defined by an MLP is parameterized by weight matrices $(W^k)_{k=1}^{N+1}$ where each $W^k\in\mathbb{R}^{m_{k-1}m_{k}}$ and can be recovered as follows. Let $x\in\mathcal{X}$, define $\mathcal{N}^0(x):=x$ and for $k\in\{1,\dots,N\}$,  denote
$W^k:=(w_1^k,...,w_{m_{k}}^k)$ where for all  $j\in[|1,m_k|]$ $w_j^k\in\mathbb{R}^{m_{k-1}}$. Then, for all $k\in\{1,...,N\}$, define the $k^{\text{th}}$ layer as
$$\mathcal{N}^{k}(x):=(\sigma_k(\langle \mathcal{N}^{k-1}(x),w_1^k \rangle), ...,\sigma_k(\langle \mathcal{N}^{k-1}(x),w_{m_k}^k \rangle))$$
We obtain $\mathcal{N}(x)=\langle \mathcal{N}^N(x),W^{N+1}\rangle_{\mathbb{R}^{m_N}}$.
We shall denote $\mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N,(m_i)_{i=1}^N}$ the function space defined by all functions $\mathcal{N}$ defined as above on $\mathcal{X}$ for any choice of $(W^k)_{k=1}^{N+1}$. We shall also consider the union space
$$\mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N}:=\bigcup_{(m_1,...,m_N)\in\mathbb{N_{*}}^N} \mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N,(m_i)_{i=1}^N}$$


\textbf{From MLPs to RKHSs.}\todo{Ce n est pas une notion basique mais un resultat de ce papier...} In the following we show that functions generated by a multi-layer perceptron can be embed into an adaptative RKHS with respect to the nonlinear activations involved in the construction of the network. Moreover we show that kernels induced by MLPs are dot product kernels of the form
\begin{align}
\label{eq:dot-product-kernel}
    K(x,y)= \sum_{m\geq 0}  b_m (\langle x,y\rangle)^{m}\text{,\quad} x,y\in \mathcal{X}
\end{align}
where $(b_m)_{m\geq 0}$ is completely determined by the non linear activation functions $(\sigma_i)_{i=1}^N$ involved in the network. When $\mathcal{X}$ happens to be the unit sphere $S^{d-1}$ of $\mathbb{R}^d$ with $d\geq 2$, we even have access to the eigenspectrum of the integral operator associated.

% \textbf{Spherical Harmonics.} Let $P_{m}(d)$ be the space of homogeneous polynomials of degree $m$ in $d$ variables with real coefficients and $\mathcal{H}_{m}(d)$ be the space of harmonics polynomials defined by
% \begin{align}
% \mathcal{H}_m(d):=\{P\in P_{m}(d)| \Delta P=0\}
% \end{align}
% where $\Delta \cdot = \sum\limits_{i=1}^d\frac{\partial^2\cdot}{\partial x_i^2} $ is the Laplace operator on $\mathbb{R}^d$. Moreover let us define
% $H_{m}(S^{d-1})$ the space of real spherical harmonics of degree $m$ defined as the set of restrictions of harmonic polynomials in $\mathcal{H}_{m}(d)$ to $S^{d-1}$. Let also $L_2^{d\sigma_{d-1}}(S^{d-1})$ be the space of (real) square-integrable functions on the sphere $S^{d-1}$ endowed with its induced Lebesgue measure $d\sigma_{d-1}$ and $|S^{d-1}|$ the surface area of $S^{d-1}$. $L_2^{d\sigma_{d-1}}(S^{d-1})$  endowed with its natural inner product is a separable Hilbert space and the family of spaces $(H_m(S^{d-1}))_{m\geq 0}$, yields a direct sum decomposition \cite{frye2012spherical}
% \begin{align}
% L_2^{d\sigma_{d-1}}(S^{d-1})=\bigoplus_{m\geq 0}H_m(S^{d-1})
% \end{align}
% which means that the summands are closed and pairwise orthogonal.
% Moreover, each $H_m(S^{d-1})$ has a finite dimension $\alpha_{m,d}$ with $\alpha_{0,d}=1$, $\alpha_{1,d}=d$ and for $m\geq 2$
% \begin{align*}
% \alpha_{m,d}=\dbinom{d-1+m}{m}-\dbinom{d-1+m-2}{m-2}
% \end{align*}
% Therefore for all $m\geq 0$, given any orthonormal basis of $H_m(S^{d-1})$, $(Y_{m}^1,...,Y_{m}^{\alpha_{m,d}})$, we can build an Hilbertian basis of $L_2^{d\sigma_{d-1}}(S^{d-1})$ by concatenating these orthonormal basis. Let us denote in the following $(Y_{m}^{l_m})_{m,l_m}$ such an Hilbertian basis of $L_2^{d\sigma_{d-1}}(S^{d-1})$.
\medbreak
\textbf{Integral Operator.} Let $d\geq 2$ and $S^{d-1}$ be the unit sphere of $\mathbb{R}^d$. Let also $L_2^{d\sigma_{d-1}}(S^{d-1})$ be the space of (real) square-integrable functions on the sphere $S^{d-1}$ endowed with its induced Lebesgue measure $d\sigma_{d-1}$ and $|S^{d-1}|$ the surface area of $S^{d-1}$.
Given a positive semi-definite kernel $K$ on $S^{d-1}$, we define the integral operator on $L_2^{d\sigma_{d-1}}(S^{d-1})$ associated 
$$\begin{array}{ccccc}
T_{K} & : &  L_2^{ d\sigma_{d-1}}(S^{d-1}) & \to &  L_2^{ d\sigma_{d-1}}(S^{d-1})\\
 & & f &\to & \int_{S^{d-1}} K(x,\cdot)f(x)d\sigma_{d-1}(x).
\end{array}$$
As soon as $\int_{S^{d-1}} K(x,x)d\sigma_{d-1}(x)$ is finite, $T_K$ is well defined, self-adjoint, positive semi-definite and trace-class \cite{smale2007learning}. Denote $H$ the Reproducing Kernel Hilbert Space (RKHS) associated to $K$. The spectral theorem for compact operators tells us for an for at most countable index set $I$, we have a positive, decreasing sequence $(\lambda_i)_{i\in I} \in \ell_1(I)$ and a family $(e_i)_{i\in I} \subset H$, such that $(\lambda_i^{1/2} e_i)_{i\in I}$ is an orthonormal system in $H$ while $(e_i)_{i\in I}$ is an orthonormal system in $L_2^{d\sigma_{d-1}}(S^{d-1})$ with
\begin{align*}
T_{K} &=\sum_{i\in I}\lambda_i\langle ., e_i\rangle_{L_2^{d\sigma_{d-1}}(S^{d-1})} e_i
\end{align*}
In fact for some kernels, one may have access to an explicit formulation of the eigensystem of $T_{K}$.
\medbreak
\textbf{Kernels on Sphere.} Kernels of the form 
\begin{align*}
    K(x,y)=\sum_{m\geq 0}  b_m (\langle x,y\rangle)^{m}\text{,\quad} x,y\in S^{d-1}
\end{align*}
in which $(b_m)_{m\geq 0}$ is an absolutely summable sequence of real numbers are called dot product kernels on $S^{d-1}$ \cite{zwicknagl2009power}. Moreover, If $b_m\geq 0$ for every $m\geq 0$ then $K$ is a continuous positive semi-definite kernel on $S^{d-1}$ \cite{pinkus2004strictly}. In fact for those specific kernels, \cite{azevedo2014sharp} obtain an explicit Mercer decomposition.  More precisely, the eigenvalues of $T_{K}$ are exactly the set $\{\lambda_m\text{: }m\geq 0\}$ where $\lambda_m$ is defined as
\begin{align}
\label{eq:formula_eigen-notions}
&\lambda_{m}=\frac{|S^{d-2}|\Gamma((d-1)/2)}{2^{m+1}}\sum_{s\geq 0}b_{2s+m}\frac{(2s+m)!}{(2s)!}\frac{\Gamma(s+1/2)}{\Gamma(s+m+d/2)}.
\end{align}
The main challenge here is to control the eigenvalues decay with their multiplicities of the kernels related to MLPs from the expression given in Eq. (\ref{eq:formula_eigen-notions}). Such controls are obtained only for very specific kernels defined on very specific domains. In Table \ref{table:1} we introduce the control obtained for kernels related to MLPs in this paper and give some examples of such controls for other kernels available in the literature \citep{bach2017breaking,bach2017equivalence,blanchard2008finite}.  
\begin{table}[h!]
\centering
\begin{tabular}{lcc}
Kernel & Space & Rate \\ 
\hline
\vspace{0.25cm}
$K(x,x'):=\exp(-b(x-x')^2)$ & $[0,1]$  & $(b/(a+b))^{m}$,$\quad a,b>0$ \\
\vspace{0.25cm}
$K(x,x'):=\nu_0+\sum_{m>0}\nu_m \cos(2\pi m(x-x'))$ & $[0,1]$&  $m^{-2s}$,$\quad s\in\mathbb{N}^{*}$\\
\vspace{0.25cm}
$K(x,x'):=\mathbb{E}_{v\sim\sigma_{d-1}}(v^T x)^s_{+}(v^T x)^s_{+}$ &$S^{d-1}$  & $m^{-1-1/(d-1)-2s/(d-1)}$, $\quad s\in\mathbb{N}$\\
\vspace{0.25cm}
$K_1$ & $S^{d-1}$ &  $m^{- \gamma m^{1/(d-1)}}$, $\quad\gamma>0$ \\
\vspace{0.25cm}
$K_2$ & $S^{d-1}$  & $e^{-\gamma m^{\frac{1}{d-1}}}$,$\quad\gamma>0$ 
\end{tabular}
\caption{Comparison of eigenvalue decay rates for different kernels. $K_1$ and $K_2$ are the kernels associated respectively to MLPs in the super-geometric and geomtric regime.\label{table:1}}
\end{table}



==> sections/section3-neurips.tex <==
\textbf{Embedding a Multi-layer Perceptron in an RKHS.}
The mapping defined by a multi-layer perceptron (MLP) can be embedded into an appropriate RKHS with respect to the nonlinear activations involved in the network architecture. Moreover the \emph{kernel induced by an MLP is a dot product kernel} of the form~(\ref{eq:dot-product-kernel})
% \begin{align}
% \label{eq:dot-product-kernel}
%     K(x,y)= \sum_{m\geq 0}  b_m (\langle x,y\rangle)^{m}\text{,\quad} x,y\in \mathcal{X}
% \end{align}
where $(b_m)_{m\geq 0}$ is completely determined by the non linear activation functions $(\sigma_i)_{i=1}^N$ involved in the network. When $\mathcal{X}$ happens to be the unit sphere $S^{d-1}$ of $\mathbb{R}^d$ with $d\geq 2$, we can actually describe the eigenspectrum of the associated integral operator.


We refer to here as a multi-layer perceptron a fully-connected deep neural network~\cite{shalevshwartz2014}. We give below useful definitions for our construction in the next sections. 
Let $\mathcal{X}$ be a subset of $\mathbb{R}^d$, $N$ be the number of hidden layers, $\sigma_1,...,\sigma_N$ real-valued functions defined on $\mathbb{R}$ be the activation functions at each layer and $m_1,...,m_N$ be the width of each layer. Set $m_0:=d$ and $m_{N+1}:=1$. Then, any function defined by a multi-layer perceptron (MLP) is parameterized by weight matrices $(W^k)_{k=1}^{N+1}$ where each $W^k\in\mathbb{R}^{m_{k-1}m_{k}}$ and can be recovered as follows. Let $x\in\mathcal{X}$, define $\mathcal{N}^0(x):=x$ and for $k\in\{1,\dots,N\}$,  denote
$W^k:=(w_1^k,...,w_{m_{k}}^k)$ where for all  $j\in[|1,m_k|]$ $w_j^k\in\mathbb{R}^{m_{k-1}}$. Then, for all $k\in\{1,...,N\}$, define the $k^{\text{th}}$ layer as
$$\mathcal{N}^{k}(x):=(\sigma_k(\langle \mathcal{N}^{k-1}(x),w_1^k \rangle), ...,\sigma_k(\langle \mathcal{N}^{k-1}(x),w_{m_k}^k \rangle))$$

We obtain $\mathcal{N}(x)=\langle \mathcal{N}^N(x),W^{N+1}\rangle_{\mathbb{R}^{m_N}}$.
We shall denote $\mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N,(m_i)_{i=1}^N}$ the function space defined by all functions $\mathcal{N}$ defined as above on $\mathcal{X}$ for any choice of $(W^k)_{k=1}^{N+1}$. We shall also consider the union space
$$\mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N}:=\bigcup_{(m_1,...,m_N)\in\mathbb{N_{*}}^N} \mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N,(m_i)_{i=1}^N} .$$


\section{Multi-layer Perceptrons through Dot Product Kernels}
\label{sec:MLP-paper}

We show that there exists an RKHS containing the function space $\mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N}$ for any activation functions, $(\sigma_i)_{i=1}^N$, admitting a Taylor decomposition on $\mathbb{R}$. Moreover, for well chosen activation maps, the kernel is a $cc$-universal kernel on $\mathcal{X}$ in~\cite{sriperumbudur2011universality} sense. Recall that a continuous positive semi-definite  kernel $k$ on a Hausdorff space $\mathcal{X}$ is said to be $cc$-universal if the RKHS, $H$ induced by $k$ is dense in $\mathcal{C}(\mathcal{X})$ endowed with the topology of compact convergence. Proofs are provided in Appendix~\ref{proof:lem-rkhs}. 

\begin{prop}
\label{prop:RKHS-MLP}
Let $\mathcal{X}$ be any subspace of $\mathbb{R}^d$, $N\geq 1$, $(\sigma_i)_{i=1}^N$ functions which admits a Taylor decomposition on $\mathbb{R}$. Moreover let $(f_i)_{i=1}^N$ be the sequence of functions such that for every $i\in\{1,...,N\}$:
\begin{align}
\label{eq:diff-sig-f}
f_i(x)=\sum_{n\geq 0}\frac{|\sigma_i^{(n)}(0)|}{n!}x^n
\end{align}
Then the RKHS $H_N$ of the kernel, $K_{N}$ defined on $\mathcal{X}\times\mathcal{X}$ by
\begin{align}
\label{eq:kernel-MLP}
K_{N}(x,x'):=f_N\circ...\circ f_1(\langle x,x'\rangle_{\mathbb{R}^d})
\end{align}
contains the function space $\mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N}$. 
If we assume in addition that for every $i\in\{1,...,N\}$ and $n\in\mathbb{N}$, $\sigma_i^{(n)}(0)\neq 0$, then the kernel $K_N$ is $cc$-universal.
%\label{def:cc-universal}
\end{prop}

We can think of the function space RKHS $H_N$ as a kind of \emph{Hilbertian envelope} of the function space $\mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N}$. Note that
the RKHS we define above does \emph{not} require that networks are infinitely wide \textit{i.e.} that all layers of the network are infinitely large, as is assumed for instance in~\cite{daniely2016toward,DBLP:conf/icml/BiettiMCM19} or~\cite{DBLP:journals/corr/abs-1712-00779}. Indeed, for any number of weights $(m_i)_{i=1}^N$, the function space $\mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N,(m_i)_{i=1}^N}$ lies inside the RKHS we have just defined. There are several consequences to the Prop. above. 

\paragraph{Consequences of universality.} A first simple fact is that 
\begin{equation*}
    \inf_{f\in H_N} \mathbb{E}[(f(X)-Y)^2] 
    \leq 
    \inf_{f\in F} \mathbb{E}[(f(X)-Y)^2]
\end{equation*}
where $F :=\mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N}$.
In other words the minimum expected risk in $H_N$ is a lower bound on the minimum expected risk in $F$. Since a major concern of recent years has been the spectacular performance of deep networks \textit{i.e.} how small they can drive the risk, analyzing them via this Hilbertian envelope can shed more light on the relation 
between their multi-layer structure and their statistical performance.

% Thanks to Prop.~\ref{prop:RKHS-MLP}, we can have a direct control on the RKHS norm of the network through the spectral norm of its weights.
% \begin{coro}
% \label{coro:norm-mlp}
% For $(W^k)_{k=1}^{N+1}$ a sequence such that for all $k\in [|1,N+1|]$, $W^k\in\mathbb{R}^{m_{k-1}m_{k}}$ and $\mathcal{N}$ the function in $\mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N}$ associated, we have
% \begin{align*}
% \Vert \mathcal{N} \Vert_{H_N}^2 \leq \Vert W^{N+1} \Vert^2 f_N(\Vert W^{N} \Vert^{2} f_{N-1} (...f_1(\Vert W^1\Vert^2)...))
% \end{align*}
% where $\Vert.\Vert$ is the spectral norm.
% \end{coro}
% We can then obtain statistical bounds for deep networks such as as the ones in~\cite{zhang2016l1,zhang2017convexified,
% bartlett2017spectrally,bietti2017group}. Indeed the RKHS norm of the network allows one to get for instance generalization bounds involving Rademacher complexities as in~\cite{boucheron2005theory}. To be more precise, if $\mathcal{X}$ is compact and $\mathcal{Y}\subset [-M,M]$, then for any $\delta>0$ with a probability $\rho^n$ not less than $1-\delta$
% % \begin{align*}
% % R(\mathcal{N})& \leq \frac{1}{\ell}\sum_{i=1}^{\ell} (\mathcal{N}(x_i)- y_i)^2
% %  +\frac{2 G \Vert \mathcal{N} \Vert_{H_N}}{n}\sqrt{\sum_{i=1}^n K_N(x_i,x_i)} 
% % +\frac{2M^2}{\sqrt{n}}+ 3B\sqrt{\frac{ \log(\frac{2}{\delta})}{2n}} \; ,
% % \end{align*}
% \begin{align*}
% R(\mathcal{N})& \leq \frac{1}{\ell}\sum_{i=1}^{\ell} (\mathcal{N}(x_i)- y_i)^2+\mathcal{O}\left( \frac {\Vert \mathcal{N} \Vert_{H_N}}{\sqrt{n}}+ \sqrt{\frac{ \log(\frac{2}{\delta})}{2n}}\right) \; ,
% \end{align*}
% There are two major issue with these bounds. First they do not consider the approximation bias of the class of functions considered which is the major issue in high dimension. Moreover these generalization bounds may blow up as the number of parameters increases. We will see in the following that we manage to obtain learning rates of the RLS algorithm on the specific RKHSs associated to MLPs which deal with the two above issues.
% \medbreak

A second consequence is that, actually, the kernel $K_N$ associated with $H_N$ defined above is $cc$-universal. Therefore, from Corollary 5.29~\cite{steinwart2008support}, Bayes-consistency holds for common loss functions
\begin{align*}
    \inf_{f\in H} \mathbb{E}[(f(X)-Y)^2]=\mathcal{R}^\star
\end{align*}
where $R^\star$ is the Bayes risk.
Universality hence Bayes-consistency holds for a number of situations. Consider a multi-layer network in which each layer involves an exponential nonlinear function $\sigma_{\text{exp}}(x)=\exp{x}$~\cite{mairal2014convolutional,daniely2016toward}. The corresponding RKHS is $cc$-universal, Bayes-consistency holds. There are many examples of activation functions satisfying the assumptions of the Prop. \ref{prop:RKHS-MLP}, such as the square activation $\sigma_2(x)=x^2$, the smooth ReLU activation $\sigma_{\text{sh}}$, the sigmoid-like activation $\sigma_{\text{erf}}$ based on the $\text{erf}$ function, the Swish activation function~\cite{DBLP:conf/emnlp/EgerYG18,DBLP:journals/corr/abs-1710-05941}. We would like to underscore that, contrary to popular beliefs perhaps fueled by some choices made in~\cite{DBLP:conf/nips/KrizhevskySH12}, many kinds of activations functions other than ReLU activation functions have been used with great success by practitioners; see~\cite{DBLP:conf/emnlp/EgerYG18} for a recent account. 


\paragraph{Discussion}
Note that coefficients in the Taylor series of $\sigma_{\text{erf}}$ or $\sigma_{\text{sh}}$ are not nonnegative. Indeed the functions $(f_i)_{i=1}^N$ introduced in Prop. \ref{prop:RKHS-MLP} to build the RKHS $H_N$ associated the function space $\mathcal{F}_{\mathcal{X},(\sigma_{i})_{i=1}^N}$ may differ from the activation functions $(\sigma_i)_{i=1}^N$ involved in the construction of the network. Indeed as the relation in  Eq.(\ref{eq:diff-sig-f}) indicates, the functions $(f_i)_{i=1}^N$ admit a Taylor decomposition with non negative coefficients. These coefficients are the absolute values of the coefficients in the Taylor series of $(\sigma_i)_{i=1}^N$. However Prop. \ref{prop:RKHS-MLP} does not require any assumption on the sign of the coefficients of $(\sigma_i)_{i=1}^N$.
% are allowed to have negative coefficients in their Taylor decomposition. Indeed recall that the functions $(f_i)_{i=1}^N$, used to build the RKHS may differ from the nonlinear functions $(\sigma_i)_{i=1}^N$ involved in the network as it is indicated in Eq.(\ref{eq:diff-sig-f}).
% For example the function space $\mathcal{F}_{\mathcal{X},(\sigma_{\text{erf}})_{i=1}^N}$ can still be embedded in the RKHS defined in Prop. \ref{prop:RKHS-MLP} even if $\sigma_{\text{erf}}$ has negative coefficients in its Taylor decomposition. 
In the following we focus only on the functions $(f_i)_{i=1}^N$ related to the kernel $K_N$ as we want to study the proprieties of the RKHS $H_N$ associated.


\textbf{Examples.} Consider the case where the input space $\mathcal{X}$ is the unit sphere. Therefore if we assume that for all $i\in\{1,...,N\}$, $f_i(1)=1$ then the norm is preserved across the layers as we obtain that
$K_i(x,x) = \Vert x\Vert_2^2$. In that case, we can consider a larger class of functions as we only need the $(f_i)_{i=1}^N$ to admit a Taylor expansion about 0 on $[-1,1]$. We list some classical functions which satistfy these assumptions \cite{bietti2017group}.
\begin{table}[ht]
\label{table:2}
\centering
\begin{tabular}{l|l}
polynomial & $f(t)=\frac{1}{p^p}(p-1+t)^p$\\
Inverse polynomial & $f(t)=\frac{1}{2-t}$\\
arc-cosine & $f(t)=\frac{1}{\pi}(\sin(\text{arcos}(t))
\\& +(\pi-\text{arcos}(t))\cos(\text{arcos}(t)))$ \\
Vovk's & $f(t)=\frac{1}{3}(1+t+t^2)$
\end{tabular}
\end{table}

Note that the inverse polynomial kernel was used by \cite{zhang2016l1,zhang2017convexified} to build convex models of fully connected networks and two-layer convolutional neural networks, while the arc-cosine kernel appears in early deep kernel machines \cite{NIPS2009_3628}.



In the following we assume that the input space $\mathcal{X}$ is the unit sphere $S^{d-1}$ of $\mathbb{R}^d$ where $d\geq 2$. This is a common assumption in the literature, motivated by common input pre-processing procedures in signal processing and computer vision ~\cite{DBLP:journals/ftcgv/MairalBP14,bach2017breaking,elad:2010}.

\paragraph{True Colors of Multi-Layer Perceptrons.} We show now how to control the eigenvalue decay of an integral operator associated with a kernel introduced in Prop.~\ref{prop:RKHS-MLP}. We exhibit two regimes: geometric and super-geometric. We can be in one or the other regime, depending on the activation functions involved. Let $N\geq 1$, $d\geq 2$ and $(f_i)_{i=1}^N$ be a sequence of $N$ real valued functions satisfying assumptions of Prop. \ref{prop:RKHS-MLP}. Therefore $f_N\circ...\circ f_1$ admits a Taylor decomposition on $[-1,1]$, and we denote its non negative coefficients $(b_m)_{m\geq 0}$ such that
 \begin{align*}
 f_N\circ...\circ f_1(x)=\sum_{m\geq 0} b_m x^m.
\end{align*}
Moreover we denote $K_N$ the kernel associated as defined in Prop. \ref{prop:RKHS-MLP}. Recall that for such kernels we have an explicit formulation of the eigenvalues $(\lambda_m)_{m\geq 0}$ associated to the integral operator $T_{K_N}$ given by (\ref{eq:formula_eigen-notions}). 
%The main purpose of this section is to obtain a tight control of the eigenvalue decay with their multiplicities under some assumptions on the non linear activations involved in the
%networks. 

\textbf{Super-Geometric Decay.} A first case of interest is the one studied in~\cite{azevedo2014sharp}. There tight estimates for eigenvalues $(\lambda_m)_{m\geq 0}$ are obtained, under the assumption that $|b_{m}/b_{m-1}|\in O(m^{-\delta})$ when $\delta$ is assumed to be strictly bigger than $1/2$. We present here a more general result, holding for any $\delta>0$.
%See Appendix~\ref{proof:menegato} for proof.
See Appendix~B for proof.
\begin{prop}
\label{prop:menegato}
If there exists $\delta>0$ such that
\begin{align}
\label{eq:b_n-final-f-2}
\left|\frac{b_{m}}{b_{m-1}}\right|\in O(m^{-\delta})
\end{align}
then, denoting $\alpha : =1/(1-2\delta)$, we have
\begin{equation*}
\lambda_m \in \begin{cases}
              \mathcal{O}\left( \frac{b_m}{2^{m+1}m^{({d-2})/2}} \right) & \text{if $\delta\geq 1/2$} \\
              \\
              \mathcal{O}\left( \frac{m^{\frac{m\delta}{2\alpha}+\frac{1}{\alpha}} b_m}{2^{m+1}m^{({d-2})/2}}\right)  & \text{if $0<\delta < 1/2$}
       \end{cases} \quad
\end{equation*}
% if $\delta\geq 1/2$ we have
% \begin{align*}
% %\label{decroissance}
% \lambda_m\in O\left(\frac{b_m}{2^{m+1}m^{({d-2})/2}}\right) \; .
% \end{align*}
% Otherwise, if $0<\delta<1/2$ we have
% \begin{align*}
% &\lambda_m\in O\left( \frac{m^{\frac{m\delta}{2\alpha}+\frac{1}{\alpha}} b_m}{2^{m+1}m^{({d-2})/2}}\right)\\
% &\text{where $\alpha : =\frac{1}{1-2\delta}$.}
% \end{align*}
\end{prop}
We have managed to obtain a tight control of the eigenvalue decay of $T_{K_N}$ ranked a non-increasing order with their multiplicities. 
%See Appendix~\ref{proof:spectrum_anal_gene} for proof.
\begin{prop}
\label{prop:spectrum_anal_gene}
Let also $\delta>0$ and denote $(\eta_m)_{m=0}^M$ the positive eigenvalues of the integral operator $T_{K_{N}}$ associated to the kernel $K_{N}$ ranked in a non-increasing order with their multiplicities, where $M\in\mathbb{N}\cup\{+\infty\}$. Then, under the same assumption as Prop. \ref{prop:menegato},
% If there exist  $\delta>0$ such that
% \begin{align}
% \label{eq:bngeome2}
% \left|\frac{b_{m}}{b_{m-1}}\right|\in O(m^{-\delta})
% \end{align}
$M=+\infty$ and there exists constant $1 \geq G >0$ independent of $\delta$ such that
\begin{align*}
\eta_m&\in \mathcal{O}\left(m^{-\frac{\delta}{s} m^{\frac{1}{d-1}}}\right) \; 
\text{where $s:=\frac{4(d-1)}{G}$.}
\end{align*}
\end{prop}

%\begin{wrapfigure}{r}{0.3\textwidth}\vspace*{-2.5ex}
%        \includegraphics[width=1.2\linewidth]{mlp/figures/b_n_decay.pdf}
%    \caption{Decay of $(|b_m/b_{m-1}|)_{m\geq 1}$. \label{fig:decay_bn}}
%\end{wrapfigure}
    
\textbf{Example.} Consider a two hidden layer MLP where activation functions are exponential ones. We have an explicit expression of the sequence $(b_m)_{m\geq 0}$ associated with $b_0=e^1$
\begin{align*}
b_{m+1}=\frac{1}{m+1}\sum_{k=0}^m \frac{b_{k}}{(m-k)!}.
\end{align*}
 We can compute the coefficients $(b_m)_{m\geq 0}$ thanks to this recurrence relation. See Appendix~\ref{proof:example} for illustrations.
%  In Figure \ref{fig:decay_bn}, we plot the rate of convergence of $(|b_m/b_{m-1}|)_{m\geq 1}$ (in blue) and compare it to $(1/m^{\delta})_{m\geq 1}$ where $\delta=1/3$ (in green) and $\delta = 1/5$ (in red). 
 For such networks, assumption~(\ref{eq:b_n-final-f-2}) holds for $\delta=1/5<1/2$ and therefore Prop. \ref{prop:spectrum_anal_gene} holds.


\textbf{Geometric Decay.} Another case of interest is when the coefficients $(b_m)_{m\geq 0}$ admits a Taylor decomposition with coefficients decreasing almost geometrically. Indeed we also obtain a tight control of the eigenvalue decay with their multiplicities of the integral operator $T_{K_N}$. 
%See Appendix~\ref{proof:eta-control} for proof.
See Appendix~C for proof.
\begin{prop}
\label{prop:eta-control}
Let us denote $(\eta_m)_{m=0}^M$ the positive eigenvalues of the integral operator $T_{K_{N}}$ associated to the kernel $K_{N}$ ranked in a non-increasing order with their multiplicities, where $M\in\mathbb{N}\cup\{+\infty\}$. If there exist $1>r>0$ and $0<c_2\leq c_1$ constants such that for all $m\geq 0$
\begin{align}
\label{eq:assump_geometric-spect}
c_2 r^{m} \leq b_m\leq c_1 r^m \;,
\end{align}
then $M=+\infty$ and there exits $0<Q_1<Q_2$ constants only depending on $d$ such that for all $m\geq 0$
\begin{align*}
C_2 e^{-Q_2\log(4/r)m^{\frac{1}{d-1}}} \leq \eta_{m}\leq C_1 e^{-Q_1\log(1/r)m^{\frac{1}{d-1}}} \; ,
\end{align*}
where $C_1= \frac{|S^{d-2}|\Gamma((d-1)/2)}{2}   \frac{2^{\frac{d-1}{2}}c_1}{1-r^2} $ and $C_2= |S^{d-2}|\Gamma((d-1)/2)\Gamma(1/2) L \frac{c_2}{2}$ and $L$ is a constant only depending on $d$.
\end{prop}

\textbf{Example.} Consider the case of a MLP where all the activation functions involved in the network are ReLU-type ones~\cite{zhang2016l1} such that $\sigma_1=...=\sigma_N=\sigma_{\text{sh}}$. Considering the function $f$ associated by the relation (\ref{eq:diff-sig-f}) to $\sigma_{\text{sh}}$,  the coefficients $(b_m)_{m\geq 0}$ of $f_N\circ...\circ f_1$ where $f_1 =...=f_N=f$ satisfies the RHS of (\ref{eq:assump_geometric-spect}) and the upper bound of the eigenvalues $(\eta_m)_{m\geq 0}$ of Prop. \ref{prop:eta-control} hold. 



% \medbreak
% Thanks to these controls, we obtain in the next section the convergence rates for Hilbertian envelope estimators, with non-trivial sets of distributions for the specific RKHSs introduced in Prop. 1 in the two regimes. In some cases, when recast in a nonparametric regression setting,  the rates can be considered optimal in the minimax sense. 

==> sections/section3.tex <==
\section{Multi-Layer Perceptron}
\label{sec:MLP-paper}
In this section we show that the functions generated by a multi-layer perceptron can be embed into an adaptative RKHS with respect to the nonlinear activations involved in the construction of the network. Moreover, we manage to obtain a tight control of the eigenvalue decay of the integral operator associated to kernel of interest in two different regimes: geometric and super-geometric. These regimes being completely determine by the nonlinear functions chosen. 

\subsection{Multi-Layer Perceptron Function Space}
Here we show that there exists an RKHS containing the function space $\mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N}$ for any activation functions, $(\sigma_i)_{i=1}^N$, admitting a Taylor decomposition on $\mathbb{R}$. Moreover, for well chosen activation maps, the kernel is a $cc$-universal kernel on $\mathcal{X}$ in~\cite{sriperumbudur2011universality} sense. See~Appendix~\ref{proof:lem-rkhs} for the proof. 

\begin{defn}[\textbf{$cc$-universal kernel}]
\label{def:cc-universal}
A continuous positive semi-definite  kernel k on a Hausdorff space $\mathcal{X}$ is said to be $cc$-universal if the RKHS, H induced by k is dense in $\mathcal{C}(\mathcal{X})$ endowed with the topology of compact convergence.
\end{defn}
\begin{prop}
\label{prop:RKHS-MLP}
Let $\mathcal{X}$ be any subspace of $\mathbb{R}^d$, $N\geq 1$, $(\sigma_i)_{i=1}^N$ functions which admits a Taylor decomposition on $\mathbb{R}$. Moreover let $(f_i)_{i=1}^N$ be the sequence of functions such that for every $i\in\{1,...,N\}$:
\begin{align}
\label{eq:diff-sig-f}
f_i(x)=\sum_{n\geq 0}\frac{|\sigma_i^{(n)}(0)|}{n!}x^n
\end{align}
The the RKHS $H_N$ of the kernel, $K_{N}$ defined on $\mathcal{X}\times\mathcal{X}$ by
\begin{align}
\label{eq:kernel-MLP}
K_{N}(x,x'):=f_N\circ...\circ f_1(\langle x,x'\rangle_{\mathbb{R}^d})
\end{align}
contains the function space $\mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N}$. 
If we assume in addition that for every $i\in\{1,...,N\}$ and $n\in\mathbb{N}$, $\sigma_i^{(n)}(0)\neq 0$, then the kernel $K_N$ is $cc$-universal.
\end{prop}

\begin{rmq}\textbf{Arbitrary Width Networks.} 
It is worth emphasizing that, for any number of weights $(m_i)_{i=1}^N$, the function space $\mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N,(m_i)_{i=1}^N}$ belongs to the RKHS we have just defined. 
In other words, the RKHS we define does \emph{not} require that all layers of the network are infinitely large as is commonly assumed in several previous works. 
\end{rmq}


% Thanks to Proposition~\ref{prop:RKHS-MLP}, we can have a direct control on the RKHS norm of the network through the spectral norm of its weights.
% \begin{coro}
% \label{coro:norm-mlp}
% For $(W^k)_{k=1}^{N+1}$ a sequence such that for all $k\in [|1,N+1|]$, $W^k\in\mathbb{R}^{m_{k-1}m_{k}}$ and $\mathcal{N}$ the function in $\mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N}$ associated, we have
% \begin{align*}
% \Vert \mathcal{N} \Vert_{H_N}^2 \leq \Vert W^{N+1} \Vert^2 f_N(\Vert W^{N} \Vert^{2} f_{N-1} (...f_1(\Vert W^1\Vert^2)...))
% \end{align*}
% where $\Vert.\Vert$ is the spectral norm.
% \end{coro}
% We can then obtain statistical bounds for deep networks such as as the ones in~\cite{zhang2016l1,zhang2017convexified,
% bartlett2017spectrally,bietti2017group}. Indeed the RKHS norm of the network allows one to get for instance generalization bounds involving Rademacher complexities as in~\cite{boucheron2005theory}. To be more precise, if $\mathcal{X}$ is compact and $\mathcal{Y}\subset [-M,M]$, then for any $\delta>0$ with a probability $\rho^n$ not less than $1-\delta$
% % \begin{align*}
% % R(\mathcal{N})& \leq \frac{1}{\ell}\sum_{i=1}^{\ell} (\mathcal{N}(x_i)- y_i)^2
% %  +\frac{2 G \Vert \mathcal{N} \Vert_{H_N}}{n}\sqrt{\sum_{i=1}^n K_N(x_i,x_i)} 
% % +\frac{2M^2}{\sqrt{n}}+ 3B\sqrt{\frac{ \log(\frac{2}{\delta})}{2n}} \; ,
% % \end{align*}
% \begin{align*}
% R(\mathcal{N})& \leq \frac{1}{\ell}\sum_{i=1}^{\ell} (\mathcal{N}(x_i)- y_i)^2+\mathcal{O}\left( \frac {\Vert \mathcal{N} \Vert_{H_N}}{\sqrt{n}}+ \sqrt{\frac{ \log(\frac{2}{\delta})}{2n}}\right) \; ,
% \end{align*}
% There are two major issue with these bounds. First they do not consider the approximation bias of the class of functions considered which is the major issue in high dimension. Moreover these generalization bounds may blow up as the number of parameters increases. We will see in the following that we manage to obtain learning rates of the RLS algorithm on the specific RKHSs associated to MLPs which deal with the two above issues.
% \medbreak
\paragraph{Activation functions.} For suitably chosen activation functions, the kernel $K_N$ defined above is $cc$-universal. Therefore the RKHS $H_N$ obtained approximate the Bayes risk of a large class of loss, in particular the least squares loss. See~Corollary 5.29~\cite{steinwart2008support}.
\begin{align*}
    \inf_{f\in H} \mathbb{E}[(f(X)-Y)^2]=\mathcal{R}^\star
\end{align*}
where $R^\star$ is the Bayes risk.
For instance, if at each layer the nonlinear function is $\sigma_{\text{exp}}(x)=\exp{x}$, then the RKHS becomes universal. There are other examples of activation functions satisfying the assumptions of the Proposition \ref{prop:RKHS-MLP}, such as the square activation $\sigma_2(x)=x^2$ as used in \cite{DBLP:journals/corr/LivniSS14}, the smooth hinge activation $\sigma_{\text{sh}}$, close to the rectifier linear unit (ReLU) activation, or a sigmoid-like function such as $\sigma_{\text{erf}}$,  similar to the sigmoid function. See~\cite{zhang2016l1}. 
\begin{align*}
\sigma_{\text{erf}}(x)&=\frac{1}{2}\left(1+\frac{1}{\sqrt{\pi}}\int_{-\sqrt{ \pi} x}^{\sqrt{ \pi} x} e^{-t^2}dt\right)&
\sigma_{\text{sh}}(x)&=\frac{1}{\sqrt{\pi}}\int_{-x}^x x e^{-t^2}dt +\frac{\exp(-\pi x^2)}{2\pi}
\end{align*}

Note that coefficients in the Taylor series of $\sigma_{\text{erf}}$ or $\sigma_{\text{sh}}$ are not nonnegative. Indeed the functions $(f_i)_{i=1}^N$ introduced in Proposition \ref{prop:RKHS-MLP} to build the RKHS $H_N$ associated the function space $\mathcal{F}_{\mathcal{X},(\sigma_{i})_{i=1}^N}$ may differ from the activation functions $(\sigma_i)_{i=1}^N$ involved in the construction of the network. Indeed as the relation in  Eq. (\ref{eq:diff-sig-f}) indicates, the functions $(f_i)_{i=1}^N$ admit a Taylor decomposition with non negative coefficients. These coefficients are the absolute values of the coefficients in the Taylor series of $(\sigma_i)_{i=1}^N$. However Proposition \ref{prop:RKHS-MLP} does not require any assumption on the sign of the coefficients of $(\sigma_i)_{i=1}^N$.
% are allowed to have negative coefficients in their Taylor decomposition. Indeed recall that the functions $(f_i)_{i=1}^N$, used to build the RKHS may differ from the nonlinear functions $(\sigma_i)_{i=1}^N$ involved in the network as it is indicated in Eq. (\ref{eq:diff-sig-f}).
% For example the function space $\mathcal{F}_{\mathcal{X},(\sigma_{\text{erf}})_{i=1}^N}$ can still be embedded in the RKHS defined in Proposition \ref{prop:RKHS-MLP} even if $\sigma_{\text{erf}}$ has negative coefficients in its Taylor decomposition. 
In the following we focus only on the functions $(f_i)_{i=1}^N$ related to the kernel $K_N$ as we want to study the proprieties of the RKHS $H_N$ associated.


\paragraph{Examples.} If we assume that for all $i\in\{1,...,N\}$, $f_i(1)=1$ then the norm is preserved across the layers as we obtain that
$K_i(x,x) = \Vert x\Vert_2^2$. Moreover, if we restrict the input space $\mathcal{X}$ to be the unit sphere, then we can consider a larger class of functions as we only need the $(f_i)_{i=1}^N$ to admit a Taylor expansion about 0 on $[-1,1]$. We list some classical functions which satistfy these assumptions \cite{bietti2017group}.
\begin{table}[h!]
\label{table:2}
\centering
\begin{tabular}{l|l}
polynomial & $f(t)=\frac{1}{p^p}(p-1+t)^p$\\
Inverse polynomial & $f(t)=\frac{1}{2-t}$\\
arc-cosine & $f(t)=\frac{1}{\pi}(\sin(\text{arcos}(t))+(\pi-\text{arcos}(t))\cos(\text{arcos}(t)))$ \\
Vovk's & $f(t)=\frac{1}{3}(1+t+t^2)$
\end{tabular}
\end{table}
\\
Note that the inverse polynomial kernel was used by \cite{zhang2016l1,zhang2017convexified} to build convex models of fully connected networks and two-layer convolutional neural networks, while the arc-cosine kernel appears in early deep kernel machines \cite{NIPS2009_3628}.

In the following we assume that the input space $\mathcal{X}$ is the unit sphere $S^{d-1}$ of $\mathbb{R}^d$ where $d\geq 2$. This is a common assumption in the literature, motivated by common input pre-processing procedures in signal processing and computer vision ~\cite{bach2017breaking,song2018mean,elad:2010}.

\subsection{Spectral Analysis of Multi-Layer Perceptrons}
In this section, we show our main results concerning the control the eigenvalue decay of the integral operators associated to the kernels introduced in Proposition \ref{prop:RKHS-MLP}. We exhibit two regimes: geometric and super-geometric depending on the choice of the nonlinear activations chosen. For that purpose let us first introduce some notations. Let $N\geq 1$, $d\geq 2$ and $(f_i)_{i=1}^N$ be a sequence of N real value functions satisfying assumptions of Proposition \ref{prop:RKHS-MLP}. Therefore $f_N\circ...\circ f_1$ admits a Taylor decomposition on $[-1,1]$, and we denote its non negative coefficients $(b_m)_{m\geq 0}$ such that
 \begin{align*}
 f_N\circ...\circ f_1(x):=\sum_{m\geq 0} b_m x^m.
\end{align*}
Moreover we denote $K_N$ the kernel associated as defined in Proposition \ref{prop:RKHS-MLP}. Recall that for such kernels we have an explicit formulation of the eigenvalues $(\lambda_m)_{m\geq 0}$ associated to the integral operator $T_{K_N}$ given by Eq. (\ref{eq:formula_eigen-notions}). The main purpose of this section is to obtain a tight control of the eigenvalue decay with their multiplicities under some assumptions on the non linear activations involved in the networks. 


\textbf{Super-Geometric Decay.} A first case of interest is the one studied in \cite{azevedo2014sharp}. Indeed in their work, they obtain sharp estimates for eigenvalues $(\lambda_m)_{m\geq 0}$ under the assumption that $|b_{m}/b_{m-1}|\in O(m^{-\delta})$ when $\delta$ is assumed to be strictly bigger than $1/2$. We extend the result for any $\delta>0$ in the following proposition. See Appendix~\ref{proof:menegato} for the proof.
\begin{prop}
\label{prop:menegato}
If there exist $\delta>0$ such that
\begin{align}
\label{eq:b_n-final-f-2}
\left|\frac{b_{m}}{b_{m-1}}\right|\in O(m^{-\delta})
\end{align}
then by denoting $\alpha : =\frac{1}{1-2\delta}$ we have

\begin{equation*}
\lambda_m \in \begin{cases}
              \mathcal{O}\left(\frac{b_m}{2^{m+1}m^{({d-2})/2}}\right) & \text{if $\delta\geq 1/2$} \\
              \\
              \mathcal{O}\left( \frac{m^{\frac{m\delta}{2\alpha}+\frac{1}{\alpha}} b_m}{2^{m+1}m^{({d-2})/2}}\right)  & \text{if $0<\delta < 1/2$}
       \end{cases} \quad
\end{equation*}
% if $\delta\geq 1/2$ we have
% \begin{align*}
% %\label{decroissance}
% \lambda_m\in O\left(\frac{b_m}{2^{m+1}m^{({d-2})/2}}\right) \; .
% \end{align*}
% Otherwise, if $0<\delta<1/2$ we have
% \begin{align*}
% &\lambda_m\in O\left( \frac{m^{\frac{m\delta}{2\alpha}+\frac{1}{\alpha}} b_m}{2^{m+1}m^{({d-2})/2}}\right)\\
% &\text{where $\alpha : =\frac{1}{1-2\delta}$.}
% \end{align*}
\end{prop}
From the above result, we manage to obtain a sharp control of the eigenvalue decay of $T_{K_N}$ ranked a non-increasing order with their multiplicities. See Appendix~\ref{proof:spectrum_anal_gene} for the proof.
\begin{prop}
\label{prop:spectrum_anal_gene}
Let also $\delta>0$ and let us denote $(\eta_m)_{m=0}^M$ the positive eigenvalues of the integral operator $T_{K_{N}}$ associated to the kernel $K_{N}$ ranked in a non-increasing order with their multiplicities, where $M\in\mathbb{N}\cup\{+\infty\}$. Then under the same assumption of Proposition \ref{prop:menegato}
% If there exist  $\delta>0$ such that
% \begin{align}
% \label{eq:bngeome2}
% \left|\frac{b_{m}}{b_{m-1}}\right|\in O(m^{-\delta})
% \end{align}
$M=+\infty$ and there exist constant $1 \geq G >0$ independent of $\delta$ such that
\begin{align*}
\eta_m&\in \mathcal{O}\left(m^{-\frac{\delta}{s} m^{\frac{1}{d-1}}}\right) \; 
\text{where $s:=\frac{4(d-1)}{G}$.}
\end{align*}
\end{prop}

\begin{wrapfigure}{r}{0.3\textwidth}\vspace*{-2.5ex}
        \includegraphics[width=1.2\linewidth]{mlp/figures/b_n_decay.pdf}
    \caption{Decay of $(|b_m/b_{m-1}|)_{m\geq 1}$. \label{fig:decay_bn}}
\end{wrapfigure}
    
\textbf{Example.} Consider the case of a MLP where all the activation functions considered are exponential functions. In particular, consider the case where $N=2$ and $f_2(t)=f_1(t)=\exp(t)$. For such networks, we have an explicit expression of the sequence $(b_m)_{m\geq 0}$ associated (See Appendix~\ref{proof:example}) with $b_0=e^1$
\begin{align*}
b_{m+1}=\frac{1}{m+1}\sum_{k=0}^m. \frac{b_{k}}{(m-k)!}
\end{align*}
We can compute the coefficients $(b_m)_{m\geq 0}$ thanks to this recurrence relation. In Figure \ref{fig:decay_bn}, we plot the rate of convergence of $(|b_m/b_{m-1}|)_{m\geq 1}$ (in blue) and compare it to $(1/m^{\delta})_{m\geq 1}$ where $\delta=1/3$ (in green) and $\delta = 1/5$ (in red). For such networks, assumption~(\ref{eq:b_n-final-f-2}) hold for $\delta=1/5<1/2$ and therefore Proposition \ref{prop:spectrum_anal_gene} hold.


\textbf{Geometric Decay.} Another case of interest is when the coefficients $(b_m)_{m\geq 0}$ admits a Taylor decomposition with coefficients decreasing almost geometrically. Indeed in that case we also obtain a tight control of the eigenvalue decay with their multiplicities of the integral operator $T_{K_N}$. See Appendix~\ref{proof:eta-control} for the proof.
\begin{prop}
\label{prop:eta-control}
Let us denote $(\eta_m)_{m=0}^M$ the positive eigenvalues of the integral operator $T_{K_{N}}$ associated to the kernel $K_{N}$ ranked in a non-increasing order with their multiplicities, where $M\in\mathbb{N}\cup\{+\infty\}$. If there exist $1>r>0$ and $0<c_2\leq c_1$ constants such that for all $m\geq 0$
\begin{align}
\label{eq:assump_geometric-spect}
c_2 r^{m} \leq b_m\leq c_1 r^m \;,
\end{align}
then $M=+\infty$ and there exits $0<Q_1<Q_2$ constants only depending on $d$ such that for all $m\geq 0$
\begin{align*}
C_2 e^{-Q_2\log(4/r)m^{\frac{1}{d-1}}} \leq \eta_{m}\leq C_1 e^{-Q_1\log(1/r)m^{\frac{1}{d-1}}} \; ,
\end{align*}
where $C_1= \frac{|S^{d-2}|\Gamma((d-1)/2)}{2}   \frac{2^{\frac{d-1}{2}}c_1}{1-r^2} $ and $C_2= |S^{d-2}|\Gamma((d-1)/2)\Gamma(1/2) L \frac{c_2}{2}$ and $L$ is a constant only depending on $d$.
\end{prop}

\textbf{Example.} Consider the case of a MLP where all the activation functions involved in the network are ReLU-like activations \cite{zhang2016l1} such that $\sigma_1=...=\sigma_N=\sigma_{\text{sh}}$. By considering the function $f$ associated by the relation Eq. (\ref{eq:diff-sig-f}) to $\sigma_{\text{sh}}$,  the coefficients $(b_m)_{m\geq 0}$ of $f_N\circ...\circ f_1$ where $f_1 =...=f_N=f$ satisfies the RHS of (\ref{eq:assump_geometric-spect}) and the upper bound of the eigenvalues $(\eta_m)_{m\geq 0}$ of Proposition \ref{prop:eta-control} hold.

\medbreak
Thanks to these controls, we obtain in the next section the learning rates of the regularized least square algorithm on non-trivial sets of distributions for the specific RKHSs introduced in Proposition 1 in two regimes. Moreover in some cases, we show that these rates are optimal in the minmax sense.










==> sections/section4-neurips.tex <==
\section{Statistical Bounds for Hilbertian Least-squares Estimators}
\label{sec:RLS-MLP}

We present here general statistical bounds on the performance of regularized least-squares estimator. These statistical bounds can be used for at least two purposes which we develop here. First, they can be used to describe the statistical performance of a regularized least-squares estimator when this estimator can be computed exactly in practice. 
This applies for instance to the kernel-based deep networks developed in~\cite{shankar2020neural} and to kernel-based methods with kernels on spheres~\cite{steinwart2008support}. Second, they can be used to obtain an optimistic estimate of the statistical performance of a deep network estimator via its Hilbertian envelope estimator (\ref{eq:rls-obj}), when the deep network estimator cannot be computed exactly in practice. It is worthwhile to underscore, that, as of today, no theoretical framework is able to tackle all aspects of deep network analysis, function approximation, numerical optimization, and statistical prediction. Here we trade numerical optimization (our results assume perfect optimization) for function approximation (our results do not assume realizability) and statistical prediction (our results match minimax rates). For simplicity of exposition, we focus on this second case in order to obtain an optimistic estimate of the power of generalization of deep networks; see Appendix~\ref{sec:RLS} for the first case.

\paragraph{Learning from data.} 
% The desiderata for the statistical bounds we wish to obtain is to uncover the effect of the network depth \textit{i.e.} the length of the chain composition defining the network. There are two regimes that arise: i) geometric case; ii) super-geometric case. A multi-layer perceptron can be analyzed via an Hilbertian envelope estimator thanks to the results presented earlier.
\medbreak
Given a dataset $\mathbf{z} = {(x_i,y_i)}_{i=1}^{\ell}$ independently sampled from an unknown distribution $\rho(x, y)$ on $Z:=\mathcal{X}\times \mathcal{Y}$ where $\mathcal{Y}\subset\mathbb{R}$, the goal of the least-squares regression is to estimate the conditional mean function $f_{\rho}:\mathcal{X}\rightarrow \mathbb{R}$ given by $f_{\rho}(x):= \mathbb{E}(Y |X = x)$. The joint distribution $\rho(x, y)$, the marginal distribution $\rho_\mathcal{X}$, and the conditional distribution $\rho(.|x)$, are related through $\rho(x, y) =\rho_{\mathcal{X}}(x)\rho(y|x)$.
% We call the $f_\mathbf{z}$ the learning method or the estimator and the learning algorithm is the procedure that, for any sample size $\ell \in \mathbb{N}$ and training set $\mathbf{z} \in Z^{\ell}$ yields the learned function or estimator $f_\mathbf{z}$. If the output space $\mathcal{Y}\subset \mathbb{R}$, given a function $f : \mathcal{X} \rightarrow \mathcal{Y}$ , the ability of $f$ to describe the distribution $\rho$ is measured by its expected risk
% \begin{align}
% R(f):=\int_{\mathcal{X}\times \mathcal{Y}}(f(x)-y)^{2}\,d\rho(x,y) \; .
% \end{align}
% The minimizer over the space of measurable  $\mathcal{Y}$-valued functions on $\mathcal{X}$ is the function
% \begin{align}
% f_{\rho}(x):=\int_{\mathcal{Y}} y d\rho(y|x) \; .
% \end{align}
% The final aim of learning theory is to find an algorithm such that $R(f_\mathbf{z})$ is close to $R(f_\rho)$ with high probability.
Consider as hypothesis space a Hilbert space $H$ of functions $f:\mathcal{X}\rightarrow \mathcal{Y}$. For any regularization parameter $\lambda>0$ and training set $\mathbf{z}\in Z^{\ell}$, the regularized least-square (RLS) estimator $f_{H,\mathbf{z},\lambda}$ is the solution of
\begin{align}
\label{eq:rls-obj}
\argminB_{f\in H} \left\{ \frac{1}{\ell}\sum_{i=1}^{\ell}( f(x_i)-y_i)^2+\lambda \Vert f\Vert_{H}^2\right\} \; .
\end{align}
% Let us recall basic definitions yet important for the exposition of the convergence rates. The goal is to establish bounds, either in expectation or in probability, on
% $\Vert f_{H_N,\mathbf{z},\lambda}-f_{\rho} \Vert_{\rho}$ where the norm  $\Vert .\Vert_{\rho}$ is the $L_2^{\rho_{\mathcal{X}}}$-norm and $H_N$ is the RKHS defined in Prop. \ref{prop:RKHS-MLP} associated to a MLP. Let $\mathcal{G}$ a class of Borel probability distributions on $\mathcal{X}\times\mathcal{Y}$ satisfying general assumptions.
% \begin{defn}(Upper rate of convergence)
% \label{defn:upper-rate}
% A sequence $(a_{\ell})_{\ell\geq 1}$ of
% positive numbers is called upper rate of convergence in $L_2^{d\rho_{\mathcal{X}}}$ norm over the model $\mathcal{G}$, for the sequence of estimated solutions $(f_{\mathbf{z},\lambda_{\ell}})_{\ell\geq 1}$ using regularization parameters $(\lambda_{\ell})_{\ell\geq 0}$ if
% \begin{equation*}
% \lim_{\tau\rightarrow +\infty}\lim \sup_{\ell\rightarrow\infty}\sup_{\rho\in \mathcal{G}} \rho^{\ell}\left(\mathbf{z}:\Vert f_{\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2>\tau a_{\ell}\right)=0 \, .
% \end{equation*}
% \end{defn}
% \begin{defn}(Minimax Lower Rate of Convergence)
% A sequence $(v_{\ell})_{\ell\geq 1}$ of
% positive numbers is called minimax lower rate of convergence in $L_2^{d\rho_{\mathcal{X}}}$ norm over the model $\mathcal{G}$ if
% \begin{align*}
%  \lim_{\tau\rightarrow 0^{+}}\lim\inf_{\ell\rightarrow\infty}\inf_{f_{\mathbf{z}}}\sup_{\rho\in\mathcal{G}} \rho^{\ell}\left(\mathbf{z}:\Vert f_{\mathbf{z}}-f_{\rho}\Vert_{\rho}^2>\tau v_{\ell}\right)=1
% \end{align*}
% where the infimum is taken over all measurable learning methods with respect to $\mathcal{G}$.
% \end{defn}
% Such sequences $(v_{\ell})_{\ell\geq 1}$ are called minimax lower rates. Every sequence $( \hat{v}_{\ell})_{\ell\geq 1}$ decreasing at least with the same rate as $(v_{\ell})_{\ell\geq 1}$ is a lower rate for this set of probability measures and at least the same lower rate holds on any larger set of probability measures. When the rate of the sequence of learned functions coincides with the minimax lower rates, it is then said to be optimal in the minimax sense.
%\medbreak
Let $N\geq 1$, $d\geq 2$ and $(f_i)_{i=1}^N$ be a sequence of N real value functions satisfying assumptions of Prop.\ref{prop:RKHS-MLP}. Denote $(b_m)_{m\geq 0}$ the coefficients in the Taylor series about 0 of $f_N\circ...\circ f_1$. The hypothesis space considered is the Hilbert space $H_N$ associated with the kernel $K_{N}(x,x')=f_N\circ...\circ f_1(\langle x,x'\rangle)$. Note that here we focus specifically on the RKHSs associated to MLPs. Define the integral operator on $L_2^{d{\rho_{\mathcal{X}}}}(\mathcal{X})$ associated as 
$T_{\rho}(f)(y) =  \int_{\mathcal{X}} K_N(x,y)f(x){d\rho_{\mathcal{X}}}(x)$.
% $$\begin{array}{ccccc}
% T_{\rho} & : &  L_2^{d{\rho_{\mathcal{X}}}}(\mathcal{X}) & \to &  L_2^{d{\rho_{\mathcal{X}}}}(\mathcal{X})\\
%  & & f &\to & \int_{\mathcal{X}} K_N(x,.)f(x){d\rho_{\mathcal{X}}}(x)
% \end{array}$$
% Since $k$ is bounded, $T_{\rho}$ is self-adjoint, positive semi-definite and trace-class~\cite{blanchard2008finite}. Let us denote $(\mu_i)_{i\in I} \in \ell_1(I)$ its eigenvalues ranked in a non decreasing order. We shall assume in the following that $I=\mathbb{N}$. When $I$ is finite, results can be found for example in~\cite{caponnetto2007optimal}. 
We work here under general assumptions on the set of probability measures $\rho$ on $\mathcal{X}\times\mathcal{Y}$.

% \textbf{Setting.} Given a dataset $\mathbf{z} = {(x_i,y_i)}_{i=1}^{\ell}$ independently sampled from an unknown distribution $\rho(x, y)$ on $Z:=\mathcal{X}\times \mathcal{Y}$ where $\mathcal{Y}\subset\mathbb{R}$, the goal least-squares regression is to estimate the conditional mean function $f_{\rho}:\mathcal{X}\rightarrow \mathbb{R}$ given by $f_{\rho}(x):= E(Y |X = x)$. Here the hypothesis space considered is the Hilbert space associated with the kernel defined in Prop. \ref{prop:RKHS-MLP}. Note that here we focus specifically on the RKHSs associated to MLPs.
% More precisely, let $N\geq 1$, $d\geq 2$ and $(f_i)_{i=1}^N$ be a sequence of N real value functions such that $f_N\circ...\circ f_1$ admits a Taylor decomposition on $[-1,1]$ with non negative coefficients $(b_m)_{m\geq 0}$:
% \begin{align*}
%  f_N\circ...\circ f_1(x):=\sum_{m\geq 0} b_m x^m
% \end{align*}
% and let $H_N$ be the RKHS associated with the kernel $K_N$ defined on $S^{d-1}$ by:
% \begin{align*}
% K_{N}(x,x'):=f_N\circ...\circ f_1(\langle x,x'\rangle_{\mathbb{R}^d}) ; .
% \end{align*}
\begin{assump}\textbf{ [Probability measures on $\mathcal{X} \times \mathcal{Y}$].} Let $\mathcal{P}$ a set of probability measures on $\mathcal{X}$. Furthermore, let $B, B_{\infty}, L, \sigma> 0$ be some constants and $0< \beta \leq 2$ a parameter. Then we denote by $\mathcal{F}_{B, B_{\infty}, L, \sigma,\beta}(\mathcal{P})$ the set of all probability measures $\rho$ on $\mathcal{X} \times\mathcal{Y}$ with the following properties. \\
(i) $\rho_{\mathcal{X}}\in\mathcal{P}$, $\int_{\mathcal{X}\times\mathcal{Y}}y^2d\rho(x,y) < \infty$, $\Vert f_{\rho}\Vert_{L_{\infty}^{d\rho_{\mathcal{X}}}}^2 \leq  B_{\infty}$\\
(ii) There exists $g\in L_2^{d\rho_{\mathcal{X}}}(\mathcal{X})$ such that $f_\rho=T_{\rho}^{\beta/2}g$ and $\Vert g\Vert_{\rho}^2\leq B$\\
(iii)  there exist $\sigma>0$ and $L>0$ such that  $\int_{\mathcal{Y}} |y-f_{\rho}(x)|^m d\rho(y|x)\leq \frac{1}{2}m!L^{m-2}$.
\end{assump}
% A sufficient condition  for the last assumption is that $\rho$ is concentrated on $\mathcal{X} \times [-M,M]$ for some constant $M>0$. 

For $\omega\geq 1$, we denote by $\mathcal{W}_{\omega}$ the set of all probability measures $\nu$ on $S^{d-1}$ which satisfying $d\nu/d\sigma_{d-1}< \omega$.
Furthermore, we introduce for a constant $\omega \geq 1 > h > 0$, $\mathcal{W}_{\omega,h}\subset\mathcal{W}_{\omega}$ the set of probability measures $\nu$ on $S^{d-1}$ which additionally satisfy 
$d\nu/d\sigma_{d-1}> h$.
In the following we denote $\mathcal{G}_{\omega, \beta}:=\mathcal{F}_{H_N,B, B_{\infty}, L, \sigma,\beta}(\mathcal{W}_{\omega})$
and $\mathcal{G}_{\omega,h,\beta}:=\mathcal{F}_{H_N,B, B_{\infty}, L, \sigma,\beta}(\mathcal{W}_{\omega,h})$. 

% \begin{rmq}
% It is worth noting that we do not make any assumption on the set of distributions related to the eigenvalue decay. Indeed, the spectral analysis of the MLPs obtained in section \ref{sec:MLP-paper}, allows us to define a non-trivial set of distributions adapted for these specific kernels. This should be contrasted with the assumptions considered in section \ref{sec:RLS}.
% \end{rmq}

\paragraph{Geometric Case}
We first consider the case corresponding to a geometric eigendecay. The convergence rates below are minimax optimal  for nonparametric regression in RKHS. Corresponding rates along with proofs can be found 
in Appendix~C.
%in Appendix~\ref{proof:rls-geo}.

\begin{thm}
\label{thm:rls-geo}
Let us assume that there exists $1>r>0$, $0<c_1$ some constants such that the sequence $(b_m)_{m\geq 0}$ satisfies for all $m\geq 0$:
\begin{align}
\label{eq:assump_geometric}
 b_m \leq c_1 r^m
\end{align}
Let also $w\geq 1$ and $0<\beta\leq 2$.
Then there exists $A,C>0$ some constants independent of $\beta$ such that for any $\rho\in \mathcal{G}_{\omega, \beta}$ and $\tau\geq 1$ we have\\
(i) If $\beta> 1$, then for $\lambda_{\ell}=\frac{1}{\ell^{1/\beta}}$ and
$\ell\geq \text{max}\left(e^{\beta},\left(\frac{A}{\beta^{d-1}}\right)^{\frac{\beta}{\beta-1}}\tau^{\frac{2\beta}{\beta-1}} \log(\ell)^{\frac{d-1\beta}{\beta-1}}\right)$, with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
    \begin{align*}
\Vert f_{H_N,\mathbf{z},\lambda}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{d-1}}{\ell}
    \end{align*}\\
(ii) If $\beta = 1$, then for $\lambda_{\ell}=\frac{\log(\ell)^{\mu}}{\ell}$, $\mu>d-1>0$ and  $\ell\geq \text{max}\left(\exp\left((A\tau)^{\frac{1}{\mu-d-1}}\right),e^{1}\log(\ell)^{\mu}\right)$, with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
    \begin{align*}
    \Vert f_{H_N,\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{\mu}}{\ell^{\beta}}
    \end{align*}\\
(iii) If $\beta < 1$, then for $\lambda_\ell=\frac{\log(\ell)^{\frac{d-1}{\beta}}}{\ell}$ and $\ell\geq \text{max}\left(\exp\left((A\tau)^{\frac{\beta}{d-1(1-\beta)}}\right),e^{1}\log(\ell)^{\frac{d-1}{\beta}}\right)$, with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
    \begin{align*}
    \Vert f_{H_N,\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{d-1}}{\ell^{\beta}}
    \end{align*}
\end{thm}

\textbf{Example.} Consider the case where $\sigma_1=...=\sigma_N=\tanh$. Indeed recall that $\tanh$ admits a Taylor decomposition on $[-1,1]$ with coefficients satisfying assumption (\ref{eq:assump_geometric}) and that $\tanh([-1,1])\subset [-1,1]$. Therefore the functions $(f_i)_{i=1}^N$ associated, even if we may have to renormalize $(f_i)_{i=1}^N$ by their largest values on $[-1,1]$, admit a Taylor decomposition on $[-1,1]$ and the coefficients $(b_m)_{m\geq 0}$ in the Taylor series about 0 of $f_N\circ...\circ f_1$ satisfy assumption (\ref{eq:assump_geometric}). Thus Theorem \ref{thm:rls-geo} can be applied. This case corresponds to the nonlinear function used in \textit{LeNet5}. Note also that the sigmoid function defined as $\sigma:=(1+\exp(-x))^{-1}$ is just a rescaled and shifted version of $\tanh$ which therefore can be used here.
%\begin{itemize}
%\item  If $\beta> 1$, then for $\lambda_{\ell}=\frac{1}{\ell^{1/\beta}}$ and
%$\ell\geq \text{max}\left(e^{\beta},\left(\frac{A}{\beta^{d-1}}\right)^{\frac{\beta}{\beta-1}}\tau^{\frac{2\beta}{\beta-1}} \log(\ell)^{\frac{d-1\beta}{\beta-1}}\right)$, with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
%    \begin{align*}
%\Vert f_{H_N,\mathbf{z},\lambda}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{d-1}}{\ell}
%    \end{align*}
%    \item  If $\beta = 1$, then for $\lambda_{\ell}=\frac{\log(\ell)^{\mu}}{\ell}$, $\mu>d-1>0$ and  $\ell\geq \text{max}\left(\exp\left((A\tau)^{\frac{1}{\mu-d-1}}\right),e^{1}\log(\ell)^{\mu}\right)$, with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
%    \begin{align*}
%    \Vert f_{H_N,\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{\mu}}{\ell^{\beta}}
%    \end{align*}
%    \item  If $\beta < 1$, then for $\lambda_\ell=\frac{\log(\ell)^{\frac{d-1}{\beta}}}{\ell}$ and $\ell\geq \text{max}\left(\exp\left((A\tau)^{\frac{\beta}{d-1(1-\beta)}}\right),e^{1}\log(\ell)^{\frac{d-1}{\beta}}\right)$, with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
%    \begin{align*}
%    \Vert f_{H_N,\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{d-1}}{\ell^{\beta}}
%    \end{align*}
%\end{itemize}


% \textbf{Example.} As we have restricted the input space to be the unit sphere, we can consider the case where $\sigma_1=...=\sigma_N=\tanh$. Indeed recall that $\tanh$ admits a Taylor decomposition on $[-1,1]$ with coefficients satisfying assumption (\ref{eq:assump_geometric}) and that $\tanh([-1,1])\subset [-1,1]$. Therefore the functions $(f_i)_{i=1}^N$ associated, even if we may have to renormalize $(f_i)_{i=1}^N$ by their largest values on $[-1,1]$, admit a Taylor decomposition on $[-1,1]$ and the coefficients $(b_m)_{m\geq 0}$ in the Taylor series about 0 of $f_N\circ...\circ f_1$ satisfy assumption (\ref{eq:assump_geometric}). Thus Th.  \ref{thm:rls-geo} can be applied. This case corresponds to the nonlinear function used in \textit{LeNet5}.


% \medbreak
% Moreover the following Th.  investigates the optimality of our learning rates. See proof in Appendix \ref{proof:rls-geo}.
% \begin{thm}
% \label{thm:lower-geo}
% Let us assume that there exists $0<c_2<c_1$ such that for all $m\geq 0$:
% \begin{align*}
%   c_2 r^m \leq b_m \leq c_1 r^m
% \end{align*}
% Then for any $\omega\geq 1 > h >0$ such that $\mathcal{W}_{\omega,h}$ is not empty it holds 
% \begin{align*}
%  \lim_{\tau\rightarrow 0^{+}}\lim\inf_{\ell\rightarrow\infty}\inf_{f_{\mathbf{z}}}\sup_{\rho\in\mathcal{G}_{\omega,h,\beta}} \rho^{\ell}\left(\mathbf{z}:\Vert f_{\mathbf{z}}-f_{\rho}\Vert_{\rho}^2>\tau b_{\ell}\right)=1
% \end{align*}
% where $b_{\ell}=\frac{\log(\ell)^{d-1}}{\ell}$. The infimum is taken over all measurable learning methods with respect to $\mathcal{G}_{\omega,h,\beta}$.
% \end{thm}
% Therefore for such networks, when $\beta>1$ the learning rates of RLS stated in Th.~\ref{thm:rls-geo} coincides with the minimax lower
% rates from Th.~\ref{thm:lower-geo} and can therefore be considered optimal in the minimax sense when recast in the context of nonparametric regression.


% \begin{rmq}
% Instead of the regularized least-squares algorithm, let us consider for any sequence $(m_i)_{i=1}^N\in\mathbb{N}_{*}^N$ the following estimator:
% \begin{align*}
%   \widehat{f}_{(m_i)_{i=1}^N}\in \argminB_{f\in \mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N,(m_i)_{i=1}^N}} \left\{ \frac{1}{\ell}\sum_{i=1}^{\ell}( f(x_i)-y_i)^2 \right\} 
% \end{align*}
% Then the results of Th. s \ref{thm:rls-geo} and \ref{thm:lower-geo} suggests that for any choice of $(m_i)_{i=1}^N$, the generalization performance of such estimator cannot have better asymptotic rates than the one obtained by regularized least square algorithm in this setting. Indeed, on the set of distributions introduced, our estimator matches the minmax rates. Therefore any other estimator cannot do better in the minmax sense.   
% \end{rmq}

% \textbf{Example.} Consider the case where $f_1$ is the inverse polynomial function $f_1(x)=1/(2-x)$, while
% the other layers are polynomial functions. Then, for all $k\geq 2$, $f_k\circ ...\circ f_1$ satisfy also Assumption~\ref{eq:assump_geometric}. Thus  Th. ~\ref{thm:rls-geo} can be applied. On the one hand, the convergence rate remains the same asymptotically as the network gets deeper. On the other hand, the space in which the target function is assumed to live is allowed to grow as the network gets deeper. \todo{a modifier}

% \textbf{Example.} Consider the case where $f_1$ is the inverse polynomial function $f_1(x)=1/(2-x)$, while
% the other layers are polynomial functions. Then, for all $k\geq 2$, $f_k\circ ...\circ f_1$ satisfy also assumption~(\ref{eq:assump_geometric}) and the result of Th.  \ref{thm:rls-geo} hold.

%Super-geometric case%
% \subsection{Super-geometric Case}
% Another regime of interest is the one where the composition of nonlinear functions involved in the network admits a Taylor decomposition with coefficients decreasing super-geometrically. As in the geometric case, the goal is to obtain a control the of the eigenvalues associated with the integral operator $T_{K_N}$. See Appendix~\ref{proof:rls-super-geo}.
% \begin{thm}
% \label{thm:super-geo}
% Assume that there exists $1 > \delta>0$ such that
% \begin{align}
% \label{eq:b_n-final}
% \left|\frac{b_{m}}{b_{m-1}}\right|\in O(m^{-\delta}) \; .
% \end{align}
% Let also $0<\beta\leq 2$ and $\omega>0$.
% Then there exist a constant $C$ independent of $\beta$ such that
% for any $\rho\in \mathcal{G}_{\omega,\beta}$ and $\tau\geq 1$ we have:
% \begin{itemize}
% \item  If $\beta> 1$, then there exists $\ell_{\tau}>0$ such that for all $\ell\geq \ell_{\tau}$ and $\lambda_{\ell}=\frac{1}{\ell^{1/\beta}}$, with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
%     \begin{align*}
%     \Vert f_{H_N,\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{d-1}}{[\log(\log(\ell))]^{d-1}\ell}
%     \end{align*}
%     \item  If $\beta = 1$, then there exists $\ell_{\tau}>0$ such that for all $\ell\geq \ell_{\tau}$, $\lambda_{\ell}=\frac{\log(\ell)^{\mu}}{[\log(\log(\ell))]^{\mu}\ell}$ and $\mu\geq d-1$, with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
%     \begin{align*}
%     \Vert f_{H_N,\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{\mu}}{[\log(\log(\ell))]^{\mu}\ell}
%     \end{align*}
%     \item If $\beta < 1$, then there exists $\ell_{\tau}>0$ such that for all $\ell\geq \ell_{\tau}$ and $\lambda_{\ell}=\frac{\log(\ell)^{\frac{d-1}{\beta}}}{[\log(\log(\ell))]^{\frac{d-1}{\beta}}\ell}$ with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
%     \begin{align*}
%     \Vert f_{H_N,\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{d-1}}{[\log(\log(\ell))]^{d-1}\ell^{\beta}}
%     \end{align*}
% \end{itemize}
% \end{thm}
% As expected, in that regime, we obtain faster rates compared to the geometric case as the eigenvalues decrease faster. 
% %Moreover as in the geometric case, we can deduce asymptotic rates. See Appendix Corollary~\ref{coro:exp-rate}.
% \medbreak

% % \textbf{Example.} Consider the case where $f_1$ is the exponential function, while the other layers are polynomial functions. Then $f_N\circ ...\circ f_1$ satisfies also assumption~(\ref{eq:b_n-final}). Then Thoerem~\ref{thm:super-geo} can be applied.
% \medbreak
% % \textbf{Example 1.} Let consider the case where $N=2$ and $f_2(t)=f_1(t)=\exp(t)$. For such networks, we have an explicit expression of the sequence $(b_m)_{m\geq 0}$ (See Appendix~\ref{proof:example}) with $b_0=e^1$
% % \begin{align*}
% % b_{m+1}=\frac{1}{m+1}\sum_{k=0}^m. \frac{b_{k}}{(m-k)!}
% % \end{align*}
% % We can compute the coefficients $(b_m)_{m\geq 0}$ thanks to this recurrence relation. In Figure \ref{fig:decay_bn}, we plot the rate of convergence of $(|b_m/b_{m-1}|)_{m\geq 1}$ (in blue) and compare it to $(1/m^{\delta})_{m\geq 1}$ where $\delta=1/3$ (in green) and $\delta = 1/5$ (in red). For such networks, assumption~(\ref{eq:b_n-final}) hold for $\delta=1/5<1/2$ and therefore Th.  \ref{thm:super-geo} hold.


% % \textbf{Example 2.} Consider the case where $f_1$ is the exponential function, while the other layers are polynomial functions. Then $f_N\circ ...\circ f_1$ satisfies also assumption~(\ref{eq:b_n-final}). Then Th. ~\ref{thm:super-geo} can be applied. \todo{A modifier}

\textbf{Discussion.} Note that, compared to the polynomial rates obtained in \cite{bach2017breaking,schmidthieber2019nonparametric}, our rates are actually faster asymptotically. Note also that, in geometric case, the rates obtained for RLS are optimal in the minimax sense and therefore no better rate can be obtained within this framework. See Appendix~\ref{proof:rls-geo} for the proof. Moreover the rates obtained highlight an interesting phenomenon. Indeed the rates obtained
are free-dimension with respect to the number of parameters considered in the network and therefore allow the number of network parameters to be much larger than the input dimension. 

\paragraph{Convergence rates and network depth.} Another important consequence of the rates obtained in Theorem~\ref{thm:rls-geo} is that the number of layers of the network can increases without scarifying the learning rates.
%See Appendix~\ref{proof:effect_depth_geo} for proof.
See Appendix~\ref{proof:rls-super-geo} for proof.
\begin{prop}
\label{prop:effect_depth_geo}
Let $N\geq 1$, $d\geq 2$ and $(f_i)_{i=1}^N$ be a sequence of N real value functions satisfying assumptions of Prop. \ref{prop:RKHS-MLP} and denote $(b_m)_{m\geq 0}$ the coefficients in the Taylor series about 0 of $f_N\circ...\circ f_1$. Let also $q\geq 1$ and $f_{N+1},...f_{N+q}$ polynomial functions of arbitrary degree with non negative coefficients. Assume that there exists $1>r>0$, $0<c_1$ some constants such that the sequence $(b_m)_{m\geq 0}$ satisfies for all $m\geq 0$, $b_m \leq c_1 r^m$ then $f_{N+q}\circ...\circ f_1(x)$ admits a Taylor decomposition about 0 with non negative coefficients and by denoting $(a_m)_{m\geq 0}$ those coefficients, we obtain that there exists $1>r'>r>0$ and $0<c_1'$ such that for all $m\geq 0$, $a_m \leq c_1' r'^m$.
\end{prop}
For a network already in the geometric regime adding more layers would not result in another regime. %Therefore as soon as the network reaches the geometric regime, adding layers to the network does not affect the learning rate of convergence. 
On the other hand, adding layers would allow to reach a greater set of target functions.
% Indeed observe that the eigenvalue decay decreases slower when the number of layers increases. Therefore, the RKHS obtained become larger. The eigenvalue decay gives a concrete notion of the complexity of the function space considered. Given an eigensystem  $(\mu_m)_{m\geq 0}$ and $(e_m)_{m\geq 0}$ of positive eigenvalues and eigenfunctions respectively of the integral operator $T_{K_N}$, associated with the Kernel $K_N$, defined on $L_2(S^{d-1})$, the RKHS $H_N$ associated is defined as:
% $$ H_N=\left\{f\in L_2(\mathcal{I})\text{:\quad} f = \sum_{m\geq 0} a_m e_m \text{\quad with\quad } \left( \frac{a_m}{\sqrt{\mu_m}} \right)\in\ell_2\right\}$$
% endowed with the following inner product:
% \begin{align*}
% \langle f,g \rangle=\sum_{m\geq 0} \frac{a_m b_m}{\mu_m}
% \end{align*}
% From this definition, we see immediately that as the eigenvalues of the integral operator decreases slower, the RKHS becomes larger. 
Therefore adding layers allows the function space of the target function to grow, while the learning rates remain the same. Similar results hold also in the super-geometric case. 
See Appendix~C for proof.
%See Appendix~\ref{proof:effect_depth_geo} for proof.

==> sections/section4.tex <==
\section{Regularized Least-Squares for Multi-layer Perceptrons}
\label{sec:RLS-MLP}
We can now get the statistical bounds for regularized least-squares with a multi-layer perceptron (MLP). 
The desiderata for the statistical bounds we wish to obtain is to uncover the effect of the network depth \textit{i.e.} the length of the chain composition defining the network. There are two regimes that arise: i) geometric case; ii) super-geometric case. We show now that a multi-layer perceptron can be concisely described thanks to the results presented earlier.
\medbreak
Given a dataset $\mathbf{z} = {(x_i,y_i)}_{i=1}^{\ell}$ independently sampled from an unknown distribution $\rho(x, y)$ on $Z:=\mathcal{X}\times \mathcal{Y}$ where $\mathcal{Y}\subset\mathbb{R}$, the goal least-squares regression is to estimate the conditional mean function $f_{\rho}:\mathcal{X}\rightarrow \mathbb{R}$ given by $f_{\rho}(x):= E(Y |X = x)$. The joint distribution $\rho(x, y)$, the marginal distribution $\rho_\mathcal{X}$, and the conditional distribution $\rho(.|x)$, are related through $\rho(x, y) =\rho_{\mathcal{X}}(x)\rho(y|x)$.
% We call the $f_\mathbf{z}$ the learning method or the estimator and the learning algorithm is the procedure that, for any sample size $\ell \in \mathbb{N}$ and training set $\mathbf{z} \in Z^{\ell}$ yields the learned function or estimator $f_\mathbf{z}$. If the output space $\mathcal{Y}\subset \mathbb{R}$, given a function $f : \mathcal{X} \rightarrow \mathcal{Y}$ , the ability of $f$ to describe the distribution $\rho$ is measured by its expected risk
% \begin{align}
% R(f):=\int_{\mathcal{X}\times \mathcal{Y}}(f(x)-y)^{2}\,d\rho(x,y) \; .
% \end{align}
% The minimizer over the space of measurable  $\mathcal{Y}$-valued functions on $\mathcal{X}$ is the function
% \begin{align}
% f_{\rho}(x):=\int_{\mathcal{Y}} y d\rho(y|x) \; .
% \end{align}
% The final aim of learning theory is to find an algorithm such that $R(f_\mathbf{z})$ is close to $R(f_\rho)$ with high probability.
Let us now introduce the regularized least-squares algorithm.
Consider as hypothesis space a Hilbert space $H$ of functions $f:\mathcal{X}\rightarrow \mathcal{Y}$. For any regularization parameter $\lambda>0$ and training set $\mathbf{z}\in Z^{\ell}$, the Regularized Least-Square (RLS) estimator $f_{H,\mathbf{z},\lambda}$ is the solution of
\begin{align}
\argminB_{f\in H} \left\{ \frac{1}{\ell}\sum_{i=1}^{\ell}( f(x_i)-y_i)^2+\lambda \Vert f\Vert_{H}^2\right\} \; .
\end{align}
% Let us recall basic definitions yet important for the exposition of the convergence rates. The goal is to establish bounds, either in expectation or in probability, on
% $\Vert f_{H_N,\mathbf{z},\lambda}-f_{\rho} \Vert_{\rho}$ where the norm  $\Vert .\Vert_{\rho}$ is the $L_2^{\rho_{\mathcal{X}}}$-norm and $H_N$ is the RKHS defined in Proposition \ref{prop:RKHS-MLP} associated to a MLP. Let $\mathcal{G}$ a class of Borel probability distributions on $\mathcal{X}\times\mathcal{Y}$ satisfying general assumptions.
% \begin{defn}(Upper rate of convergence)
% \label{defn:upper-rate}
% A sequence $(a_{\ell})_{\ell\geq 1}$ of
% positive numbers is called upper rate of convergence in $L_2^{d\rho_{\mathcal{X}}}$ norm over the model $\mathcal{G}$, for the sequence of estimated solutions $(f_{\mathbf{z},\lambda_{\ell}})_{\ell\geq 1}$ using regularization parameters $(\lambda_{\ell})_{\ell\geq 0}$ if
% \begin{equation*}
% \lim_{\tau\rightarrow +\infty}\lim \sup_{\ell\rightarrow\infty}\sup_{\rho\in \mathcal{G}} \rho^{\ell}\left(\mathbf{z}:\Vert f_{\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2>\tau a_{\ell}\right)=0 \, .
% \end{equation*}
% \end{defn}
% \begin{defn}(Minimax Lower Rate of Convergence)
% A sequence $(v_{\ell})_{\ell\geq 1}$ of
% positive numbers is called minimax lower rate of convergence in $L_2^{d\rho_{\mathcal{X}}}$ norm over the model $\mathcal{G}$ if
% \begin{align*}
%  \lim_{\tau\rightarrow 0^{+}}\lim\inf_{\ell\rightarrow\infty}\inf_{f_{\mathbf{z}}}\sup_{\rho\in\mathcal{G}} \rho^{\ell}\left(\mathbf{z}:\Vert f_{\mathbf{z}}-f_{\rho}\Vert_{\rho}^2>\tau v_{\ell}\right)=1
% \end{align*}
% where the infimum is taken over all measurable learning methods with respect to $\mathcal{G}$.
% \end{defn}
% Such sequences $(v_{\ell})_{\ell\geq 1}$ are called minimax lower rates. Every sequence $( \hat{v}_{\ell})_{\ell\geq 1}$ decreasing at least with the same rate as $(v_{\ell})_{\ell\geq 1}$ is a lower rate for this set of probability measures and at least the same lower rate holds on any larger set of probability measures. When the rate of the sequence of learned functions coincides with the minimax lower rates, it is then said to be optimal in the minimax sense.
%\medbreak
\textbf{Setting.} Let $N\geq 1$, $d\geq 2$ and $(f_i)_{i=1}^N$ be a sequence of N real value functions satisfying assumptions of Proposition \ref{prop:RKHS-MLP}. Denote $(b_m)_{m\geq 0}$ the coefficients in the Taylor series about 0 of $f_N\circ...\circ f_1$. The hypothesis space considered is the Hilbert space $H_N$ associated with the kernel $K_{N}(x,x')=f_N\circ...\circ f_1(\langle x,x'\rangle)$. Note that here we focus specifically on the RKHSs associated to MLPs. Define the integral operator on $L_2^{d{\rho_{\mathcal{X}}}}(\mathcal{X})$ associated as 
$T_{\rho}(f)(y) =  \int_{\mathcal{X}} K_N(x,y)f(x){d\rho_{\mathcal{X}}}(x)$.
% $$\begin{array}{ccccc}
% T_{\rho} & : &  L_2^{d{\rho_{\mathcal{X}}}}(\mathcal{X}) & \to &  L_2^{d{\rho_{\mathcal{X}}}}(\mathcal{X})\\
%  & & f &\to & \int_{\mathcal{X}} K_N(x,.)f(x){d\rho_{\mathcal{X}}}(x)
% \end{array}$$
% Since $k$ is bounded, $T_{\rho}$ is self-adjoint, positive semi-definite and trace-class~\cite{blanchard2008finite}. Let us denote $(\mu_i)_{i\in I} \in \ell_1(I)$ its eigenvalues ranked in a non decreasing order. We shall assume in the following that $I=\mathbb{N}$. When $I$ is finite, results can be found for example in~\cite{caponnetto2007optimal}. 
We work here under general assumptions on the set of probability measures $\rho$ on $\mathcal{X}\times\mathcal{Y}$.

% \textbf{Setting.} Given a dataset $\mathbf{z} = {(x_i,y_i)}_{i=1}^{\ell}$ independently sampled from an unknown distribution $\rho(x, y)$ on $Z:=\mathcal{X}\times \mathcal{Y}$ where $\mathcal{Y}\subset\mathbb{R}$, the goal least-squares regression is to estimate the conditional mean function $f_{\rho}:\mathcal{X}\rightarrow \mathbb{R}$ given by $f_{\rho}(x):= E(Y |X = x)$. Here the hypothesis space considered is the Hilbert space associated with the kernel defined in Proposition \ref{prop:RKHS-MLP}. Note that here we focus specifically on the RKHSs associated to MLPs.
% More precisely, let $N\geq 1$, $d\geq 2$ and $(f_i)_{i=1}^N$ be a sequence of N real value functions such that $f_N\circ...\circ f_1$ admits a Taylor decomposition on $[-1,1]$ with non negative coefficients $(b_m)_{m\geq 0}$:
% \begin{align*}
%  f_N\circ...\circ f_1(x):=\sum_{m\geq 0} b_m x^m
% \end{align*}
% and let $H_N$ be the RKHS associated with the kernel $K_N$ defined on $S^{d-1}$ by:
% \begin{align*}
% K_{N}(x,x'):=f_N\circ...\circ f_1(\langle x,x'\rangle_{\mathbb{R}^d}) ; .
% \end{align*}
\medbreak
\begin{assump}\textbf{ [Probability measures on $\mathcal{X} \times \mathcal{Y}$].} Let $\mathcal{P}$ a set of probability measures on $\mathcal{X}$. Furthermore, let $B, B_{\infty}, L, \sigma> 0$ be some constants and $0< \beta \leq 2$ a parameter. Then we denote by $\mathcal{F}_{B, B_{\infty}, L, \sigma,\beta}(\mathcal{P})$ the set of all probability measures $\rho$ on $\mathcal{X} \times\mathcal{Y}$ with the following properties:
\begin{itemize}
    \item $\rho_{\mathcal{X}}\in\mathcal{P}$, $\int_{\mathcal{X}\times\mathcal{Y}}y^2d\rho(x,y) < \infty$, $\Vert f_{\rho}\Vert_{L_{\infty}^{d\rho_{\mathcal{X}}}}^2 \leq  B_{\infty}$
    \item There exists $g\in L_2^{d\rho_{\mathcal{X}}}(\mathcal{X})$ such that $f_\rho=T_{\rho}^{\beta/2}g$ and $\Vert g\Vert_{\rho}^2\leq B$
    \item there exist $\sigma>0$ and $L>0$ such that
 $\int_{\mathcal{Y}} |y-f_{\rho}(x)|^m d\rho(y|x)\leq \frac{1}{2}m!L^{m-2}$
\end{itemize}
\end{assump}
A sufficient condition  for the last assumption is that $\rho$ is concentrated on $\mathcal{X} \times [-M,M]$ for some constant $M>0$. 
\medbreak

For $\omega\geq 1$, we denote by $\mathcal{W}_{\omega}$ the set of all probability measures $\nu$ on $S^{d-1}$ which satisfying $\frac{d\nu}{d\sigma_{d-1}}< \omega$.
Furthermore, we introduce for a constant $\omega \geq 1 > h > 0$, $\mathcal{W}_{\omega,h}\subset\mathcal{W}_{\omega}$ the set of probability measures $\nu$ on $S^{d-1}$ which additionally satisfy 
$\frac{d\nu}{d\sigma_{d-1}}> h$.
In the following we denote $\mathcal{G}_{\omega, \beta}:=\mathcal{F}_{H_N,B, B_{\infty}, L, \sigma,\beta}(\mathcal{W}_{\omega})$
and $\mathcal{G}_{\omega,h,\beta}:=\mathcal{F}_{H_N,B, B_{\infty}, L, \sigma,\beta}(\mathcal{W}_{\omega,h})$. 

% \begin{rmq}
% It is worth noting that we do not make any assumption on the set of distributions related to the eigenvalue decay. Indeed, the spectral analysis of the MLPs obtained in section \ref{sec:MLP-paper}, allows us to define a non-trivial set of distributions adapted for these specific kernels. This should be contrasted with the assumptions considered in section \ref{sec:RLS}.
% \end{rmq}

\subsection{Geometric Case}
We first consider the case of multi-layer perceptrons such that the composition of nonlinear functions involved in the network admits a Taylor decomposition with coefficients decreasing almost geometrically. In the following theorem, we provides our result about generalization error analysis for the empirical risk minimizer. See proof in  Appendix~\ref{proof:rls-geo}.

\begin{thm}
\label{thm:rls-geo}
Let us assume that there exists $1>r>0$, $0<c_1$ some constants such that the sequence $(b_m)_{m\geq 0}$ satisfies for all $m\geq 0$:
\begin{align}
\label{eq:assump_geometric}
 b_m \leq c_1 r^m
\end{align}
Let also $w\geq 1$ and $0<\beta\leq 2$.
Then there exists $A,C>0$ some constants independent of $\beta$ (see Appendix \ref{sec:RLS} for their definitions) such that for any $\rho\in \mathcal{G}_{\omega, \beta}$ and $\tau\geq 1$ we have:
\begin{itemize}
\item  If $\beta> 1$, then for $\lambda_{\ell}=\frac{1}{\ell^{1/\beta}}$ and
$\ell\geq \text{max}\left(e^{\beta},\left(\frac{A}{\beta^{d-1}}\right)^{\frac{\beta}{\beta-1}}\tau^{\frac{2\beta}{\beta-1}} \log(\ell)^{\frac{d-1\beta}{\beta-1}}\right)$, with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
    \begin{align*}
\Vert f_{H_N,\mathbf{z},\lambda}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{d-1}}{\ell}
    \end{align*}
    \item  If $\beta = 1$, then for $\lambda_{\ell}=\frac{\log(\ell)^{\mu}}{\ell}$, $\mu>d-1>0$ and  $\ell\geq \text{max}\left(\exp\left((A\tau)^{\frac{1}{\mu-d-1}}\right),e^{1}\log(\ell)^{\mu}\right)$, with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
    \begin{align*}
    \Vert f_{H_N,\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{\mu}}{\ell^{\beta}}
    \end{align*}
    \item  If $\beta < 1$, then for $\lambda_\ell=\frac{\log(\ell)^{\frac{d-1}{\beta}}}{\ell}$ and $\ell\geq \text{max}\left(\exp\left((A\tau)^{\frac{\beta}{d-1(1-\beta)}}\right),e^{1}\log(\ell)^{\frac{d-1}{\beta}}\right)$, with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
    \begin{align*}
    \Vert f_{H_N,\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{d-1}}{\ell^{\beta}}
    \end{align*}
\end{itemize}
\end{thm}
\textbf{Example.} As we have restricted the input space to be the unit sphere, we can consider the case where $\sigma_1=...=\sigma_N=\tanh$. Indeed recall that $\tanh$ admits a Taylor decomposition on $[-1,1]$ with coefficients satisfying assumption (\ref{eq:assump_geometric}) and that $\tanh([-1,1])\subset [-1,1]$. Therefore the functions $(f_i)_{i=1}^N$ associated, even if we may have to renormalize $(f_i)_{i=1}^N$ by their largest values on $[-1,1]$, admit a Taylor decomposition on $[-1,1]$ and the coefficients $(b_m)_{m\geq 0}$ in the Taylor series about 0 of $f_N\circ...\circ f_1$ satisfy assumption (\ref{eq:assump_geometric}). Thus Theorem \ref{thm:rls-geo} can be applied. This case corresponds to the nonlinear function used in \textit{LeNet5}. Note also that the sigmoid function defined as $\sigma:=(1+\exp(-x))^{-1}$ is just a rescaled and shifted version of $\tanh$ which therefore can be used here.



\medbreak
Moreover the following theorem investigates the optimality of our learning rates. See proof in Appendix \ref{proof:rls-geo}.
\begin{thm}
\label{thm:lower-geo}
Let us assume that there exists $0<c_2<c_1$ such that for all $m\geq 0$:
\begin{align*}
  c_2 r^m \leq b_m \leq c_1 r^m
\end{align*}
Then for any $\omega\geq 1 > h >0$ such that $\mathcal{W}_{\omega,h}$ is not empty it holds 
\begin{align*}
 \lim_{\tau\rightarrow 0^{+}}\lim\inf_{\ell\rightarrow\infty}\inf_{f_{\mathbf{z}}}\sup_{\rho\in\mathcal{G}_{\omega,h,\beta}} \rho^{\ell}\left(\mathbf{z}:\Vert f_{\mathbf{z}}-f_{\rho}\Vert_{\rho}^2>\tau b_{\ell}\right)=1
\end{align*}
where $b_{\ell}=\frac{\log(\ell)^{d-1}}{\ell}$. The infimum is taken over all measurable learning methods with respect to $\mathcal{G}_{\omega,h,\beta}$.
\end{thm}
Therefore for such networks, when $\beta>1$ the learning rates of the regularized least-squares estimator stated in theorem  \ref{thm:rls-geo} coincide with the minimax lower
rates from theorem \ref{thm:lower-geo} and therefore are optimal in the minimax sense. 


% \begin{rmq}
% Instead of the regularized least-squares algorithm, let us consider for any sequence $(m_i)_{i=1}^N\in\mathbb{N}_{*}^N$ the following estimator:
% \begin{align*}
%   \widehat{f}_{(m_i)_{i=1}^N}\in \argminB_{f\in \mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N,(m_i)_{i=1}^N}} \left\{ \frac{1}{\ell}\sum_{i=1}^{\ell}( f(x_i)-y_i)^2 \right\} 
% \end{align*}
% Then the results of theorems \ref{thm:rls-geo} and \ref{thm:lower-geo} suggests that for any choice of $(m_i)_{i=1}^N$, the generalization performance of such estimator cannot have better asymptotic rates than the one obtained by regularized least square algorithm in this setting. Indeed, on the set of distributions introduced, our estimator matches the minmax rates. Therefore any other estimator cannot do better in the minmax sense.   
% \end{rmq}

% \textbf{Example.} Consider the case where $f_1$ is the inverse polynomial function $f_1(x)=1/(2-x)$, while
% the other layers are polynomial functions. Then, for all $k\geq 2$, $f_k\circ ...\circ f_1$ satisfy also Assumption~\ref{eq:assump_geometric}. Thus  Theorem~\ref{thm:rls-geo} can be applied. On the one hand, the convergence rate remains the same asymptotically as the network gets deeper. On the other hand, the space in which the target function is assumed to live is allowed to grow as the network gets deeper. \todo{a modifier}

% \textbf{Example.} Consider the case where $f_1$ is the inverse polynomial function $f_1(x)=1/(2-x)$, while
% the other layers are polynomial functions. Then, for all $k\geq 2$, $f_k\circ ...\circ f_1$ satisfy also assumption~(\ref{eq:assump_geometric}) and the result of Theorem \ref{thm:rls-geo} hold.

\subsection{Super-geometric Case}
Another regime of interest is the one where the composition of nonlinear functions involved in the network admits a Taylor decomposition with coefficients decreasing super-geometrically. As in the geometric case, the goal is to obtain a control the of the eigenvalues associated with the integral operator $T_{K_N}$. See Appendix~\ref{proof:rls-super-geo}.
\begin{thm}
\label{thm:super-geo}
Assume that there exists $1 > \delta>0$ such that
\begin{align}
\label{eq:b_n-final}
\left|\frac{b_{m}}{b_{m-1}}\right|\in O(m^{-\delta}) \; .
\end{align}
Let also $0<\beta\leq 2$ and $\omega>0$.
Then there exist a constant $C$ independent of $\beta$ such that
for any $\rho\in \mathcal{G}_{\omega,\beta}$ and $\tau\geq 1$ we have:
\begin{itemize}
\item  If $\beta> 1$, then there exists $\ell_{\tau}>0$ such that for all $\ell\geq \ell_{\tau}$ and $\lambda_{\ell}=\frac{1}{\ell^{1/\beta}}$, with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
    \begin{align*}
    \Vert f_{H_N,\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{d-1}}{[\log(\log(\ell))]^{d-1}\ell}
    \end{align*}
    \item  If $\beta = 1$, then there exists $\ell_{\tau}>0$ such that for all $\ell\geq \ell_{\tau}$, $\lambda_{\ell}=\frac{\log(\ell)^{\mu}}{[\log(\log(\ell))]^{\mu}\ell}$ and $\mu\geq d-1$, with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
    \begin{align*}
    \Vert f_{H_N,\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{\mu}}{[\log(\log(\ell))]^{\mu}\ell}
    \end{align*}
    \item If $\beta < 1$, then there exists $\ell_{\tau}>0$ such that for all $\ell\geq \ell_{\tau}$ and $\lambda_{\ell}=\frac{\log(\ell)^{\frac{d-1}{\beta}}}{[\log(\log(\ell))]^{\frac{d-1}{\beta}}\ell}$ with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
    \begin{align*}
    \Vert f_{H_N,\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{d-1}}{[\log(\log(\ell))]^{d-1}\ell^{\beta}}
    \end{align*}
\end{itemize}
\end{thm}
As expected, in that regime, we obtain faster rates compared to the geometric case as the eigenvalues decrease faster. 
%Moreover as in the geometric case, we can deduce asymptotic rates. See Appendix Corollary~\ref{coro:exp-rate}.
\medbreak

% \textbf{Example.} Consider the case where $f_1$ is the exponential function, while the other layers are polynomial functions. Then $f_N\circ ...\circ f_1$ satisfies also assumption~(\ref{eq:b_n-final}). Then Thoerem~\ref{thm:super-geo} can be applied.
\medbreak
% \textbf{Example 1.} Let consider the case where $N=2$ and $f_2(t)=f_1(t)=\exp(t)$. For such networks, we have an explicit expression of the sequence $(b_m)_{m\geq 0}$ (See Appendix~\ref{proof:example}) with $b_0=e^1$
% \begin{align*}
% b_{m+1}=\frac{1}{m+1}\sum_{k=0}^m. \frac{b_{k}}{(m-k)!}
% \end{align*}
% We can compute the coefficients $(b_m)_{m\geq 0}$ thanks to this recurrence relation. In Figure \ref{fig:decay_bn}, we plot the rate of convergence of $(|b_m/b_{m-1}|)_{m\geq 1}$ (in blue) and compare it to $(1/m^{\delta})_{m\geq 1}$ where $\delta=1/3$ (in green) and $\delta = 1/5$ (in red). For such networks, assumption~(\ref{eq:b_n-final}) hold for $\delta=1/5<1/2$ and therefore theorem \ref{thm:super-geo} hold.


% \textbf{Example 2.} Consider the case where $f_1$ is the exponential function, while the other layers are polynomial functions. Then $f_N\circ ...\circ f_1$ satisfies also assumption~(\ref{eq:b_n-final}). Then Theorem~\ref{thm:super-geo} can be applied. \todo{A modifier}

\textbf{Discussion.} The rates obtained in Theorems \ref{thm:rls-geo} and \ref{thm:super-geo} have a logarithmic term which depends exponentially in the dimension. However asymptotically, compared to the polynomial rates as the one obtained in \cite{bach2017breaking,schmidthieber2019nonparametric}, our rates are clearly faster. Note also that in the geometric case, the rates obtained for RLS are optimal in the minmax sense and therefore no other algorithm can have better rates in this setting. In addition the rates obtained highlight another important aspect of the behavior of MLPs. Indeed the learning rates obtained in both regimes do not depend on the number of parameters considered in the network which may be much bigger than the input dimension. Here we show that even on the largest possible function space generated by multi-layer perceptrons, the algorithm is still able to learn. In the next section, we investigate the effect of depth on the learning rates obtained.

\subsection{Effects of the depth for MLPs}
In this section, we investigate the effect of the depth for these specific networks. More precisely, we show in the next proposition that as soon as the network reach the geometric regime, adding layers may not change the actual regime. See Appendix \ref{proof:effect_depth_geo} for the proof.
\begin{prop}
\label{prop:effect_depth_geo}
Let $N\geq 1$, $d\geq 2$ and $(f_i)_{i=1}^N$ be a sequence of N real value functions satisfying assumptions of Proposition \ref{prop:RKHS-MLP} and denote $(b_m)_{m\geq 0}$ the coefficients in the Taylor series about 0 of $f_N\circ...\circ f_1$. Let also $q\geq 1$ and $f_{N+1},...f_{N+q}$ polynomial functions of arbitrary degree with non negative coefficients. Assume that there exists $1>r>0$, $0<c_1$ some constants such that the sequence $(b_m)_{m\geq 0}$ satisfies for all $m\geq 0$, $b_m \leq c_1 r^m$ then $f_{N+q}\circ...\circ f_1(x)$ admits a Taylor decomposition about 0 with non negative coefficients and by denoting $(a_m)_{m\geq 0}$ those coefficients, we obtain that there exists $1>r'>r>0$ and $0<c_1'$ such that for all $m\geq 0$, $a_m \leq c_1' r'^m$.
\end{prop}
Adding layer to the network when it has already reached a geometric regime does not change the regime and therefore the results of Theorem \ref{thm:rls-geo} can be applied. %Therefore as soon as the network reaches the geometric regime, adding layers to the network does not affect the learning rate of convergence. 
However adding layers to the network allows the function space of target function to grow.
% Indeed observe that the eigenvalue decay decreases slower when the number of layers increases. Therefore, the RKHS obtained become larger. The eigenvalue decay gives a concrete notion of the complexity of the function space considered. Given an eigensystem  $(\mu_m)_{m\geq 0}$ and $(e_m)_{m\geq 0}$ of positive eigenvalues and eigenfunctions respectively of the integral operator $T_{K_N}$, associated with the Kernel $K_N$, defined on $L_2(S^{d-1})$, the RKHS $H_N$ associated is defined as:
% $$ H_N=\left\{f\in L_2(\mathcal{I})\text{:\quad} f = \sum_{m\geq 0} a_m e_m \text{\quad with\quad } \left( \frac{a_m}{\sqrt{\mu_m}} \right)\in\ell_2\right\}$$
% endowed with the following inner product:
% \begin{align*}
% \langle f,g \rangle=\sum_{m\geq 0} \frac{a_m b_m}{\mu_m}
% \end{align*}
% From this definition, we see immediately that as the eigenvalues of the integral operator decreases slower, the RKHS becomes larger. 
Therefore adding layers allows the function space of the target function to grow, while the learning rates remain the same.

\begin{rmq}
Similar results hold also in the super-geometric case. See Appendix \ref{proof:effect_depth_geo} for the proof.
\end{rmq}





==> sections/section5.tex <==
\section{Experiments}
% \begin{figure}[ht]
%   \centering
%   \subfigure[Accuracy vs Depth.\label{fig:accuracy}]{\includegraphics[scale=0.3]{mlp/figures/MLP-depth.pdf}}\quad \quad
%   \subfigure[Decay vs. Depth.\label{fig:spectrum-512}]{\includegraphics[scale=0.3]{mlp/figures/MLP-spect-512.pdf}}
% \end{figure}

\begin{wrapfigure}{r}{0.3\textwidth}\vspace*{-4.5ex}
        \includegraphics[width=0.7\linewidth]{mlp/figures/MLP-depth.pdf}
    \caption{Accuracy vs Depth.\label{fig:accuracy}}
\end{wrapfigure}


First, we investigate the relations between network depth and prediction accuracy on MNIST~\footnote{ http://yann.lecun.com/exdb/mnist/}. We construct fully connected neural networks from 1 to 3 layers. We model large-width networks by setting number of weights per layer to be constant and sufficiently large. The number of weights can be either 128, 256 or 512 at each layer. Moreover we normalize the input data so that the input datapoints lie on a subspace of the unit sphere. 
We see in Figure~\ref{fig:accuracy} that, in each situation, as the number of layers increases, the prediction accuracy gets better. This means that the networks get better at approximating the target function as the network depth increases.
\medbreak


\begin{wrapfigure}{r}{0.3\textwidth}\vspace*{-4.5ex}
        \includegraphics[width=0.7\linewidth]{mlp/figures/MLP-spect-512.pdf}
    \caption{Decay vs. Depth.\label{fig:spectrum-512}}
\end{wrapfigure}


Second, we investigate the relation between the network depth and the eigenvalue decay, in the super-geometric setting. We proceed similarly, including regarding input normalization. The first nonlinear activation is the exponential function, while the others are quadratic activation functions for which assumption (\ref{eq:b_n-final}) is indeed satisfied. We obtain the spectral decomposition of the kernel associated with the network by computing the eigenvalues associated with the last hidden layer as a feature map of the kernel. Figure~\ref{fig:spectrum-512} shows the result after 15 epochs and for a number of weights per layer equal to 512. See Appendix~\ref{sec:experiments} for 128 and 256. We observe that, as the number of layers increases, the eigenvalue decay is slower, which means that the function space generated by such structures is larger. Therefore, as the number of layers increases, the network gets better at approximating the target function in the asymptotic regime. 




==> sections/section6.tex <==
\section{Related works}
\todo{Rajouter equation la plus rapproche}
An extensive survey of the abundant literature on theoretical analysis of deep networks is beyond the scope of this paper. We focus here on relevant recent works to contrast our work with.

\paragraph{Eigenvalue decay regimes.}
Recent works such as~\cite{blanchard2018optimal,fischer2017sobolev,caponnetto2007optimal} establish convergence rates for regularized least-squares in reproducing kernel Hilbert spaces; see~\cite{steinwart2008support} for an earlier survey of this literature.
In these papers and previous ones referenced therein, the analysis focuses on the case of polynomial eigenvalue decay of the the integral operator, while we extend the analysis to geometric and super-geometric decays. 

Moreover, thanks to the spectral analysis of the RKHS-s introduced in Proposition \ref{prop:RKHS-MLP}, we exhibit non-trivial sets of distributions for which learning rates for these specific RKHSs are indeed obtained. The tight control of the eigenspectrum decay of the integral operator associated to these specific kernels is key here. Indeed it allows to avoid all the assumptions on the set of distributions related to the eigenvalue decay to obtain learning rates for these specific kernels. Note that in some cases, these rates are optimal in the minmax sense. This contrasts for instance \cite{caponnetto2007optimal}, in which learning rates are obtained on a hypothetical set of distributions which, may not capture the regime considered here, and depends on the RKHS itself. There the authors considered (a subset of) the set of all the distributions for which the eigenvalue decay of the integral operator associated to the kernel is polynomial. Therefore the set of distributions obtained depends on the RKHS considered and may be not adapted. Recall that in our cases, we show that the eigenvalue decay could be geometric or even super-geometric. Finally  the set of distributions introduced in section \ref{sec:RLS-MLP} is completely independent of the choice of the RKHS (except for the source condition which can just be fixed). Therefore we are able to compare the learning rates obtained for the different RKHSs defined in proposition \ref{prop:RKHS-MLP} on this set of distributions. Particularly, we can compare the learning rates obtained when the number of layers differs.

In \cite{bach2017breaking}, the author studies also single-hidden layer neural networks with input data on the sphere. An RKHS is built allowing to get an explicit control of the eigenvalue decay of the integral operator. The eigenvalue considered in~\cite{bach2017breaking} is $m^{-1-1/d-2s/d}$, that is a polynomial eigenvalue decay. Our work considers multiple hidden layer neural networks and cover a wider range of eigenvalue decay regimes. Moreover, the author also exhibited an exponential dependence with respect to the dimension. When making structural assumptions on the function space in which the target function lives, the author manages to make the scaling in d disappear. Indeed, thanks to these assumptions, the bias of the model is not longer exponential in the dimension. In our setting, we obtain optimal minmax rates with mild assumptions on the regression functions.

\paragraph{Embedding an MLP in a function space.}
In \cite{zhang2016l1}, the authors provide a control of the generalization error for network functions thanks to their RKHS norms. Note that we have obtained a similar control. But these bounds do not consider the approximation bias of the class of functions considered which is the major issue in high dimension. Moreover these generalization bounds may blow up as the number of parameters increases while the learning rates obtained in section 5 do not depend on the number of parameters. Note also that the kernels defined in Proposition \ref{prop:RKHS-MLP} generalize the kernel studied in \cite{zhang2016l1}, which is a special case of ours when considering that all the $(f_i)_{i=1}^n$ are the same and equal to $f_i(x)=1/ (2 – x)$. Moreover the RKHS norm of the neural network (and thus the bounds) obtained in \cite{zhang2016l1} is less tight the one presented in Section \ref{section:MLP-def} as our kernel is adaptive the network considered.


The papers~\cite{savarese:etal:2019,ongie:etal:2020} focus on the realizable case, \textit{i.e.} when the target function $f_{\rho}$ lives in the function space used to learn, and characterize the norm required to realize such functions using a network, with a single-hidden layer, with an infinite width, and a ReLU activation.
Their viewpoint is diametrically opposed to ours, the proof techniques as well, since we do not assume that the target function is realizable, nor do we assume that the layers have infinite width, and consider deep networks instead of a single-hidden layer ones. The two viewpoints can therefore be seen as complementary. 

The paper~\cite{suzuki2018fast} presents generalization bounds for multi-layer perceptrons. While the paper may seem related to ours on a superficial level, the developments and resulting bounds in each paper differ substantially. We highlight below these differences. First, in this paper as well, the target function $f_{\rho}$ is assumed to live in the function space used to learn. In our setting this assumption corresponds to the case where $\beta=1$.
The goal there is to obtain bounds for the learning method $\widehat{f}_{(m_i)_{i=1}^N}$ with ${(m_i)_{i=1}^N}\in\mathbb{N}_{*}^N$ fixed defined as
\begin{align*}
   \widehat{f}_{(m_i)_{i=1}^N}\in \argminB_{f\in \mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N,(m_i)_{i=1}^N}} \left\{ \frac{1}{\ell}\sum_{i=1}^{\ell}( f(x_i)-y_i)^2 \right\} \; .
\end{align*}

Assuming that the number of weights per layer is of the same order as the degrees-of-freedom up to a log term, the number of samples $\ell$ is large enough and the regularization parameter  small enough,
the resulting high probability bound has the form 
\begin{align}
    \left\Vert \widehat{f}_{(m_i)_{i=1}^N} - f_{\rho}\right\Vert^2_{\rho}\in\mathcal{O}
    \left(\frac{\log(\ell)\text{df}(\lambda)^2}{\ell}
    \, +\lambda  
    \right) \; ,
\end{align}
where $$\text{df}(\lambda):=\text{Tr}\left((C_{\rho}+\lambda)^{-1}C_{\rho}\right)=\sum_{i\in I}\frac{\mu_i}{\mu_i+\lambda}$$
and $(\mu_i)_{i\geq 0}$ are the eigenvalues associated to the integral operator. A major difference of our work is the explicit control of the degrees-of-freedom $\text{df}(\lambda)$ through the eigenvalue decay of the integral operator. However the control of the degrees-of-freedom within the framework of \cite{suzuki2018fast} is unclear and deserves further investigation. In \cite{suzuki2018fast}, the author does not control the eigenspectrum decay of the integral operator considered, while we do for the integral operator we consider. Furthermore in our case, a similar bias-variance trade-off appears. Yet, when applying the above bound in each of two regimes we considered, the resulting bounds are less tight than ours in both regimes.

\paragraph{Effect of depth.}
In \cite{schmidthieber2019nonparametric}, the author studies the effect of the depth of the network. Note that the L log2 n-factor in \cite{schmidthieber2019nonparametric} rates where L is the number of hidden layer is, as he put it, likely an artifact of the proof, which does not appear in the lower bound. The dependence in the number of layers there concerns the estimator used, not the rates. \todo{a ameliorer}

==> sections/section7.tex <==
\section{Conclusion.}
We studied the complexity of the function space generated by multi-layer perceptrons in relation to the network depth. Investigating the effect of the number of weights per layer is an interesting venue for future work.

==> sections/suppmat_aistats.tex <==
% \documentclass[twoside]{article}

% \usepackage{aistats2021}
% % If your paper is accepted, change the options for the package
% % aistats2021 as follows:
% %
% %\usepackage[accepted]{aistats2021}
% %
% % This option will print headings for the title of your paper and
% % headings for the authors names, plus a copyright note at the end of
% % the first column of the first page.

% % If you set papersize explicitly, activate the following three lines:
% %\special{papersize = 8.5in, 11in}
% %\setlength{\pdfpageheight}{11in}
% %\setlength{\pdfpagewidth}{8.5in}

% % If you use natbib package, activate the following three lines:
% %\usepackage[round]{natbib}
% %\renewcommand{\bibname}{References}
% %\renewcommand{\bibsection}{\subsubsection*{\bibname}}

% % If you use BibTeX in apalike style, activate the following line:
% %\bibliographystyle{apalike}

% \begin{document}

% % If your paper is accepted and the title of your paper is very long,
% % the style will print as headings an error message. Use the following
% % command to supply a shorter title of your paper so that it can be
% % used as headings.
% %
% %\runningtitle{I use this title instead because the last one was very long}

% % If your paper is accepted and the number of authors is large, the
% % style will print as headings an error message. Use the following
% % command to supply a shorter version of the authors names so that
% % they can be used as headings (for example, use only the surnames)
% %
% %\runningauthor{Surname 1, Surname 2, Surname 3, ...., Surname n}

% % Supplementary material: To improve readability, you must use a single-column format for the supplementary material.
% \onecolumn
% \aistatstitle{Instructions for Paper Submissions to AISTATS 2021: \\
% Supplementary Materials}

% \section{FORMATTING INSTRUCTIONS}

% To prepare a supplementary pdf file, we ask the authors to use \texttt{aistats2021.sty} as a style file and to follow the same formatting instructions as in the main paper.
% The only difference is that the supplementary material must be in a \emph{single-column} format.
% You can use \texttt{supplement.tex} in our starter pack as a starting point, or append the supplementary content to the main paper and split the final PDF into two separate files.

% Note that reviewers are under no obligation to examine your supplementary material.

% \section{MISSING PROOFS}

% The supplementary materials may contain detailed proofs of the results that are missing in the main paper.

% \subsection{Proof of Lemma 3}

% \textit{In this section, we present the detailed proof of Lemma 3 and then [ ... ]}

% \section{ADDITIONAL EXPERIMENTS}

% If you have additional experimental results, you may include them in the supplementary materials.

% \subsection{The Effect of Regularization Parameter}

% \textit{Our algorithm depends on the regularization parameter $\lambda$. Figure 1 below illustrates the effect of this parameter on the performance of our algorithm. As we can see, [ ... ]}

% \vfill

% \end{document}

\onecolumn
\section*{Supplementary material}
\paragraph{Overview.}
We provide all the proofs of the mathematical statements in the main text. The statistical bounds we have obtained can be used in at least two contexts which we consider in detail. 

First, they can be used to describe the statistical performance of a regularized least-squares estimator when this estimator can be computed exactly. 
This can be potentially applied to the recent kernel-based deep networks developed in~\cite{shankar2020neural} and to kernel-based methods with kernels on spheres~\cite{steinwart2008support}.

Second, they can be used to obtain an optimistic estimate of the statistical performance of a deep network estimator via its Hilbertian envelope estimator (\ref{eq:rls-obj}), when the deep network estimator cannot be computed exactly in practice. It is worthwhile to underscore, that, as of today, no theoretical framework is able to tackle all aspects of deep network analysis, function approximation, numerical optimization, and statistical prediction. Here we trade numerical optimization (our results assume perfect optimization) for function approximation (our results apply to both the realizable and the non-realizable cases) and statistical prediction (our results match minimax rates). 

\paragraph{Outline.} 
In Sec.~\ref{sec:RLS}
%~\ref{sec:upper-lower},
we prove a statistical bound on the performance of a regularized least-squares estimator under the assumption of geometric eigenvalue decay. This corresponds to the first context described above. In Sec.~\ref{def:cc-universal}, we build a reproducing kernel Hilbert space (RKHS) that contains the function space generated by multi-layer perceptrons and state sufficient conditions for universal consistency. We also give a control of the RKHS norm of multi-layer perceptrons and provides a first generalization bound for MLPs. In Sec.~\ref{sec:sp-mlp} we provide a control on the eigenvalue decay of the integral operators associated to this kernel in two regimes: geometric and super-geometric. In Sec.~\ref{sec:RLS-geo-exp}, we establish high-probability bounds related to the performance of a deep network estimator via its Hilbertian envelope estimator in these two regimes. This corresponds to the second context described above. We also discuss the effect of the depth on the convergence rates obtained. In Sec.~\ref{sec:background}-\ref{sec:useful-thm}-\ref{sec:tech-lem}, we collect useful technical results and basic notions. In Sec.~\ref{sec:experiments}, we give some illustrations of the eigenvalue decay regimes considered in the paper. 
%Finally, in Section~\ref{sec:discussion}, we provide more %detailed discussions of related works.

\input{mlp/sections/section_RLS_gene}


% \section{General Convergence Rates}
% \label{sec:upper-lower}
% Let us first recall the general assumptions on the set of probability measures $\rho$ on $\mathcal{X}\times\mathcal{Y}$ for the general setting.\\

% \textbf{Assumption [Probability measures on $\mathcal{X}$].}
% Let $H$ be an infinite dimensional separable reproducing kernel Hilbert space (RKHS) on $\mathcal{X}$ with respect to a bounded and measurable kernel $k$. Furthermore, let $C,\gamma>0$ be some constants and $\alpha>0$ be a parameter. By $\mathcal{P}_{H,C,\gamma,\alpha}$ we denote the set of all probability measures $\nu$ on $\mathcal{X}$ with the following.
% \begin{itemize}
%     \item The measurable space $(\mathcal{X}, \mathcal{B})$ is $\nu$-complete.
%     \item  The eigenvalues fulfill the following upper bound $\mu_i \leq C_0 e^{-\gamma i^{1/\alpha}}$ for all $i \in I$.
% \end{itemize}
% Let us introduce for a constant $c > 0$ and a parameter $q\geq \gamma>0$ the subset $\mathcal{P}_{H,C_0,\gamma,\alpha,c,q}\subset\mathcal{P}_{H,C_0,\gamma,\alpha}$ of probability measures $\mu$ on $\mathcal{X}$ which additionally have the following property.
% \begin{itemize}
%     \item The eigenvalues fulfill the following lower bound $\mu_i \geq c e^{-q i^{1/\alpha}}$ for all $i \in I$.
% \end{itemize}
% We shall denote $\mathcal{P}_{H,\alpha}:= \mathcal{P}_{H,C_0,\gamma,\alpha}$ and  $\mathcal{P}_{H,\alpha,q}:=\mathcal{P}_{H,C_0,\gamma,\alpha,c,q}$.\\

% \textbf{Assumption [Probability measures on $\mathcal{X} \times \mathcal{Y}$].} Let $H$ be a separable RKHS on $\mathcal{X}$ with respect to a bounded and measurable kernel $k$ and $\mathcal{P}$ a set of probability measures on $\mathcal{X}$. Furthermore, let $B, B_{\infty}, L, \sigma> 0$ be some constants and $0< \beta \leq 2$ a parameter. Then we denote by $\mathcal{F}_{H,B, B_{\infty}, L, \sigma,\beta}(\mathcal{P})$ the set of all probability measures $\rho$ on $\mathcal{X}\times\mathcal{Y}$ with the following properties:
% \begin{itemize}
%     \item $\rho_{\mathcal{X}}\in\mathcal{P}$, $\int_{\mathcal{X}\times\mathcal{Y}}y^2d\rho(x,y) < \infty$, $\Vert f_{\rho}\Vert_{L_{\infty}^{d\rho_{\mathcal{X}}}}^2 \leq  B_{\infty}$
%     \item There exist $g\in L_2^{d\rho_{\mathcal{X}}}(\mathcal{X})$ such that $f_\rho=T_{\rho}^{\beta/2}g$ and $\Vert g\Vert_{\rho}^2\leq B$
%     \item there exist $\sigma>0$ and $L>0$ such that
%  $\int_{\mathcal{Y}} |y-f_{\rho}(x)|^m d\rho(y|x)\leq \frac{1}{2}m!L^{m-2}$
% \end{itemize}
% A sufficient condition  for the last assumption is that $\rho$ is concentrated on $\mathcal{X} \times [-M,M]$ for some constant $M>0$. 
% We shall denote $\mathcal{F}_{H,\alpha,\beta}:=\mathcal{F}_{H,B, B_{\infty}, L, \sigma,\beta}(\mathcal{P}_{H,\alpha})$
% and $\mathcal{F}_{H,\alpha,q,\beta}:=\mathcal{F}_{H,B, B_{\infty}, L, \sigma,\beta}(\mathcal{P}_{H,\alpha,q})$.

% \subsection{Proof of Theorem \ref{thm:upper-rate}}
% \label{proof:upper-rate}
% \begin{proof}
% To show the result let us first define the degrees-of-freedom $\text{df}(\lambda):=\text{Tr}\left((C_{\rho}+\lambda)^{-1}C_{\rho}\right)=\sum_{i\in I}\frac{\mu_i}{\mu_i+\lambda}$.
% Moreover for $\lambda > 0$ the minimization problem
% \begin{align*}
% \inf_{f\in H}\left\{ R(f)+\lambda \Vert f\Vert_H^2 \right\}
% \end{align*}
% has a unique solution defined as $f_{H,\rho,\lambda}=(C_{\rho}+\lambda)^{-1}T_{\rho} f_{\rho}\in H$.
% To obtain an upper rate of convergence we first control the degrees-of-freedom with respect to the regularization parameter.
% \begin{lemma}
% \label{lem:effective-dim-geo}
% Let $\alpha >0$. If there exist $C,\gamma>0$ such that $\mu_i \leq C_0 e^{-\gamma i^{1/\alpha}}$ for all $i \in I$. Then  all $0<\lambda\leq e^{-1}$ we have:
% \begin{align*}
% \textsl{df}(\lambda)&\leq Q \log(\lambda^{-1})^{\alpha}\\
% \text{where \quad} Q&=\gamma^{-\alpha} \left[1+C_0\int_{1}^{\infty} \frac{(\log(u)+1)^{\alpha-1}}{C_0 u+u^2}du\right]
% \end{align*}
% \end{lemma}

% \begin{proof}
% By definition of $\textsl{df}(\lambda)$ we have
% \begin{align*}
% \textsl{df}(\lambda)\leq \sum_{m\geq 1}\frac{C_0}{C_0+\lambda e^{\gamma m^{\frac{1}{\alpha}}}} \; .
% \end{align*}
% Moreover as the $x\rightarrow \frac{C_0}{C_0+\lambda e^{\gamma x^{\frac{1}{\alpha}}}}$ is positive and decreasing, therefore we have
% \begin{align*}
% \textsl{df}(\lambda)\leq \int_{0}^{+\infty}\frac{C_0}{C_0+\lambda e^{\gamma x^{\frac{1}{\alpha}}}} dx \; .
% \end{align*}
% Let us consider the following substitution
% \begin{align*}
% u=\lambda e^{\gamma x^\frac{1}{\alpha}} \; .
% \end{align*}
% Therefore we have
% \begin{align*}
% \textsl{df}(\lambda)&\leq \int_{\lambda}^{\infty}C_0\gamma^{-\alpha}\alpha\frac{(\log(u\lambda^{-1}))^{\alpha-1}}{C_0 u+u^2}du\\
% &\leq  \int_{\lambda}^{1}C_0\gamma^{-\alpha}\alpha\frac{(\log(u\lambda^{-1}))^{\alpha-1}}{C_0 u+u^2}du+ \int_{1}^{\infty}C_0\gamma^{-\alpha}\alpha\frac{(\log(u\lambda^{-1}))^{\alpha-1}}{C_0 u+u^2}du
% \end{align*}
% Therefore for all $\lambda\leq e^{-1}$, we obtain that
% \begin{align*}
% \textsl{df}(\lambda)\leq  \int_{\lambda}^{1}\gamma^{-\alpha}(\alpha)\frac{(\log(u\lambda^{-1}))^{\alpha-1}}{u}du+C_0\gamma^{-\alpha}\alpha\log(\lambda^{-1})^{\alpha-1}\int_{1}^{\infty} \frac{(\log(u)+1)^{\alpha-1}}{C_0 u+u^2}du
% \end{align*}
% Finally we obtain that
% \begin{align*}
% \textsl{df}(\lambda)\leq \gamma^{-\alpha}[\log(\lambda^{-1})^{\alpha}] +\log(\lambda^{-1})^{\alpha-1}[C_0\gamma^{-\alpha}\alpha \int_{1}^{\infty} \frac{(\log(u)+1)^{\alpha-1}}{C_0 u+u^2}du]
% \end{align*}
% Therefore we have
% \begin{align*}
% \textsl{df}(\lambda)&\leq Q \log(\lambda^{-1})^{\alpha}\\
% \text{where \quad} Q&=\gamma^{-\alpha} \left[1+C_0\int_{1}^{\infty} \frac{(\log(u)+1)^{\alpha-1}}{C_0 u+u^2}du\right]
% \end{align*}
% \end{proof}

% % Let us now introduce the following result which give us a standard way to obtain a tight bound of the estimation error:


% % \begin{thm}{\cite{fischer2017sobolev}}
% % \label{thm:stein-oracle-1}
% % Let $0<\beta\leq 2$ and $H$ a separable RKHS on $\mathcal{X}$ with respect to a bounded and measurable kernel $k$ and $\rho$ a probability measure on $\mathcal{X}\times\mathcal{Y}$ with $\int_{\mathcal{X}\times\mathcal{Y}}y^2d\rho(x,y) < \infty$. We assume that $\Vert f_{\rho}\Vert_{L_{\infty}^{d\rho_{\mathcal{X}}}} < \infty$ and that there exist $g\in L_2^{d\rho_{\mathcal{X}}}(\mathcal{X})$ such that $f_\rho=T_{\rho}^{\beta/2}g$.
% % Furthermore, we assume that there exist $\sigma>0$ and $L>0$ such that
% % \begin{equation}
% %  \int_{\mathcal{Y}} |y-f_{\rho}(x)|^m d\rho(y|x)\leq \frac{1}{2}m!L^{m-2} 
% % \end{equation}
% % for $\rho_{X}$-almost all $x\in\mathcal{X}$ and all $m\geq 2$.
% % Then for $\tau \geq 1$, $\lambda>0$ and $\ell\geq N_{\lambda,\tau}$
% %  we have with $\rho^{\ell}$-probability $\geq 1-4e^{-\tau}$,
% % \begin{equation}
% % \label{eq:main-upper-inequality}
% % \Vert f_{\mathbf{z},\lambda}-f_{\rho,\lambda}\Vert_{\rho}^2\leq 128\frac{\tau^2}{\ell}\left(5\text{df}(\lambda)\sigma_{\lambda}^2+ K \frac{L_{\lambda}}{\ell\lambda}   \right)
% % \end{equation}
% % where
% % \begin{align*}
% % N_{\lambda,\tau}&= \text{max}\left(\frac{256\tau^2 K\text{df}(\lambda)}{\lambda},\frac{16\tau K}{\lambda}, \tau \right)\\
% % \sigma_{\lambda}&=\text{max}(\sigma,\Vert f_{\rho}- f_{\rho,\lambda}\Vert_{L_\infty^{d\rho_{\mathcal{X}}}})\\
% % L_{\lambda}&=\text{max}(L,\Vert f_{\rho}-f_{\rho,\lambda}\Vert_{L_\infty^{d\rho_{\mathcal{X}}}})\\
% % K &= sup_{x\in\mathcal{X}}k(x,x)
% % \end{align*}
% % \end{thm}
% Let us now split the error $\Vert f_{H,\mathbf{z},\lambda}-f_{\rho}\Vert_{\rho}^2$ into two parts.
% \begin{equation*}
% \Vert f_{H,\mathbf{z},\lambda}-f_{\rho}\Vert_{\rho}^2\leq 2 \Vert f_{H,\mathbf{z},\lambda}-f_{H,\rho,\lambda}\Vert_{\rho}^2 + 2\Vert f_{H,\rho,\lambda}-f_{\rho}\Vert_{\rho}^2
% \end{equation*}
% The following Lemma provides a control of the approximation error.
% \begin{lemma}
% \label{lem:approx-error}
% Let $0 < \beta \leq 2$, $\rho$ a probability measure on $\mathcal{X} \times\mathcal{Y}$ and H a separable RKHS on $\mathcal{X}$ with respect to a bounded and measurable kernel k. If there exist $g\in L_2^{d\rho_{\mathcal{X}}}(\mathcal{X})$ such that $f_\rho=T_{\rho}^{\beta/2}g$, then for all $\lambda > 0$ it holds
% $$\Vert f_{H,\rho,\lambda}-f_{\rho}\Vert_{\rho}^2 \leq  \lambda^{\beta} \Vert g\Vert^{2}_{\rho}$$ 
% \end{lemma}
% \begin{proof}
% By denoting $a_i:=\langle f_{\rho},e_i\rangle_{L_2^{d\rho_{\mathcal{X}}}}$ we have
% \begin{align*}
% \Big\Vert f_{H,\rho,\lambda}-f_{\rho}\Big\Vert_{\rho}^2&=\Big\Vert \sum_{i\in\mathcal{I}}\frac{\mu_i}{\mu_i+\lambda}a_i e_i - \sum_{i\in\mathcal{I}} a_i e_i\Big\Vert_{\rho}^2\\
% &=\lambda^2 \sum_{i\in \mathcal{I}}  \left(\frac{\mu_i^{\frac{\beta}{2}}}{\mu_i+\lambda}\right)^{2}\mu_{i}^{-\beta}a_i^2
% \end{align*}
% Let us consider the following function for $\lambda>0$ and $0\leq \gamma\leq 1$ $f_{\lambda,\gamma}:t\in\mathbb{R}_{+}\rightarrow \frac{t^{\gamma}}{t+\lambda}$. By considering the derivative of $f_{\lambda,\gamma}$, we obtain that $\text{sup}_{t\in\mathbb{R}_{+}}f_{\lambda,\gamma}\leq \lambda^{\gamma-1}$, therefore we have
% \begin{align*}
% \Vert f_{H,\rho,\lambda}-f_{\rho}\Vert_{\rho}^2&\leq \lambda^{\beta}\sum_{i\in\mathcal{I}}\mu_{i}^{-\beta}a_i^2\\
% &\leq \lambda^{\beta} \Vert g\Vert^{2}_{\rho}
% \end{align*}
% \end{proof}
% Let us now focus on the estimation error. Let $\tau \geq 1$, $\lambda>0$. Thanks to theorem \ref{thm:stein-oracle-1} we have with $\rho^{\ell}$-probability $\geq 1-4e^{-\tau}$,
% \begin{equation}
% \label{eq:main-upper-inequality}
% \Vert f_{\mathbf{z},\lambda}-f_{\rho,\lambda}\Vert_{\rho}^2\leq 128\frac{\tau^2}{\ell}\left(5\text{df}(\lambda)\sigma_{\lambda}^2+ K \frac{L_{\lambda}}{\ell\lambda}   \right)
% \end{equation}
% as soon as  $\ell\geq N_{\lambda,\tau}$ where $K = \sup_{x\in\mathcal{X}}k(x,x)$ and 
% \begin{align*}
% N_{\lambda,\tau}&= \max\left(\frac{256\tau^2 K\text{df}(\lambda)}{\lambda},\frac{16\tau K}{\lambda}, \tau \right)\\
% \sigma_{\lambda}&=\max(\sigma,\Vert f_{\rho}- f_{\rho,\lambda}\Vert_{L_\infty^{d\rho_{\mathcal{X}}}})\\
% L_{\lambda}&=\max(L,\Vert f_{\rho}-f_{\rho,\lambda}\Vert_{L_\infty^{d\rho_{\mathcal{X}}}})
% \end{align*}
% In the next Lemma, we exhibit a control $N_{\lambda,\tau}$, $L_{\lambda}^2$ and $\sigma_{\lambda}^2$.
% \begin{lemma}
% \label{lem:control-const}
% Let $\rho\in  \mathcal{F}_{H,\alpha,\beta}$ be a probability measure. Then there are constants $N, V >0$ depending only on $\mathcal{F}_{H,\alpha,\beta}$ such that $N_{\lambda,\tau}\leq N \frac{\tau^2\log(\lambda^{-1})^{\alpha}}{\lambda}$  and $L_{\lambda}^2,\sigma_{\lambda}^2\leq \frac{V}{\lambda^{\text{max}(1-\beta,0)}}$ for all $0<\lambda \leq e^{-1}$ and $\tau\geq 1$.
% \end{lemma}
% \begin{proof}
% Thanks to Lemma \ref{lem:effective-dim-geo}, we have that
% \begin{align*}
% \textsl{df}(\lambda)&\leq Q \log(\lambda^{-1})^{\alpha}\\
% \text{where \quad} Q&=\gamma^{-\alpha} \left[1+C_0\int_{1}^{\infty} \frac{(\log(u)+1)^{\alpha-1}}{C_0 u+u^2}du\right]
% \end{align*}
% And by definition we have
% \begin{align*}
% N_{\lambda,\tau}&\leq \text{max}\left(\frac{256\tau^2 K\text{df}(\lambda)}{\lambda},\frac{16\tau K}{\lambda}, \tau \right)\\
% &\leq N \frac{\tau^2 \log(\lambda^{-1})^{\alpha}}{\lambda}\\
% \text{where \quad} N&=\text{max}(256KQ,16K,1)
% \end{align*}
% Moreover we have
% \begin{align*}
% \Vert f_{\rho}- f_{H,\rho,\lambda}\Vert_{L_\infty^{d\rho_{\mathcal{X}}}}^2&\leq 2(\Vert f_{\rho}\Vert_{L_\infty^{d\rho_{\mathcal{X}}}}^2+\Vert f_{\rho,\lambda}\Vert_{L_\infty^{d\rho_{\mathcal{X}}}}^2\\
% &\leq 2B_{\infty}+2K\Vert f_{H,\rho,\lambda}\Vert_{H}^2)\\
% \end{align*}
% But by denoting $a_i:=\langle f_{\rho},e_i\rangle_{L_2^{d\rho_{\mathcal{X}}}(\mathcal{X})}$ we remark that
% \begin{align*}
% \Vert f_{H,\rho,\lambda}\Vert_{H}^2=\Big\Vert \sum_{i\in I}\frac{\mu_i}{\mu_i+\lambda}a_i e_i\Big\Vert_H^2= \sum_{i\in I}\left(\frac{\mu_i}{\mu_i+\lambda}\right)^2 a_i^2 \mu_i^{-1}=\sum_{i\in I}\left(\frac{\mu_{i}^{\frac{\beta+1}{2}}}{\mu_i+\lambda}\right)^2 a_i^2 \mu_i^{-\beta}
% \end{align*}
% Indeed the first equality is due to the fact that we have assumed the existence of $\beta>0$ and $g\in L_2^{d\rho_{\mathcal{X}}}(\mathcal{X})$ such that $f_\rho=T_{\rho}^{\beta/2} g$.
% Let us now consider the following function for $\lambda>0$ and $0\leq \gamma\leq 1$ $f_{\lambda,\gamma}:t\in\mathbb{R}_{+}\rightarrow \frac{t^{\gamma}}{t+\lambda}$. By considering the derivative of $f_{\lambda,\gamma}$, we obtain that $\sup\limits_{t\in\mathbb{R}_{+}}f_{\lambda,\gamma}\leq \lambda^{\gamma-1}$
% Therefore if $0<\beta \leq 1$ we have that
% \begin{align*}
% \Vert f_{H,\rho,\lambda}\Vert_{H}^2 \leq \lambda^{\beta-1} \Vert g\Vert_{\rho}^{2}\leq \lambda^{\beta-1} B  
% \end{align*}
% Finally if $\beta>1$ then $f_{\rho}\in H$ and we have
% \begin{align*}
% \Vert f_{\rho}- f_{H,\rho,\lambda}\Vert_{L_\infty^{d\rho_{\mathcal{X}}}}^2\leq K\Vert f_{\rho}- f_{H,\rho,\lambda}\Vert_{H}^2
% \end{align*}
% But we have
% \begin{align*}
% \Vert f_{\rho}- f_{H,\rho,\lambda}\Vert_{H}^2=\Big\Vert \sum_{i\in I}\frac{\lambda}{\mu_i+\lambda} a_i e_i\Big\Vert_{H}^2=\sum_{i\in I} \left(\frac{\lambda}{\mu_i+\lambda}\right)^2 a_i^2\mu_i^{-1}=\lambda^2\sum_{i\in I} \left(\frac{\mu_i^{\frac{\beta-1}{2}}}{\mu_i+\lambda}\right)^2 a_i^2\mu_i^{-\beta}
% \end{align*}
% And as $\beta > 1$, we obtain that
% \begin{align*}
% \Vert f_{\rho}- f_{H,\rho,\lambda}\Vert_{H}^2\leq \lambda^{\beta-1}\Vert g\Vert_{\rho}\leq B 
% \end{align*}
% Finally by choosing $V=\text{max}(L^2,\sigma^2,2BK+ 2B_{\infty})$ we obtain that
% $L_{\lambda}^2,\sigma_{\lambda}^2\leq \frac{V}{\lambda^{\text{max}(1-\beta,0)}}$.
% \end{proof}
% We can now prove the Theorem. If $\ell\geq N\frac{\tau^2 \log(\lambda^{-1})^{\alpha}}{\lambda}$ with $N$ a constant from Lemma \ref{lem:control-const} we obtain that
% \begin{align*}
% \Vert f_{H,\mathbf{z},\lambda}-f_{H,\rho,\lambda}\Vert_{\rho}^2&\leq
% C_1\left[\frac{\tau^2}{\ell \lambda^{\text{max}(0,1-\beta)}}\left(\log(\lambda^{-1})^{\alpha}+\frac{1}{\ell \lambda}\right)\right]\\
% \text{where\quad } C_1&=128*V\text{max}(5*Q,K)
% \end{align*}
% with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$. We finally have
% \begin{align*}
% \Vert f_{H,\mathbf{z},\lambda}-f_{\rho}\Vert_{\rho}^2&\leq
% C\left[\lambda^{\beta}+\frac{\tau^2}{\ell \lambda^{\text{max}(0,1-\beta)}}\left(\log(\lambda^{-1})^{\alpha}+\frac{1}{\ell \lambda}\right)\right]\\
% \text{where\quad } C&=2*\text{max}(B,128*V\text{max}(5*Q,K))
% \end{align*}
% with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$.
% Now if we assume that $\beta>1$ and $\lambda_{\ell} = \frac{1}{\ell^{1/\beta}}$, we obtain that
% \begin{align*}
% \Vert f_{H,\mathbf{z},\lambda}-f_{\rho}\Vert_{\rho}^2&\leq
% C\left[\frac{1}{\ell}+\frac{\tau^2}{\ell}\left(\frac{1}{\beta^{\alpha}}\log(\ell)^{\alpha}+\frac{1}{\ell^{1-\frac{1}{\beta}}}\right)\right]\\
% &\leq 3C\tau^2\frac{\log(\ell)^{\alpha}}{\ell}
% \end{align*}
% with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ provided that
% \begin{align}
% \label{condition-ell}
%  \ell\geq  \text{max}\left(e^{\beta}, N\frac{\tau^2 \log(\lambda_{\ell}^{-1})^{\alpha}}{\lambda_{\ell}}\right)
% \end{align}
% Moreover as $\beta>1$, $\frac{\ell \lambda_{\ell}}{\log(\lambda_{\ell}^{-1})^{\alpha}}=\frac{\ell^{1-\frac{1}{\beta}}}{\frac{1}{\beta^{\alpha}}\log(\ell)^{\alpha}}$ goes to infinity as $\ell$ goes to infinity, we conclude that there exist $\ell_{\tau}$ such that for all $\ell\geq \ell_{\tau}$, the condition (\ref{condition-ell}) is satisfied and we finally have
% \begin{equation*}
% \lim_{\tau\rightarrow +\infty}\lim \sup_{\ell\rightarrow\infty}\sup_{\rho\in \mathcal{F}_{H,\alpha,\beta}} \rho^{\ell}\left(\mathbf{z}:\Vert f_{H,\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2>\tau \frac{\log(\ell)^{\alpha}}{\ell}\right)=0
% \end{equation*}
% Now if we consider the case where $0<\beta< 1$, by considering $\lambda_\ell=\frac{\log(\ell)^{\frac{\alpha}{\beta}}}{\ell}$ we obtain
%  \begin{align*}
%  \Vert f_{H,\mathbf{z},\lambda}-f_{\rho}\Vert_{\rho}^2&\leq
% C\left[\frac{\log(\ell)^{\alpha}}{\ell^{\beta}}+\frac{\tau^2}{\ell^{\beta}}\left([\log(\ell)-\log(\log(\ell)^{\frac{\alpha}{\beta}})]^{\alpha}+\frac{1}{\log(\ell)^{\frac{\alpha}{\beta}}}\right)\right]\\
% &\leq 3C\tau^2\frac{\log(\ell)^{\alpha}}{\ell^{\beta}}
% \end{align*}
% with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ provided that 
% \begin{align*}
% \ell\geq \text{max}\left(N\frac{\tau^2 \log(\lambda_{\ell}^{-1})^{\alpha}}{\lambda_{\ell}},e^1\log(\ell)^{\frac{\alpha}{\beta}}\right)
% \end{align*}
% Moreover we have that
% \begin{align*}
% \frac{\ell \lambda_{\ell}}{\log(\lambda_{\ell}^{-1})^{\alpha}}=\frac{\log(\ell)^{\frac{\alpha}{\beta}}}{[\log(\ell)-\log(\log(\ell)^{\frac{\alpha}{\beta}})]^{\alpha}}
% \end{align*}
% And as $0<\beta<1$, we finally have that  $\frac{\ell \lambda_{\ell}}{\log(\lambda_{\ell}^{-1})^{\alpha}}\rightarrow \infty$ as $\ell$ goes to infinity and we have
% \begin{equation*}
% \lim_{\tau\rightarrow +\infty}\lim \sup_{\ell\rightarrow\infty}\sup_{\rho\in \mathcal{F}_{H,\alpha,\beta}} \rho^{\ell}\left(\mathbf{z}:\Vert f_{H,\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2>\tau \frac{\log(\ell)^{\alpha}}{\ell^{\beta}}\right)=0
% \end{equation*}

% Finally let consider the case where $\beta =1$. By considering $\lambda_{\ell}=\frac{\log(\ell)^{\mu}}{\ell}$ with $\mu>\alpha>0$ we obtain
%  \begin{align*}
%  \Vert f_{H,\mathbf{z},\lambda}-f_{\rho}\Vert_{\rho}^2\leq 3C\tau^2\frac{\log(\ell)^{\mu}}{\ell}
% \end{align*}
% with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ provided that 
% \begin{align*}
% \ell\geq \text{max}\left(N\frac{\tau^2 \log(\lambda_{\ell}^{-1})^{\alpha}}{\lambda_{\ell}}, e^1\log(\ell)^{\mu} \right)
% \end{align*}
% Finally as $\mu>\alpha>0$ we have that
%  $\frac{\ell \lambda_{\ell}}{\log(\lambda_{\ell}^{-1})^{\alpha}}=\frac{\log(\ell)^{\mu}}{[\log(\ell)-\log(\log(\ell)^{\frac{\mu}{\beta}})]^{\alpha}}\rightarrow \infty$ as $\ell$ goes to infinity and the asymptotic result follows.
%  \medbreak
%  As a reminder, we have obtained the result for $C=2*\text{max}(B,128*V\text{max}(5*Q,K))$ and $N= \text{max}(256KQ,16K,1)$ where $Q=\gamma^{-\alpha} \left[1+C_0\int_{1}^{\infty} \frac{(\log(u)+1)^{\alpha-1}}{C_0 u+u^2}du\right]$,  $V=\text{max}(L^2,\sigma^2,2BK+ 2B_{\infty})$, and $K=  \sup_{x\in\mathcal{X}}k(x,x)$.
 



% % \begin{thm}
% % Let $H$ be a separable RKHS on $\mathcal{X}$ with respect to a bounded and measurable kernel k, $\alpha>0$, $0<\beta\leq 2$ and $\rho\in \mathcal{F}_{H,\alpha,\beta}$. Moreover let $\tau\geq 1$ and $(\lambda_{\ell})_{\ell\geq 1}$ a sequence of regularization parameters. By denoting $N=\text{max}(256KQ,16K,1)$, $C=2*\text{max}(B,128*V\text{max}(5*Q,K))$, 
% % $V=\text{max}(L^2,\sigma^2,2BK+ 2B_{\infty})$, $Q=\gamma^{-\alpha} \left[1+C\int_{1}^{\infty} \frac{(\log(u)+1)^{\alpha-1}}{C u+u^2}du\right]$ and $K = sup_{x\in\mathcal{X}}k(x,x)$ we have:
% % \begin{itemize}
% % \item  If $\beta> 1$, then for $\ell\geq \text{max}\left(e^{\beta},\left(\frac{N}{\beta^{\alpha}}\right)^{\frac{\beta}{\beta-1}}\tau^{\frac{2\beta}{\beta-1}} \log(\ell)^{\frac{\alpha\beta}{\beta-1}}\right)$ and $\lambda_{\ell}=\frac{1}{\ell^{1/\beta}}$, with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
% %     \begin{align*}
% % \Vert f_{\mathbf{z},\lambda}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{\alpha}}{\ell}
% %     \end{align*}
    
% %     \item  If $\beta = 1$, then for $\ell\geq \text{max}\left(\exp\left((N\tau)^{\frac{1}{\mu-\alpha}}\right),e^{1}\log(\ell)^{\mu}\right)$ and $\mu>\alpha>0$, with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
% %     \begin{align*}
% %     \Vert f_{\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{\mu}}{\ell^{\beta}}
% %     \end{align*}
% %     \item  If $\beta < 1$, then for $\ell\geq \text{max}\left(\exp\left((N\tau)^{\frac{\beta}{\alpha(1-\beta)}}\right),e^{1}\log(\ell)^{\frac{\alpha}{\beta}}\right)$, with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
% %     \begin{align*}
% %     \Vert f_{\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{\alpha}}{\ell^{\beta}}
% %     \end{align*}
% % \end{itemize}
% % \end{thm}
% \end{proof}

% \subsection{Proof of Theorem \ref{thm:lower-rate}}
% \label{proof:lower-rate}
% \begin{proof}
% We follow the suggestion of presented in section 3 of \cite{fischer2017sobolev} in order to construct a family of probability measures $\rho_{f}\in\mathcal{F}_{H,\alpha,q,\beta}$ parametrized by suitable vectors $f\in H$. Let $\nu\in \mathcal{P}_{H,\alpha,q}$  and let us denote $\hat{\sigma} = \text{min}(\sigma, L)$. Then we define for a measurable function $f: \mathcal{X}\rightarrow \mathcal{Y}$ and $x\in\mathcal{X}$ the distribution $\rho_f(.|x):= \mathcal{N}(f(x),\hat{\sigma}^2)$ as the normal distribution on $\mathcal{Y} = \mathbb{R}$ with mean $f(x)$ and variance $\hat{\sigma}^2$. Hence $\rho_f(A)=\int_{\mathcal{X}}\int_{\mathcal{Y}}\mathbf{1}_{A}(x,y) d\rho_{f}(y|x)d\nu(x)$ defines a probability measure on $\mathcal{X}\times \mathcal{Y}$ with marginal distribution $\nu$ on $\mathcal{X}$, i.e. $(\rho_f)_{\mathcal{X}} = \nu$. 
% For $f\in L_2^{d\nu}(\mathcal{X})$ we have $\int_{\mathcal{X}\times\mathcal{Y}} y^2 d\rho_{f}(x,y) = \hat{\sigma}^2 + \Vert f \Vert_{L_2^{d\nu}(\mathcal{X})}^2 <\infty$ and $f_{\rho_{f}}=f$. Moreover, the properties of the normal distribution
% implies $\int_{\mathcal{Y}} |y-f(x)|^m d\rho_{f}(y|x)\leq \frac{1}{2}m!\hat{\sigma}^m$ for all $x\in\mathcal{X}$. Hence if $\Vert f \Vert^{2}_{L_{\infty}^{d\nu}(\mathcal{X})}<B_{\infty}$  and there exist $g\in L_2^{d\nu}(\mathcal{X})$ such that $f_{\rho_{f}}=T_{\rho_{f}}^{\beta/2}g$ and $\Vert g\Vert_{L_2^{d\nu}(\mathcal{X})}^2\leq B$, then $\rho_f\in \mathcal{F}_{H,\alpha,q,\beta}$. So we reduced the construction of probability measures to the construction of appropriate functions $f$. To this end we use binary strings $\omega = (\omega_1,...,\omega_m)\in\{-1,1\}^{m}$ and define for $0<\epsilon <1$
% \begin{align*}
% g_{\omega}&:=\left(\frac{\epsilon}{m}\right)^{1/2}\sum_{i=1}^m \omega_i \mu_i^{-\beta/2} e_i\\
% \text{and \quad} f_{\omega}&:=T_{\nu}^{\beta/2}g_{\omega}=\left(\frac{\epsilon}{m}\right)^{1/2}\sum_{i=1}^m \omega_i  e_i
% \end{align*}
% Because $f_{\omega}$ is a finite linear combination of the eigenvectors $e_i$ of $T_{\nu}$ it holds $\Vert f_{\omega} \Vert^{2}_{L_{\infty}^{d\nu}(\mathcal{X})}<\infty$  and $\Vert g_{\omega}\Vert_{L_2^{d\nu}(\mathcal{X})}^2\leq +\infty$. First we want to establish sufficient conditions on $\epsilon$ and $m$ such that $\Vert f_{\omega} \Vert^{2}_{L_{\infty}^{d\nu}(\mathcal{X})}<B_{\infty}$ and $\Vert g_{\omega}\Vert_{L_2^{d\nu}(\mathcal{X})}^2\leq B$. In the following we denote  $\Vert .\Vert_{\nu}:=\Vert .\Vert_{L_2^{d\nu}(\mathcal{X})}$. 
% \begin{lemma}
% \label{lem:epsilon_1}
% Let $H$ be a separable RKHS on $\mathcal{X}$ with respect to a bounded and measurable kernel k, $q\geq\gamma >0$, $\alpha>0$, $0<\beta\leq 2$ such that $\mathcal{P}_{H,\alpha,q}$ is not empty and let $\nu\in \mathcal{P}_{H,\alpha,q}$. Then there is are constants $U,v> 0$ and $0 < \epsilon_1 \leq 1$ depending only on $\mathcal{F}_{H,\alpha,q,\beta}$, such that $\Vert f_{\omega} \Vert^{2}_{L_{\infty}^{d\nu}(\mathcal{X})}<B_{\infty}$ and $\Vert g_{\omega}\Vert_{\nu}^2\leq B$ holds for all $0 < \epsilon \leq \epsilon_1$ and all $m \leq  U\log(v\epsilon^{-1})^{\alpha}$.
% \end{lemma}
% \begin{proof}
% Let $m\in\mathbb{N}$ and $0<\epsilon<1$. Therefore we have
% \begin{align*}
%  \Vert g_{\omega}\Vert_{\nu}^2= \frac{\epsilon}{m}\sum_{i=1}^m \omega_i \mu_{i}^{-\beta}
%  \leq \epsilon \mu_{m}^{-\beta}
%  \leq c^{-\beta}\epsilon e^{q\beta m^{1/\alpha}}
% \end{align*}
% Moreover we have
% \begin{align*}
% \Vert f_{\omega} \Vert^{2}_{L_{\infty}^{d\nu}(\mathcal{X})}\leq K\Vert f_{\omega}\Vert_{H}^2\leq \frac{K}{c}\epsilon e^{q m^{1/\alpha}}
% \end{align*}
% Therefore by considering $U:=\text{min}(\frac{1}{q^{\alpha}},\frac{1}{(q\beta)^{\alpha}})$ and $v:=\text{min}(\frac{BC}{K},B_{\infty}c^{\beta})$, we obtain that for all $\epsilon\leq \epsilon_1:= \text{min}(1,v)$ and all $m \leq  U\log(v\epsilon^{-1})^{\alpha}$, $\Vert f_{\omega} \Vert^{2}_{L_{\infty}^{d\nu}(\mathcal{X})}<B_{\infty}$ and $\Vert g_{\omega}\Vert_{\nu}^2\leq B$.
% \end{proof}


% If $\omega' = (\omega_1', . . ., \omega_m') \in\{-1,1\}^m$ is an other binary string, we investigate the norm of the difference $f_{\omega}-f_{\omega'}$. We obtain that
% \begin{align*}
% \Vert f_{\omega}-f_{\omega'}\Vert_{\nu}^2=\frac{\epsilon}{m}\sum_{i=1}^m(\omega_i-\omega_i')^2
% \end{align*}
% Therefore as $(\omega_i-\omega_i')^2\leq 4$ we obtain that:
% \begin{align*}
% \Vert f_{\omega}-f_{\omega'}\Vert_{\nu}^2\leq 4\epsilon
% \end{align*}
% In order to obtain a lower bound,  we assume that $\sum_{i=1}^m (\omega_i - \omega_i')^2 \geq m$, i.e. the distance between $\omega$ and $\omega'$ is large, and finally we obtain
% \begin{align*}
% \Vert f_{\omega}-f_{\omega'}\Vert_{\nu}^2\geq \epsilon
% \end{align*}
% The following theorem is a restatement of Theorem 3.1 of \cite{devore2006approximation} in our setting.
% \begin{thm}
% \label{thm:before-thm}
% Let $H$ be a separable RKHS on $\mathcal{X}$ with respect to a bounded and measurable kernel k, $q\geq \gamma>0$, $\alpha>0$, $0<\beta\leq 2$ such that $\mathcal{P}_{H,\alpha,q}$ is not empty and let $\nu\in \mathcal{P}_{H,\alpha,q}$. Let also $\mathbf{z}\rightarrow f_{\mathbf{z}}$ an arbitrary measurable learning method  for $\ell\in\mathbb{N}$ and $\mathbf{z}\in Z^{\ell}$.  Then there exist $0<\epsilon_0\leq 1$ such that for all $\epsilon \leq \epsilon_0$ and for all $\ell\in\mathbb{N}$ there is a $\rho\in \mathcal{F}_{H,\alpha,q,\beta}$ such that 
% \begin{align*}
% \rho^{\ell}\left(\mathbf{z}: \Vert f_{\mathbf{z}}-f_{\rho}\Vert_{\rho}^2>\frac{\epsilon}{4}\right)\geq\text{min}\left(\frac{N_{\epsilon}^*}{N_{\epsilon}^* +1}, \hat{\eta}\sqrt{N_{\epsilon}^*}e^{-\frac{4\epsilon \ell}{2\hat{\sigma}^2}}\right)
% \end{align*}
% where $N_{\epsilon}^*=e^{\frac{U}{48}\log(v\epsilon^{-1})^{\alpha}}$ and $\hat{\eta}=e^{-3/e}$.
% \end{thm}
% \begin{proof}
% Thanks to Lemma \ref{lem:epsilon_1},  there exists $1\geq \epsilon_1>0$ and $U,v>0$ such that for all $\omega$, $0<\epsilon\leq \epsilon_1$ and $m\leq U\log(v\epsilon^{-1})^{\alpha}$ we have $\rho_{f_{\omega}}\in\mathcal{F}_{H,\alpha,q,\beta}$. Let us now fix $0<\epsilon<\epsilon_1$, and consider the case where $m=\lfloor U\log(v\epsilon^{-1})\rfloor$. Moreover Theorem \ref{prop:number_of_func} suggests that there are many binary strings with large distances. Indeed as soon as $m\geq 16$, 
% there exists $f_{\omega^1},...,f_{\omega^{N_{\epsilon}}}$ where $N_{\epsilon}\geq e^{m/24}\geq N_{\epsilon}^{*} $ such that $\rho_{f_{\omega^1}},...,\rho_{f_{\omega^{N_{\epsilon}}}}\in\mathcal{F}_{H,\alpha,q,\beta}$, and for all $i\neq j\in[|1,N_{\epsilon}|]$ we have: 
% \begin{align*}
% \label{eq:lower-bound}
% 4\epsilon \geq \Vert f_{\omega^{i}}-f_{\omega^{j}}\Vert_{\nu}^2\geq \epsilon
% \end{align*}
% In fact if we assume that $\epsilon\leq\epsilon_0:= \text{min}(\epsilon_1,v e^{-(\frac{17}{U})^{1/\alpha}})$, then $m\geq 16$ is satisfied and the above results hold. Now, given $\ell\in\mathbb{N}$, let
% \begin{align*}
% A_i:=\left\{\mathbf{z}:\Vert f_{\mathbf{z}}-f_{\omega^{i}}\Vert_{\nu}^2 <\frac{\epsilon}{4} \right\}
% \end{align*}
% for all $i=1,...,N^{\epsilon}$. Thanks to the lower bound Eq.\ref{eq:lower-bound}, we obtain that $A_i\cap A_j = \emptyset$ 
% if $i\neq j$, therefore thanks to Lemma \ref{lem:devore-approx}  we have that there exist $i\in[|1,N_{\epsilon}|]$, such that $\rho=\rho_{f_{\omega^i}}$ and that either
% \begin{align*}
% p:=\rho^{\ell}(A_i)>\frac{N_{\epsilon}}{N_{\epsilon}+1}\geq \frac{N_{\epsilon}^*}{N_{\epsilon}^*+1}
% \end{align*}
%  or
% \begin{align*}
% \frac{4\epsilon \ell}{2\hat{\sigma}^2}\geq -\log(p)+\log(\sqrt{N_{\epsilon}^*})-3/e
% \end{align*}
% The left-hand side of the latter inequality comes from the fact that we can describe the Kullback-Leibler divergence for these measures. Indeed thanks to Lemma \ref{lem:KL-div} for $f,f'\in L_2^{d\nu}(\mathcal{X})$ and $\ell \geq  1$ it holds $\rho_f^{\ell} \ll \rho_{f'}^{\ell}$ and $\rho_f^{\ell} \gg \rho_{f'}^{\ell}$ . Furthermore, the KL
% divergence fulfills
% \begin{align*}
% \text{KL}(\rho_f^{\ell},\rho_{f'}^{\ell})=\frac{\ell}{2\hat{\sigma}^2}\Vert f-f'\Vert_{L_2^{d\nu}(\mathcal{X})}^2
% \end{align*}
% And as $f_{\rho}=f_{\rho_{f_{\omega^i}}}=f_{\omega^i}$ we obtain that
% \begin{align*}
% \rho^{\ell}\left(\mathbf{z}: \Vert f_{\mathbf{z}}-f_{\rho}\Vert_{\rho}^2>\frac{\epsilon}{4}\right)\geq\text{min}\left(\frac{N_{\epsilon}^*}{N_{\epsilon}^* +1}, \hat{\eta}\sqrt{N_{\epsilon}^*}e^{-\frac{4\epsilon \ell}{2\hat{\sigma}^2}}\right)
% \end{align*}
% \end{proof}
% %We can finally provides the proof of the theorem:
% % \begin{thm}
% % Let $H$ be a separable RKHS on $\mathcal{X}$ with respect to a bounded and measurable kernel k, $q\geq \gamma>0$, $\alpha>0$, $0<\beta\leq 2$ such that $\mathcal{P}_{H,\alpha,q}$ is not empty. Then it holds 
% % \begin{align*}
% %  \lim_{\tau\rightarrow 0^{+}}\lim\inf_{\ell\rightarrow\infty}\inf_{f_{\mathbf{z}}}\sup_{\rho\in\mathcal{F}_{H,\alpha,q,\beta}} \rho^{\ell}\left(\mathbf{z}:\Vert f_{\mathbf{z}}-f_{\rho}\Vert_{\rho}^2>\tau b_{\ell}\right)=1
% % \end{align*}
% % where $b_{\ell}=\frac{\log(\ell)^{\alpha}}{\ell}$. The infimum is taken over all measurable learning methods with respect to $\mathcal{F}_{H,\alpha,q,\beta}$.
% % \end{thm}
% We can now give a proof of the theorem. Given $\tau>0$, for all $\ell\in\mathbb{N}$, let $\epsilon_{\ell}=4\tau\frac{\log(\ell)^{\alpha}}{\ell}$. Since $\epsilon_{\ell}$ goes to $0$ when $\ell$ goes to $\infty$, for $\ell$ large enough, $\epsilon_{\ell}\leq \epsilon_0$, and we can apply Theorem \ref{thm:before-thm} and we obtain
% \begin{align*}
% \inf_{f_{\mathbf{z}}}\sup_{\rho\in\mathcal{F}_{H,\alpha,q,\beta}}\rho^{\ell}\left(\mathbf{z}: \Vert f_{\mathbf{z}}-f_{\rho}\Vert_{\rho}^2>\tau\frac{\log(\ell)^{\alpha}}{\ell}  \right)\geq \text{min}\left(\frac{N_{\epsilon_{\ell}}^*}{N_{\epsilon_{\ell}}^* +1}, \hat{\eta}\sqrt{N_{\epsilon_{\ell}}^*}e^{-\frac{4\epsilon_{\ell} \ell}{2\hat{\sigma}^2}} \right)
% \end{align*}
% Moreover we have
% \begin{align*}
% \sqrt{N_{\epsilon_{\ell}}^*}e^{-\frac{4\epsilon_{\ell} \ell}{2\hat{\sigma}^2}}=e^{\frac{U}{96}[\log(\ell)-\frac{v}{4\tau\log(l)^{\alpha}}]^{\alpha}}\times e^{-\frac{8\tau\log(\ell)^{\alpha}}{\hat{\sigma}^2}}
% \end{align*}
% Therefore if $\tau$ is small enough such that $\tau<\frac{U\hat{\sigma}^2}{768}$, the quantity $\sqrt{N_{\epsilon_{\ell}}^*}e^{-\frac{4\epsilon_{\ell} \ell}{2\hat{\sigma}^2}}$ goes to $\infty$ as $\ell$ goes to $\infty$. Also if $\ell$ goes to $\infty$, $\frac{N_{\epsilon_{\ell}}^*}{N_{\epsilon_{\ell}}^* +1}$ goes to $1$. Finally we obtain that: 
% \begin{align*}
%  \lim_{\tau\rightarrow 0^{+}}\lim\inf_{\ell\rightarrow\infty}\inf_{f_{\mathbf{z}}}\sup_{\rho\in\mathcal{F}_{H,\alpha,q,\beta}} \rho^{\ell}\left(\mathbf{z}:\Vert f_{\mathbf{z}}-f_{\rho}\Vert_{\rho}^2>\tau b_{\ell}\right)=1
% \end{align*}
% \end{proof}



\section{Multi-Layer Perceptrons}
\label{section:MLP-def}
We refer to here as a multi-layer perceptron a fully-connected deep neural network~\cite{shalevshwartz2014}. We give below useful definitions for our construction in the next sections. 
Let $\mathcal{X}$ be a subset of $\mathbb{R}^d$, $N$ be the number of hidden layers, $\sigma_1,...,\sigma_N$ real-valued functions defined on $\mathbb{R}$ be the activation functions at each layer and $m_1,...,m_N$ be the width of each layer. Set $m_0:=d$ and $m_{N+1}:=1$. Then, any function defined by a multi-layer perceptron (MLP) is parameterized by weight matrices $(W^k)_{k=1}^{N+1}$ where each $W^k\in\mathbb{R}^{m_{k-1}m_{k}}$ and can be recovered as follows. Let $x\in\mathcal{X}$, define $\mathcal{N}^0(x):=x$ and for $k\in\{1,\dots,N\}$,  denote
$W^k:=(w_1^k,...,w_{m_{k}}^k)$ where for all  $j\in[|1,m_k|]$ $w_j^k\in\mathbb{R}^{m_{k-1}}$. Then, for all $k\in\{1,...,N\}$, define the $k^{\text{th}}$ layer as
$$\mathcal{N}^{k}(x):=(\sigma_k(\langle \mathcal{N}^{k-1}(x),w_1^k \rangle), ...,\sigma_k(\langle \mathcal{N}^{k-1}(x),w_{m_k}^k \rangle))$$

We obtain $\mathcal{N}(x)=\langle \mathcal{N}^N(x),W^{N+1}\rangle_{\mathbb{R}^{m_N}}$.
We shall denote $\mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N,(m_i)_{i=1}^N}$ the function space defined by all functions $\mathcal{N}$ defined as above on $\mathcal{X}$ for any choice of $(W^k)_{k=1}^{N+1}$. We shall also consider the union space
$$\mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N}:=\bigcup_{(m_1,...,m_N)\in\mathbb{N_{*}}^N} \mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N,(m_i)_{i=1}^N} .$$



\subsection{Proof of Proposition \ref{prop:RKHS-MLP}}
\label{proof:lem-rkhs}

Before proving the result, let us first recall the following definition.
\begin{defn}[\textbf{$cc$-universal kernel}]
\label{def:cc-universal}
A continuous positive semi-definite  kernel k on a Hausdorff space $\mathcal{X}$ is said to be $cc$-universal if the RKHS, H induced by k is dense in $\mathcal{C}(\mathcal{X})$ endowed with the topology of compact convergence.
\end{defn}

\begin{proof}
Let $N\geq 0$ be the number of layers, $(m_1,...,m_N)\in\mathbb{N_{*}}^N$ and let $(\sigma_i)_{i=1}^N$ be a sequence of N functions which admits a Taylor decomposition in 0 on $\mathbb{R}$ such that for every $i\in[|1,N|]$ and $x\in\mathbb{R}$
\begin{align*}
\sigma_i(x)=\sum_{t\geq 0} a_{i,t} x^t
\end{align*}
We can now define the sequence $(f_i)_{i=1}^N$ such that  for every $i\in[|1,N|]$ and $x\in\mathbb{R}$
\begin{align*}
f_i(x):=\sum_{t\geq 0} |a_{i,t}| x^t
\end{align*}
Let us now introduce two sequence of functions  $(\phi_i)_{i=1}^N$ and $(\psi_i)_{i=1}^N$  such that for all $ i\in[|1,N|]$ and $x\in \ell_2$
\begin{align*}
\phi_i(x):=\left(\sqrt{|a_{i,t}|}x_{k_1}...x_{k_t}\right)_{\underset{k_1,...,k_t\in\mathbb{N}}{t\in\mathbb{N}}}\\
\psi_i(x):=\left(\frac{a_{i,t}}{\sqrt{|a_{i,t}|}}x_{k_1}...x_{k_t}\right)_{\underset{k_1,...,k_t\in\mathbb{N}}{t\in\mathbb{N}}}\\
\end{align*}
with the convention that $\frac{0}{0}=0$. Moreover as a countable union of countable sets is countable and $(\sigma_i)_{i=1}^N$ are defined on $\mathbb{R}$, we have that for all $x\in\ell_2$ and $i\in[|1,N|]$,  $\phi_i(x),\psi_i(x)\in\ell_2$. Indeed there exists a bijection $\mu:\mathbb{N}\rightarrow\cup_{t\geq 0} \mathbb{N}^t$, therefore we can denote for all $i\in[|1,N|]$ and $x\in\ell_2$, 
$\phi_i(x)=(\phi_i(x)_{\mu(j)})_{j\in\mathbb{N}}$ and $\psi_i(x)=(\psi_i(x)_{\mu(j)})_{j\in\mathbb{N}}$. We have then
\begin{align*}
%\label{eq:feature-map}
\langle \phi_i(x), \phi_i(x')\rangle_{\ell_2}&=\sum_{j\in\mathbb{N}} \phi_i(x)_{\mu(j)}\phi_i(x')_{\mu(j)}\\
&=\sum_{t\geq 0} |a_{i,t}| \sum_{k_1,...,k_t} x_{k_1}...x_{k_t} x_{k_1}'..x_{k_t}'\\
&=\sum_{t\geq 0} |a_{i,t}| \langle x,x'\rangle_{\ell_2}^t\\
&=f_i( \langle x,x'\rangle_{\ell_2})
\end{align*}
Moreover the same calculations lead also to the fact that
\begin{align*}
\langle \psi_i(x), \psi_i(x')\rangle_{\ell_2}=f_i( \langle x,x'\rangle_{\ell_2})
\end{align*}
Therefore $\phi_i$ and $\psi_i$ are a feature maps of the positive semi-definite kernel $k_i:x,x'\in\ell_2\times\ell_2\rightarrow f_i( \langle x,x'\rangle_{\ell_2})$ and we have
\begin{align*}
\langle \phi_i(x), \phi_i(x)\rangle_{\ell_2}=\langle \psi_i(x), \psi_i(x)\rangle_{\ell_2}=f_i(\Vert x\Vert^2_{\ell_2})<\infty
\end{align*}  
Finally let us define the sequence of kernels $(K_i)_{i=1}^N$ defined on $\mathcal{X}\times\mathcal{X}$ such that, for all $x,x'\in\mathcal{X}$
\begin{align*}
K_i(x,x'):=f_i\circ...\circ f_1(\langle x,x'\rangle_{\mathbb{R}^d})
\end{align*}
and let us denote $(H_i)_{i=1}^N$ the sequence of RKHS associated. Moreover in the following, we consider $\mathbb{R}^d$ as a subset of $\ell_2$. One can easily show by induction on $i\in[|1,N|]$ that for all $x,x'\in\mathcal{X}$
\begin{align*}
K_i(x,x')=\langle \phi_i\circ...\phi_1(x), \phi_i\circ...\phi_1(x')\rangle_{\ell_2}
\end{align*}
Let us denote $\mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N}$ the function space defined by a neural network where the activations are the $(\sigma_i)_{i=1}^N$. Moreover let $(W^k)_{k=1}^{N+1}$ be any sequence such that for all $k\in [|1,N+1|]$, $W^k:=(w_j^k)_{j=1}^{m_k}\in\mathcal{M}_{m_{k-1},m_{k}}(\mathbb{R})$  and $\mathcal{N}$ the function in $\mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N}$  associated. Let us now show by induction that at each layer $i\in[|1,N|]$ of the neural network, for $k\in [|1,m_{i}|]$, the coordinate $N^i_{k}$ is a function which lives in $H_i$ such that for all $x\in\mathcal{X}$
\begin{align*}
N_{k}^i(x)=\left\langle \psi_i\left(\sum_{j_{i-1}=1}^{m_{i-1}} W^{i}_{j_{i-1},k}\psi_{i-1}\left(...\psi_2\left(\sum_{j_1=1}^{m_1}W^{2}_{j_1,j_2}\psi_1(w^{1}_{j_1})\right)...\right)\right),\phi_i\circ...\circ\phi_1(x)\right\rangle_{\ell_2}
\end{align*} 
For $i=1$, we have for all $k\in [|1,m_{1}|]$
\begin{align*}
N_{k}^1(x)=\sigma_1(\langle x,w_{k}^{1}\rangle)
\end{align*}
where $w_{k}^{1}\in\mathbb{R}^d\subset\ell_2$. In fact we can show that for every $w\in\mathbb{R}^d$, $x\in\mathcal{X}\rightarrow \sigma_1(\langle x,w\rangle)$ lives in $H_1$. Indeed we have
\begin{align*}
\sigma_1(\langle x,w\rangle)&=\sum_{t\geq 0} a_{1,t} \langle x,w\rangle^t\\
&=\sum_{t\geq 0} a_{1,t} \sum_{k_1,...,k_t} x_{k_1}...x_{k_t}w_{k_1}...w_{k_t}\\
&=\sum_{t\geq 0} \sum_{k_1,...,k_t}\sqrt{a_{1,t}} x_{k_1}...x_{k_t}\frac{a_{1,t}}{\sqrt{a_{1,t}} }w_{k_1}...w_{k_t}\\
&=\langle \phi_1(x),\psi_1(w)\rangle_{\ell_2}
\end{align*}
Thanks to Theorem \ref{thm:RKHS-Inclusion} the following application $x\in\mathcal{X}\rightarrow \sigma_1(\langle x,w\rangle)$ lives in $H_1$ and finally we have for all $k\in[|1,m_1|]$: 
\begin{align*}
N_{k}^1(x)=\langle \phi_1(x),\psi_1(w^1_k)\rangle\in H_1
\end{align*}
\end{proof}
Let us assume that the result hold for $i\in[|1,N-1|]$ and let $k\in[|1,m_{i+1}|]$, then we have by definition of the neural network that for all $x\in\mathcal{X}$
\begin{align*}
N_{k}^{i+1}(x)&=\sigma_{i+1}\left(\langle N^{i}(x),w^{i+1}_k\rangle_{\mathbb{R}^{m_i}}\right)\\
&=\sigma_{i+1}\left(\sum_{j_{i}=1}^{m_{i}} W^{i+1}_{j_i,k} N^{i}_{j_i}(x)\right)
\end{align*}
Then by induction we have that
\begin{align*}
N_{k}^{i+1}(x)&=\sigma_{i+1}\left(\left\langle \sum_{j_{i}=1}^{m_{i}} W^{i+1}_{j_i,k} V^i_{j_i},\phi_i\circ...\circ\phi_1(x) \right\rangle_{\ell_2}\right)\\
\text{where \quad} V^i_{j_i}&:= \psi_i\left(\sum_{j_{i-1}=1}^{m_{i-1}} W^{i}_{j_{i-1},j_i}\psi_{i-1}\left(...\psi_2\left(\sum_{j_1=1}^{m_1}W^{2}_{j_1,j_2}\psi_1(w^{1}_{j_1})\right)...\right)\right)\in \ell_2
\end{align*}
Therefore we obtain
\begin{align*}
N_{k}^{i+1}(x)=\left\langle \psi_{i+1}\left(\sum_{j_{i}=1}^{m_{i}} W^{i+1}_{j_i,k} V^i_{j_i}\right),\phi_{i+1}\circ...\circ\phi_1(x) \right\rangle_{\ell_2}
\end{align*}
And finally, thanks to Theorem \ref{thm:RKHS-Inclusion}, we have that
$x\in\mathcal{X}\rightarrow N_{k}^{i+1}(x)$ lives in $H_{i+1}$ and  we have for all $k\in[|1,m_{i+1}|]$
\begin{align*}
N_{k}^{i+1}(x)=\left\langle \psi_{i+1}\left(\sum_{j_{i}=1}^{m_{i}} W^{i+1}_{j_{i},k}\psi_{i}\left(...\psi_2\left(\sum_{j_1=1}^{m_1}W^{2}_{j_1,j_2}\psi_1(w^{1}_{j_1})\right)...\right)\right),\phi_{i+1}\circ...\circ\phi_1(x)\right\rangle_{\ell_2}
\end{align*} 

Now let us show that $\mathcal{N}$ lives in $H_N$ and that we can bound its RKHS norm. Indeed by definition of $\mathcal{N}$ we have that for all 
$x\in\mathcal{X}$
\begin{align*}
\mathcal{N}(x)&=\langle \mathcal{N}^N(x), W^{N+1}\rangle_{\mathbb{R}^{m_N}}\\
&=\sum_{j_{N}=1}^{m_N} W^{N+1}_{j_{N}} \mathcal{N}^N_{j_N}(x)
\end{align*}
And thanks to what precedes, we have that for all $j_N\in[|1,m_N|]$, $\mathcal{N}^{N}_{j_N}\in H_N$, then as a linear combination of the $(\mathcal{N}^{N}_{j_N})_{j=1}^{m_N}$, we finally have that $\mathcal{N}\in H_N$. Moreover thanks to what precedes we have
\begin{align*}
\mathcal{N}(x)=\left\langle \sum_{j_{N}=1}^{m_N} W^{N+1}_{j_{N}} \psi_{N}\left(\sum_{j_{N-1}=1}^{m_{N-1}} W^{N}_{j_{N-1},j_N}\psi_{N-1}\left(...\psi_2\left(\sum_{j_1=1}^{m_1}W^{2}_{j_1,j_2}\psi_1(w^{1}_{j_1})\right)...\right)\right),\phi_{N}\circ...\circ\phi_1(x)\right\rangle_{\ell_2}
\end{align*}
Therefore thanks to the Theorem \ref{thm:RKHS-Inclusion} we have that
\begin{align*}
\Vert \mathcal{N} \Vert_{H_N}^2\leq \left\Vert \sum_{j_{N}=1}^{m_N} W^{N+1}_{j_{N}} \psi_{N}\left(\sum_{j_{N-1}=1}^{m_{N-1}} W^{N}_{j_{N-1},j_N}\psi_{N-1}\left(...\psi_2\left(\sum_{j_1=1}^{m_1}W^{2}_{j_1,j_2}\psi_1(w^{1}_{j_1})\right)...\right)\right) \right\Vert_{\ell_2}^2
\end{align*}
Moreover, as  the $(\phi_i)_{i=1}^N$ are respectively  feature maps of the kernels $(k_i)_{i=1}^N$,  one can show by  induction that
\begin{align*}
&\left\Vert \sum_{j_{N}=1}^{m_N} W^{N+1}_{j_{N}} \psi_{N}\left(\sum_{j_{N-1}=1}^{m_{N-1}} W^{N}_{j_{N-1},j_N}\psi_{N-1}\left(...\psi_2\left(\sum_{j_1=1}^{m_1}W^{2}_{j_1,j_2}\psi_1(w^{1}_{j_1})\right)...\right)\right) \right\Vert_{\ell_2}^2\\
&=(W^{N+1})^Tf_N\left((W^{N})^{T} f_{N-1}\left((W^{N-1})^{T}...f_2\left((W^{2})^{T}f_1\left((W^1)^{T}W^1\right)W^2\right)...W^{N-1}\right)W^{N}\right)W^{N+1}
\end{align*}
where the $(f_i)_{i=1}^N$ are functions acting coordinate-wise. Thanks to the Schur Inequality \cite{horn2012matrix}, we obtain that for all $k\in\mathbb{N}$ and any $A\in\mathcal{M}_n(\mathbb{R})$
\begin{align*}
\Vert A^{\circ k}\Vert\leq \Vert A \Vert^k
\end{align*}
And as for all $i \in [|1,N|]$, $(|a_{i,t}|)_{t\geq 0}$ are non negative sequences, we obtain that for all $i\in [|1,N|]$ and $A\in\mathcal{M}_n(\mathbb{R})$
\begin{align*}
\Vert f_i(A) \Vert \leq f_i(\Vert A\Vert)
\end{align*}
Finally by a simple induction we obtain that
\begin{align*}
&(W^{N+1})^Tf_N\left((W^{N})^{T} f_{N-1}\left((W^{N-1})^{T}...f_2\left((W^{2})^{T}f_1\left((W^1)^{T}W^1\right)W^2\right)...W^{N-1}\right)W^{N}\right)W^{N+1}\\
&\leq \Vert W^{N+1} \Vert^2 f_N(\Vert W^{N} \Vert^{2} f_{N-1} (...f_1(\Vert W^1\Vert^2)...))
\end{align*}
And we obtain our upper bound of the RKHS norm of $\mathcal{N}$.



Finally let us assume that for every $i\in[|1,N|]$ and $n\in\mathbb{N}$ we have $\sigma_i^{(n)}(0)\neq 0$. Then by denoting by $(b_m)_{m\geq 0}$ the coefficients of the Taylor decomposition of $f_N\circ ...\circ f_1$, the following Lemma ensures that for every $m\geq 0$, $b_m>0$. 
See proof in Sec.~\ref{lem-proof-explicitcoeffcomp}).
\begin{lemma}
\label{lem:explicitcoeffcomp}
Let $(f_i)_{i=1}^N$ a family of functions that can be expanded in Taylor series in 0 on $\mathbb{R}$ such that for all $k\in[|1,N|]$, $(f_{k}^{(n)}(0))_{n\geq 0}$ are positive. Let us define also $\phi_{1},...,\phi_{N-1}:\mathbb{N}^2\rightarrow \mathbb{R}_{+}$ such that for every $k\in[|1,N-1|]$ and $l,m\geq 0$:
\begin{align*}
\phi_{k}(l,m):=\frac{d^m}{dt^m}|_{t=0}\frac{f_{k}^{l}(t)}{m!}
\end{align*}
Then $g:=f_N\circ ...\circ f_1$ can be expanded in its Taylor series in 0 on $\mathbb{R}$ such that for all $t\in\mathbb{R}$:
\begin{align*}
g(t)=\sum_{l_1,...,l_{N}\geq 0}\frac{f_N^{(l_N)}(0)}{l_{N}!}\times 
\phi_{N-1}(l_N,l_{N-1}) \text{...}\times \phi_{1}(l_2,l_1) t^{l_1}
\end{align*}
Moreover $(g^{(n)}(0))_{n\geq 0}$ is a positive sequence.
\end{lemma}
Therefore thanks to the positivity of the coefficient $(b_m)_{m\geq 0}$ the $cc$-universality of $K_N$ follows directly from Theorem \ref{thm:univ_classic}.

\textbf{Examples.} Consider the case where the input space $\mathcal{X}$ is the unit sphere. Therefore if we assume that for all $i\in\{1,...,N\}$, $f_i(1)=1$ then the norm is preserved across the layers as we obtain that
$K_i(x,x) = \Vert x\Vert_2^2$. In that case, we can consider a larger class of functions as we only need the $(f_i)_{i=1}^N$ to admit a Taylor expansion about 0 on $[-1,1]$. We list some classical functions which satisfy these assumptions \cite{bietti2017group}.
\begin{table}[ht]
%\label{table:2}
\centering
\begin{tabular}{l|l}
polynomial & $f(t)=\frac{1}{p^p}(p-1+t)^p$\\
Inverse polynomial & $f(t)=\frac{1}{2-t}$\\
arc-cosine & $f(t)=\frac{1}{\pi}(\sin(\text{arcos}(t))+(\pi-\text{arcos}(t))\cos(\text{arcos}(t)))$ \\
Vovk's & $f(t)=\frac{1}{3}(1+t+t^2)$
\end{tabular}
\end{table}

Note that the inverse polynomial kernel was used by \cite{zhang2016l1,zhang2017convexified} to build convex models of fully connected networks and two-layer convolutional neural networks, while the arc-cosine kernel appears in early deep kernel machines \cite{NIPS2009_3628}.


Thanks to Proposition~\ref{prop:RKHS-MLP}, we can have a direct control on the RKHS norm of the network through the spectral norm of its weights.
\begin{coro}
\label{coro:norm-mlp}
For $(W^k)_{k=1}^{N+1}$ a sequence such that for all $k\in [|1,N+1|]$, $W^k\in\mathbb{R}^{m_{k-1}m_{k}}$ and $\mathcal{N}$ the function in $\mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N}$ associated, we have
\begin{align*}
\Vert \mathcal{N} \Vert_{H_N}^2 \leq \Vert W^{N+1} \Vert^2 f_N(\Vert W^{N} \Vert^{2} f_{N-1} (...f_1(\Vert W^1\Vert^2)...))
\end{align*}
where $\Vert.\Vert$ is the spectral norm.
\end{coro}
We can then obtain statistical bounds for deep networks such as as the ones in~\cite{zhang2016l1,zhang2017convexified,
bartlett2017spectrally,bietti2017group}. Indeed the RKHS norm of the network allows one to get for instance generalization bounds involving Rademacher complexities as in~\cite{boucheron2005theory}. To be more precise, if $\mathcal{X}$ is compact and $\mathcal{Y}\subset [-M,M]$, then for any $\delta>0$ with a probability $\rho^n$ not less than $1-\delta$
% \begin{align*}
% R(\mathcal{N})& \leq \frac{1}{\ell}\sum_{i=1}^{\ell} (\mathcal{N}(x_i)- y_i)^2
%  +\frac{2 G \Vert \mathcal{N} \Vert_{H_N}}{n}\sqrt{\sum_{i=1}^n K_N(x_i,x_i)} 
% +\frac{2M^2}{\sqrt{n}}+ 3B\sqrt{\frac{ \log(\frac{2}{\delta})}{2n}} \; ,
% \end{align*}
\begin{align*}
R(\mathcal{N})& \leq \frac{1}{\ell}\sum_{i=1}^{\ell} (\mathcal{N}(x_i)- y_i)^2+\mathcal{O}\left( \frac {\Vert \mathcal{N} \Vert_{H_N}}{\sqrt{n}}+ \sqrt{\frac{ \log(\frac{2}{\delta})}{2n}}\right) \; ,
\end{align*}
There are two major issue with these bounds. First they do not consider the approximation bias of the class of functions considered which is the major issue in high dimension. Moreover these generalization bounds may blow up as the number of parameters increases. We will see in the following that we manage to obtain learning rates of the RLS algorithm on the specific RKHSs associated to MLPs which deal with the two above issues.

\subsection{Spectral Analysis of Multi-Layer Perceptrons}
\label{sec:sp-mlp}
\subsubsection{Basic Notions and Notations}

\textbf{Spherical Harmonics.} Let $P_{m}(d)$ be the space of homogeneous polynomials of degree $m$ in $d$ variables with real coefficients and $\mathcal{H}_{m}(d)$ be the space of harmonics polynomials defined by
\begin{align}
\mathcal{H}_m(d):=\{P\in P_{m}(d)| \Delta P=0\}
\end{align}
where $\Delta \cdot = \sum\limits_{i=1}^d\frac{\partial^2\cdot}{\partial x_i^2} $ is the Laplace operator on $\mathbb{R}^d$. Moreover let us define
$H_{m}(S^{d-1})$ the space of real spherical harmonics of degree $m$ defined as the set of restrictions of harmonic polynomials in $\mathcal{H}_{m}(d)$ to $S^{d-1}$. Let also $L_2^{d\sigma_{d-1}}(S^{d-1})$ be the space of (real) square-integrable functions on the sphere $S^{d-1}$ endowed with its induced Lebesgue measure $d\sigma_{d-1}$ and $|S^{d-1}|$ the surface area of $S^{d-1}$. $L_2^{d\sigma_{d-1}}(S^{d-1})$  endowed with its natural inner product is a separable Hilbert space and the family of spaces $(H_m(S^{d-1}))_{m\geq 0}$, yields a direct sum decomposition \cite{frye2012spherical}
\begin{align}
L_2^{d\sigma_{d-1}}(S^{d-1})=\bigoplus_{m\geq 0}H_m(S^{d-1})
\end{align}
which means that the summands are closed and pairwise orthogonal.
Moreover, each $H_m(S^{d-1})$ has a finite dimension $\alpha_{m,d}$ with $\alpha_{0,d}=1$, $\alpha_{1,d}=d$ and for $m\geq 2$
\begin{align*}
\alpha_{m,d}=\dbinom{d-1+m}{m}-\dbinom{d-1+m-2}{m-2}
\end{align*}
Therefore for all $m\geq 0$, given any orthonormal basis of $H_m(S^{d-1})$, $(Y_{m}^1,...,Y_{m}^{\alpha_{m,d}})$, we can build an Hilbertian basis of $L_2^{d\sigma_{d-1}}(S^{d-1})$ by concatenating these orthonormal basis. Let us denote in the following $(Y_{m}^{l_m})_{m,l_m}$ such an Hilbertian basis of $L_2^{d\sigma_{d-1}}(S^{d-1})$.


Before proving the results obtained on the eigenvalue decay in the different regimes, let us recall some useful notations. Let $N\geq 1$, $d\geq 2$ and $(f_i)_{i=1}^N$ be a sequence of N real value functions satisfying assumptions of Proposition \ref{prop:RKHS-MLP}. Therefore $f_N\circ...\circ f_1$ admits a Taylor decomposition on $[-1,1]$, and we can denote its non negative coefficients $(b_m)_{m\geq 0}$ such that
\begin{align*}
 f_N\circ...\circ f_1(x):=\sum_{m\geq 0} b_m x^m.
\end{align*}
Moreover, let $K_N$ be the kernel associated on $S^{d-1}$ defined by:
\begin{align*}
K_{N}(x,x'):=f_N\circ...\circ f_1(\langle x,x'\rangle_{\mathbb{R}^d}) ; .
\end{align*}
we denote the integral operator on $L_2^{d\sigma_{d-1}}(S^{d-1})$ associated 
$$\begin{array}{ccccc}
T_{K_N} & : &  L_2^{ d\sigma_{d-1}}(S^{d-1}) & \to &  L_2^{ d\sigma_{d-1}}(S^{d-1})\\
 & & f &\to & \int_{S^{d-1}} K(x,\cdot)f(x)d\sigma_{d-1}(x).
\end{array}$$
Thanks to theorem \ref{thm:eigenval} we have an explicit formula of the eigenvalues of $T_{K_N}$, the integral operator associated with the kernel $K_N$ defined on $L_{2}^{d\sigma_{d-1}}(S^{d-1})$. Indeed each spherical harmonics of degree $m$, $Y_{m}\in H_{m}(S^{d-1})$, is an eigenfunction of $T_{K_N}$ with associated eigenvalue given by the formula
\begin{align}
\label{eq:lamba-supp-mat}
\lambda_{m}=\frac{|S^{d-2}|\Gamma((d-1)/2)}{2^{m+1}}\sum_{s\geq 0}b_{2s+m}\frac{(2s+m)!}{(2s)!}\frac{\Gamma(s+1/2)}{\Gamma(s+m+d/2)}
\end{align}


\subsubsection{Proof of Proposition \ref{prop:menegato}}
\label{proof:menegato}
\begin{proof}
We consider only the case when $0<\delta <1/2$ as \cite{azevedo2014sharp} show the result for $\delta\geq 1/2$.
Let us denote $\theta_{s,m}=b_{2s+m}\frac{(2s+m)!}{(2s)!}\frac{\Gamma(s+1/2)}{\Gamma(s+m+d/2)}$.
Therefore we have
\begin{align*}
\bigg|\frac{\theta_{s+1,m}}{\theta_{s,m}}\bigg|&= \frac{b_{2s+2+m}}{b_{2s+m}}\frac{(2s+m+2)(2s+m+1)}{(2s+2)(2s+2m+d)}
\end{align*}
Let $0<\delta<1/2$ such that Assumption (\ref{eq:b_n-final-f-2}) hold. There exists a $\gamma$ such that for all $m\geq 1$
\begin{align*}
\frac{|b_{m}|}{|b_{m-1}|}\leq \frac{\gamma}{m^{\delta}} \; .
\end{align*}
Therefore we obtain
\begin{align*}
\bigg|\frac{\theta_{s+1,m}}{\theta_{s,m}}\bigg|\leq \gamma^2 \frac{(2s+m+2)^{1-\delta}(2s+m+1)^{1-\delta}}{(2s+2)(2s+2m+d)} \; .
\end{align*}
Yet since $0<\delta<1/2$ we have
\begin{align*}
\bigg|\frac{\theta_{s+1,m}}{\theta_{s,m}}\bigg|&\leq \gamma^2 \frac{(2s+m+2)^{2-2\delta}}{(2s+2)(2s+2m+d)}\\
&\leq \gamma^2 \frac{(2s+m+2)^{2-2\delta}}{(2s+2)(2s+m+2)}\\
&\leq \gamma^2 \frac{(2s+m+2)^{1-2\delta}}{(2s+2)}
\end{align*}
Let $\alpha:=\frac{1}{1-2\delta}$, therefore we have
\begin{align*}
\bigg|\frac{\theta_{s+1,m}}{\theta_{s,m}}\bigg|^{\alpha}&\leq \gamma^{2\alpha} \frac{(2s+m+2)}{(2s+2)^{\alpha}}\\
&\leq \frac{\gamma^{2\alpha}}{(2s+2)^{\alpha-1}}+\frac{\gamma^{2\alpha}m}{(2s+2)^{\alpha}}
\end{align*}
Therefore we have for all $m,s\geq 0$
\begin{align*}
\bigg|\theta_{s+1,m}\bigg|^{\alpha}\leq \bigg|\theta_{0,m}\bigg|^{\alpha}\prod_{i=0}^s\left(1+\frac{m}{2i+2}\right) \frac{\gamma^{2\alpha (s+1)}}{2^{(\alpha-1)(s+1)}((s+1)!)^{\alpha-1}}
\end{align*}
Moreover, as soon as $s+1\geq m\delta/2$, we have
\begin{align*}
1+\frac{m}{2s+2}\leq 1+ \frac{1}{\delta} \; .
\end{align*}
Therefore for all $m,s\geq 0$ we obtain that
\begin{align*}
\prod_{i=0}^s\left(1+\frac{m}{2i+2}\right)\leq
\left(1+\frac{1}{\delta}\right)^{s+1}
\times \prod_{i=0}^{\lfloor \frac{m\delta}{2}\rfloor}
\left(1+\frac{m}{2i+2}\right)
 \end{align*}
For all $m\geq 2$, and $s\geq 0$, we obtain finally
\begin{align*}
\bigg|\theta_{s+1,m}\bigg|^{\alpha}\leq \bigg|\theta_{0,m}\bigg|^{\alpha} m^{\frac{m\delta}{2}+1}\times \left(\frac{\left(1+\frac{1}{\delta}\right)+\gamma^{2\alpha}}{2^{\alpha-1}}\right)^{s+1}\times \frac{1}{((s+1)!)^{\alpha-1}}
\end{align*}
Let $C:=\frac{\left(1+\frac{1}{\delta}\right)+\gamma^{2\alpha}}{2^{\alpha-1}}$
Therefore we obtain that, for all $m\geq 2$
\begin{align*}
\bigg|\theta_{s,m}\bigg|\leq \bigg|\theta_{0,m}\bigg| m^{\frac{m\delta}{2\alpha}+\frac{1}{\alpha}}\times \frac{(C^{\frac{1}{\alpha}})^s}{(s!)^{\frac{\alpha-1}{\alpha}}}
\end{align*}
And finally for all $m\geq 2$
\begin{align*}
\sum_{s\geq 0} \bigg|\theta_{s,m}\bigg|\leq \bigg|\theta_{0,m}\bigg| m^{\frac{m\delta}{2\alpha}+\frac{1}{\alpha}}\times \sum_{s\geq 0 }\frac{(C^{\frac{1}{\alpha}})^s}{(s!)^{\frac{\alpha-1}{\alpha}}}
\end{align*}
Therefore thanks to Theorem \ref{thm:eigenval} we have
\begin{align*}
\bigg|\lambda_m\bigg| \leq \frac{\sigma_{d-2}\Gamma((d-1)/2)}{2^{m+1}}  \bigg|\theta_{0,m}\bigg| m^{\frac{m\delta}{2\alpha}+\frac{1}{\alpha}}\times \sum_{s\geq 0 }\frac{(C^{\frac{1}{\alpha}})^s}{(s!)^{\frac{\alpha-1}{\alpha}}}
\end{align*}
But as $\bigg|\theta_{0,m}\bigg|=\Gamma(1/2)\frac{b_m m!}{\Gamma(m+d/2)}$, then we obtain
\begin{align*}
\bigg|\lambda_m\bigg| \leq \sigma_{d-2}\Gamma (1/2)\Gamma((d-1)/2)\times 
\sum_{s\geq 0 } \frac{(C^{\frac{1}{\alpha}})^s}{(s!)^{\frac{\alpha-1}{\alpha}}} \times m^{\frac{m\delta}{2\alpha}+\frac{1}{\alpha}} \frac{b_m m!}{2^{m+1} \Gamma(m+d/2)} 
\end{align*}
And as we have
\begin{align*}
\frac{m!}{\Gamma(m+d/2)}\in O\left(\frac{1}{m^{(d-2)/2}}\right)
\end{align*}
Finally we have
\begin{align*}
\lambda_m\in O\left( \frac{m^{\frac{m\delta}{2\alpha}+\frac{1}{\alpha}-\frac{(d-2)}{2}} b_m}{2^{m+1}}\right) \; .
\end{align*}
\end{proof}



\subsubsection{Proof of Proposition \ref{prop:spectrum_anal_gene}}
\label{proof:spectrum_anal_gene}
\begin{proof}
From Theorem \ref{thm:eigenval}, the $(Y_{k}^{l_k})_{k,l_k}$ is an orthonormal basis of eigenfunctions of $T_{K_N}$ associated with the eigenvalues $(\lambda_{k,l_k})_{k,l_k}$ such that for all $k\geq 0$ and $1\leq l_k\leq \alpha_{k,d}$, $\lambda_{k,l_k}:=\lambda_k\geq 0$ where $\lambda_k$ is given by the formula (\ref{eq:lamba-supp-mat}). Moreover Assumption (\ref{eq:b_n-final-f-2}) guarantees that $b_m>0$ for all $m\geq 0$, and thanks to the formula of (\ref{eq:lamba-supp-mat}), we deduce that $(\lambda_{k,l_k})_{k,l_k}$ are exactly the positive eigenvalues of $T_{K_N}$ with their multiplicities and that $M=+\infty$. Let us now define an indexation of the sequence of eigenvalues of $T_{K_N}$. For that purpose we define this following application.
$$\begin{array}{ccccc}
\phi & : &  \mathbb{N}\times\mathbb{N} & \to &  \mathbb{N}\\
 & & (k,q) &\to & \sum\limits_{i=0}^{k-1} \alpha_{i,d} + q - 1
\end{array}$$
with the convention that $\sum\limits_{i=0}^{-1} \alpha_{i,d}=0$. 
Therefore by defining $E:=\{(k,l_k): k\in \mathbb{N} \text{  and  } l_k\in[|1,\alpha_{k,d}|]\}$ we have first that $\phi(E)=\mathbb{N}$ and $\phi_{|E}$ is injective.
Therefore we can define $(\delta_m)_{m\geq 0}$ the sequence of eigenvalues of $T_{K_N}$ with their multiplicities such that for every $m\geq 0$  there exists a unique $(k,l_k)\in E$ such that
\begin{align}
\label{eq:def-order-gene}
m&:=\phi(k,l_k)=\sum\limits_{i=0}^{k-1} \alpha_{i,d} + l_k - 1\\
\delta_m&:=\lambda_{k,l_k}
\end{align}
Let us define also $ q(\delta,k) = \left\{
              \begin{array}{ll}
                 \frac{k\delta}{2\alpha}+\frac{1}{\alpha}\text{ if  } \frac{1}{2}>\delta>0 \\
                \ 0 \text{ otherwise.}
                \end{array}\right.$\\
Thanks to Proposition \ref{prop:menegato}, there exists a constant $C$ independent of $k$ such that:
\begin{align*}
\lambda_k\leq C \frac{b_k k^{q(\delta,k)}}{2^{k+1}k^{({d-2})/2}}
\end{align*}
Therefore we have:
\begin{align*}
&\delta_m\leq C\frac{b_k k^{q(\delta,k)}}{2^{k+1}k^{({d-2})/2}}\\
\end{align*}
But there exist a constant $Q\geq 2$ such that, for all $k\geq 1$, we have
\begin{align*}
b_k&\leq \frac{Q}{k^{\delta}}b_{k-1}\\
&\leq \frac{Q^k}{(k!)^{\delta}}b_0
\end{align*}
Therefore we have
\begin{align*}
\delta_m \leq C b_0 \frac{Q^k k^{q(\delta,k)}}{2^{k+1}k^{({d-2})/2}(k!)^{\delta}}
\end{align*}
Then by applying the Stirling formula, there exist a constant $L>0$  such that
\begin{align*}
\delta_m\leq C L b_0 \frac{e^{\delta k} Q^k}{2^{k+1}k^{({d-2})/2+\delta/2}}\frac{ k^{q(\delta,k)}}{ k^{\delta k }}
\end{align*}
Moreover we remarks that if $\delta >\frac{1}{2}$,
\begin{align*}
\delta k-q(\delta,k)= \delta k
\end{align*}
Otherwise we have that
\begin{align*}
\delta k-q(\delta,k)= \delta k(1-\frac{1}{2\alpha})-\frac{1}{\alpha}
\end{align*}
But as soon as $0<\delta<1/2$, $\alpha>1$, therefore we have that for all $\delta>0$
\begin{align*}
\delta_m\leq C L b_0 \frac{e^{\delta k} Q^k}{2^{k+1}k^{({d-2})/2+\delta/2}}\frac{1}{ k^{\frac{\delta k}{2}-1}}
\end{align*}
Moreover there exist $Q_2\geq 1\geq Q_1>0$ constants only depending on $d$  such that
\begin{align*}
Q_1  m^{\frac{1}{d-1}} \leq k \leq Q_2 m^{\frac{1}{d-1}}
\end{align*}
Therefore we obtain that
\begin{align*}
\delta_m \leq \frac{C L b_0}{2 Q_1^{(d-2)/2}} \frac{(\frac{e^{\delta}Q}{2})^{Q_2 m^{\frac{1}{d-1}}} Q_2 m^{\frac{1}{d-1}}}{ (Q_1m^{\frac{1}{d-1}})^{\frac{Q_1 \delta}{2}  m^{\frac{1}{d-1}}}}
\end{align*}
Finally by denoting $s:= \frac{4(d-1)}{Q_1}$ which is independent of $\delta$ we obtain that
\begin{align*}
\delta_m\times m^{\frac{\delta}{s}m^{\frac{1}{d-1}}}\leq \frac{C L b_0}{2 Q_1^{(d-2)/2}} \frac{(\frac{e^{\delta}Q}{2})^{Q_2 m^{\frac{1}{d-1}}} Q_2 m^{\frac{1}{d-1}}}{ (Q_1)^{\frac{Q_1 \delta}{2}  m^{\frac{1}{d-1}}}  m^{\frac{\delta}{s}m^{\frac{1}{d-1}}}}
\end{align*}
And as the Right-Hand side of the inequality is bounded we obtain that:
\begin{align*}
\delta_m&\in O\left(m^{-\frac{\delta}{s} m^{\frac{1}{d-1}}}\right)\\
\end{align*}
Finally Assumption (\ref{eq:b_n-final-f-2}) guarantees that eventually the sequence $(\delta_{m})_{m\geq 0}$ is exactly the sequence of eigenvalues ordered in the non-increasing order. Indeed we have the following Proposition.
\begin{lemma}
\label{decroissance_gene}
If $(b_m)_{m\geq 0}$ is a non-increasing sequence eventually, then $(\delta_m)_{m\geq 0}$ is a non-increasing sequence eventually. 
\end{lemma}
\begin{proof}
For a fixed $k$ we have that
\begin{align*}
\frac{2s+k+1}{2s+2k+d}<1 \text{  for all  }s\geq 0
\end{align*}
and as $(b_m)_{m\geq 0}$ is a non increasing sequence eventually, then there exists $k_0\geq 0$ such that for all $k\geq k_0$ and $s\geq 0$
\begin{align*}
    b_{2s+k+1}\leq b_{2s+k}
\end{align*}
Therefore for all $k\geq k_0$, we have $\lambda_k\geq \lambda_{k+1}>0$ and the result follows.
\end{proof}
Therefore the sequence $(\delta_{m})_{m\geq 0}$ coincides eventually with the sequence of eigenvalues of the integral operator $T_{K_N}$ ordered in the non-increasing order and the result follows.
\end{proof}


\subsubsection{Proof of Proposition \ref{prop:eta-control}}
\label{proof:eta-control}
\begin{proof}
Let us first provides a control of $(\lambda_m)_{m\geq 0}$ defined in Eq. (\ref{eq:lamba-supp-mat}).
\begin{prop} 
\label{prop:control_lambda_k}
If there exist $1>r>0$ and $0<c_2\leq c_1$ constants  such that for all $m\geq 0$
\begin{align}
\label{eq:assump_geometric-2}
c_2 r^{m} \leq b_m\leq c_1 r^m
\end{align}
then by denoting $C_1= \frac{|S^{d-2}|\Gamma((d-1)/2)}{2}   \frac{2^{\frac{d-1}{2}}c_1}{1-r^2} $ and $C_2= |S^{d-2}|\Gamma((d-1)/2)\Gamma(1/2) L \frac{c_2}{2}$ where $L$ is a constant only depending on $d$, we have that
all $m\geq 0$
\begin{align*}
C_2 \left(\frac{r}{4}\right)^m \leq \lambda_{m}\leq C_1 r^m
\end{align*}
\end{prop}
\begin{proof}
Let us denote $\theta_{s,m}=b_{2s+m}\frac{(2s+m)!}{(2s)!}\frac{\Gamma(s+1/2)}{\Gamma(s+m+d/2)}$.
Therefore we have:
\begin{align*}
\theta_{s,m}&= b_{2s+m} \frac{(2s+m)...(2s+1)}{(s+m+\frac{d-2}{2})...(s+\frac{1}{2})}\\
&=b_{2s+m} \frac{(2s+m)...(2s+1)}{(2s+2m+d-2)...(2s+1)}\times 2^{m+\frac{d-1}{2}}\\
&\leq 2^{\frac{d-1}{2}}c_1 (2r)^m r^{2s} 
\end{align*}
The last inequality comes from the fact that $ \frac{(2s+m)...(2s+1)}{(2s+2m+d-2)...(2s+1)}\leq 1$ and the upper bound given in Eq. (\ref{eq:assump_geometric-2}).
Therefore we have
\begin{align*}
\sum_{s\geq 0}\theta_{s,m}\leq (2r)^m \frac{2^{\frac{d-1}{2}}c_1}{1-r^2} 
\end{align*}
We also have
\begin{align*}
\lambda_{m}=\frac{|S^{d-2}|\Gamma((d-1)/2)}{2^{m+1}}\sum_{s\geq 0}\theta_{s,m}\leq r^m \frac{|S^{d-2}|\Gamma((d-1)/2)}{2}   \frac{2^{\frac{d-1}{2}}c_1}{1-r^2} 
\end{align*}
Moreover we have
\begin{align*}
\lambda_{m}=\frac{|S^{d-2}|\Gamma((d-1)/2)}{2^{m+1}}\sum_{s\geq 0}\theta_{s,m}&\geq  \frac{|S^{d-2}|\Gamma((d-1)/2)}{2^{m+1}} \theta_{0,m}\\
&\geq b_m \frac{|S^{d-2}|\Gamma((d-1)/2)}{2^{m+1}} \frac{m!\Gamma(1/2)}{\Gamma(m+d/2)}\\
&\geq   |S^{d-2}|\Gamma((d-1)/2)\Gamma(1/2) \frac{c_2}{2} \left(\frac{r}{2}\right)^m \frac{m!}{\Gamma(m+d/2)}
\end{align*}
The last inequality comes from the lower bound given in in Eq. (\ref{eq:assump_geometric-2}).
Moreover thanks to the Stirling’s approximation formula we have
\begin{align*}
\Gamma(x)\sim   \sqrt{2\pi} x^{x-1/2}e^{-x}
\end{align*}
which leads to 
\begin{align*}
\frac{m!}{\Gamma(m+d/2)}\sim e^{d/2}\left(1-\frac{d/2}{m+d/2} \right)^m \frac{m^{1/2}}{(m+d/2)^{d-1/2}}
\end{align*}
Finally we obtain
\begin{align*}
 \frac{m!}{\Gamma(m+d/2)}\sim\frac{1}{m^{d-1/2}}   
\end{align*}
Therefore there exists a constant $L>0$ only depending on $d$ such that for all $m\geq 0$ we have
\begin{align*}
\frac{m!}{\Gamma(m+d/2)}\geq L \frac{1}{2^m}
\end{align*}
Finally we have
\begin{align*}
\lambda_{m}\geq |S^{d-2}|\Gamma((d-1)/2)\Gamma(1/2) L \frac{c_2}{2} \left(\frac{r}{4}\right)^m 
\end{align*}
\end{proof}
We are now able to prove the result. From Theorem \ref{thm:eigenval}, the $(Y_{k}^{l_k})_{k,l_k}$ is an orthonormal basis of eigenfunctions of $T_{K_N}$ associated with the eigenvalues $(\lambda_{k,l_k})_{k,l_k}$ such that for all $k\geq 0$ and $1\leq l_k\leq \alpha_{k,d}$, $\lambda_{k,l_k}:=\lambda_k\geq 0$ where $\lambda_k$ is given by the formula (\ref{def:formula_eigen}). Moreover the assumption (\ref{eq:assump_geometric-2}) guarantees that $b_m>0$ for all $m\geq 0$, and thanks to the formula of (\ref{eq:lamba-supp-mat}), we deduce that $(\lambda_{k,l_k})_{k,l_k}$ are exactly the positive eigenvalues of $T_{K_N}$ with their multiplicities and that $M=+\infty$.
Let us now define an indexation of the sequence of eigenvalues of $T_{K_N}$. Therefore we can define $(\delta_m)_{m\geq 0}$ the sequence of eigenvalues of $T_{K_N}$ with their multiplicities such that for every $m\geq 0$  there exists a unique $(k,l_k)\in  E:=\{(k,l_k): k\in \mathbb{N} \text{  and  } l_k\in[|1,\alpha_{k,d}|]\}$ such that
\begin{align*}
%\label{eq:def-order-gene}
m&:=\phi(k,l_k)=\sum\limits_{i=0}^{k-1} \alpha_{i,d} + l_k - 1\\
\delta_m&:=\lambda_{k,l_k}
\end{align*}
Thanks to Proposition \ref{prop:control_lambda_k} we have that for all $k\geq 0$
\begin{align*}
C_2 \left(\frac{r}{4}\right)^k \leq \lambda_{k}\leq C_1 r^k
\end{align*}
Let $m\geq 0$ and $k,l_k$ defined as in Eq. (\ref{eq:def-order-gene}).
First we have that for all $k\geq 2$
\begin{align*}
\alpha_{k,d}=\dbinom{d-1+k}{k}-\dbinom{d-1+k-2}{k-2}
\end{align*}
Therefore we have that
\begin{align*}
\sum\limits_{i=0}^{k} \alpha_{i,d}\sim \frac{2k^{d-1}}{(d-1)!}
\end{align*}
Then there exist $Q_2>Q_1>0$ constants only depending on $d$  such that
\begin{align*}
Q_1  m^{\frac{1}{d-1}} \leq k \leq Q_2 m^{\frac{1}{d-1}}
\end{align*}
Then we have
\begin{align*}
   C_2 \left(\frac{r}{2}\right)^{Q_2 m^{\frac{1}{d-1}}}\leq \delta_m\leq C_1 r^{Q_1 m^{\frac{1}{d-1}}}  
\end{align*}
And finally by definition of the $(\eta_m)_{m\geq 0}$ and as the upper and lower bounds of $\delta_m$ are decreasing functions, we obtain that for all $m\geq 0$
\begin{align*}
C_2 e^{-Q_2\log(4/r)m^{\frac{1}{d-1}}} \leq \eta_{m}\leq C_1 e^{-Q_1\log(1/r)m^{\frac{1}{d-1}}} \; .
\end{align*}
% Therefore there exists $C_1,C_2>0$ constants such that for all $m\geq 0$
% \begin{align*}
% C_2 e^{-Q_2\log(4/r)m^{\frac{1}{d-1}}} \leq \eta_{m}\leq C_1 e^{-Q_1\log(1/r)m^{\frac{1}{d-1}}}
% \end{align*}
\end{proof}

\section{Regularized Least-squares for Multi-Layer Perceptrons}
\label{sec:RLS-geo-exp}

\subsection{Proof of Theorem \ref{thm:rls-geo}}
\label{proof:rls-geo}
\begin{proof}
Here the main goal is to control the rate of decay of the eigenvalues associated with the integral operator $T_{\rho}$. Indeed to show the upper rate, we show that there exists $\alpha, C_0,\gamma>0$ such that for any $\rho\in\mathcal{G}_{\omega,\beta}$, the eigenvalues, $(\mu_i)_{i\in I}$ where $I$ is at most countable, of the integral operator $T_{\rho}$ associated with $K_N$ fulfill the following upper bound for all $i \in I$:
\begin{align*}
\mu_i \leq C_0 e^{-\gamma i^{1/\alpha}}
\end{align*}
therefore $\mathcal{G}_{\omega,\beta}\subset $
$\mathcal{F}_{H_N,\alpha,\beta}$ and the result will follow from Theorem \ref{thm:upper-rate}.
Moreover to show the minimax-rate, we show that $I=\mathbb{N}$ and that there exists $c>0$ and $q\geq \gamma>0$ such that for any $\rho\in\mathcal{G}_{\omega,h,\beta}$, the eigenvalues, $(\mu_i)_{i\in I}$ of the integral operator $T_{\rho}$ associated with $K_N$ fulfill the following lower bound for all $i \in I$
\begin{align*}
\mu_i \geq c e^{-q i^{1/\alpha}}
\end{align*}
and the result will follow from Theorem \ref{thm:lower-rate}.
By definition of $(b_m)_{m\geq 0}$, we have
\begin{align}
%\label{def:kernel-dot}
&K_N(x,x')=\sum_{m\geq 0}b_m (\langle x,x'\rangle_{\mathbb{R}^d})^{m}
\end{align}
Let us now derive a tight control of the eigenvalues of $T_{\rho}$, denoted $(\mu_m)_{m\in\mathcal{I}}$, which will conclude the proof. Let us first show that $I=\mathbb{N}$. Indeed as $S^{d-1}$ is compact and $K_N$ continuous,  the Mercer theorem guarantees that $H_N$ and $\mathcal{L}_2^{d\nu}(S^{d-1})$ are isomorphic. Recall now the two key assumptions to obtain a control on the eigenvalues of $T_{\rho}$.
Indeed we have assumed that
\begin{align}
\label{assump:low-upp}
\frac{d\nu}{d\sigma_{d-1}}< \omega\quad\text{ and }\quad \frac{d\nu}{d\sigma_{d-1}}> h
\end{align}
Let us now define 
$$\begin{array}{ccccc}
T_{\omega} & : &  L_2^{ d\sigma_{d-1}}(S^{d-1}) & \to &  L_2^{ d\sigma_{d-1}}(S^{d-1})\\
 & & f &\to & \omega \int_{S^{d-1}} K_N(x,.)f(x)d\sigma_{d-1}(x) - \int_{S^{d-1}} K_N(x,.)f(x)d\nu(x) 
\end{array}$$
and let us denote $E^{k}$, the span of the greatest $k$ eigenvalues strictly positive of $T_{\rho}$ with their multiplicities.\\
Thanks to the Courant–Fischer–Weyl theorem~\cite{HirschF.Francis1999Eofa} we have that
\begin{align*}
\mu_k=\max_{V\subset G_k}\min_{\substack{x\in V\setminus\{0\} \\ \Vert x \Vert = 1}} \langle T_{\rho} x,x\rangle_{L_2^{ d\sigma_{d-1}}(S^{d-1})}
\end{align*}
where $G_k$ is the set of all s.e.v of dimension $k$ in $L_2^{ d\sigma_{d-1}}(S^{d-1})$.
Therefore we have
\begin{align*}
 \eta_k&\geq \frac{1}{\omega}\min_{\substack{x\in E^{k}\setminus\{0\} \\ \Vert x \Vert = 1}} \langle \omega \times T_{K_{N}} x,x\rangle_{L_2^{ d\sigma_{d-1}}(S^{d-1})}\\
&=\frac{1}{\omega}\min_{\substack{x\in E^{k}\setminus\{0\} \\ \Vert x \Vert = 1}} \{\langle T_{\rho} x,x\rangle_{L_2^{ d\sigma_{d-1}}(S^{d-1})}+\langle T_{\omega} x,x\rangle_{L_2^{ d\sigma_{d-1}}(S^{d-1})}\}\\
&\geq \frac{1}{\omega}\min_{\substack{x\in E^{k}\setminus\{0\} \\ \Vert x \Vert = 1}} \langle T_{\rho} x,x\rangle_{L_2^{ d\sigma_{d-1}}(S^{d-1})}+ \frac{1}{\omega}\min_{\substack{x\in E^{k}\setminus\{0\} \\ \Vert x \Vert = 1}} \langle T_{\omega} x,x\rangle_{L_2^{d\sigma_{d-1}}(S^{d-1})}\\
\end{align*}
Then if $T_{\omega}$ is positive we obtain that
\begin{align*}
\eta_k  \geq \frac{1}{\omega} \mu_k  
\end{align*}
Let us now show the positivity of $T_{\omega}$. Thanks to the assumption (\ref{assump:low-upp}), we have that for all $f\in L_2^{d\sigma_{d-1}}(S^{d-1})$ 
\begin{align*}
T_{\omega}(f)=\int_{S^{d-1}}\left[\omega-\frac{d\nu}{d\sigma_{d-1}}\right]K_N(x,.)f(x)d\sigma_{d-1}(x)
\end{align*}
Therefore $v:=\omega-\frac{d\nu}{d\sigma_{d-1}(x)}$ is positive and by denoting $M=\int_{S^{d-1}}v(x)d\sigma_{d-1}(x)$ and by re-scaling the above equality by $\frac{1}{M}$, we have that $V:x\rightarrow \frac{v(x)}{M}$ is a density function and by denoting $d\Gamma=V d\sigma_{d-1}$ we have 
\begin{align*}
 \frac{1}{M}\times T_{\omega}(f)=\int_{S^{d-1}}K_N(x,.)f(x) d\Gamma(x)   
\end{align*}
Therefore $T_{\omega}$ is positive and thanks to Proposition \ref{prop:eta-control}, we have
\begin{align*}
 \mu_m \leq  \omega \eta_m \leq \omega C_1 e^{-Q_1\log(1/r)m^{\frac{1}{d-1}}}  
\end{align*}

Moreover if we assume in addition that the assumption (\ref{assump:low-upp}), we obtain by a similar reasoning that for all $k\geq 0$
\begin{align*}
\eta_k  \leq  \frac{1}{h} \mu_k  \; .
\end{align*}
And we have that for all $m\geq 0$
\begin{align}
\label{eq:geo-control-eigen-rho}
h C_2 e^{-Q_2\log(4/r)m^{\frac{1}{d-1}}}  \leq h \eta_m  \leq \mu_m \leq  \omega \eta_m \leq \omega C_1 e^{-Q_1\log(1/r)m^{\frac{1}{d-1}}} \; .
\end{align}
\textbf{Upper Rate}. Let us now prove Theorem \ref{thm:rls-geo}. Let  $w\geq 1$ and $0<\beta\leq 2$ and
let us denote $\alpha = d-1$ and $\gamma = Q_1\log(\frac{1}{r})$. Thanks to the RHS of Eq. (\ref{eq:geo-control-eigen-rho}) we have that for any $\rho\in\mathcal{G}_{\omega,\beta}$, the eigenvalues, $(\mu_i)_{i\geq 0}$, of the integral operator $T_{\rho}$ associated with $K_N$ fulfill the following upper bound for all $i$:
\begin{align*}
\mu_i \leq \omega C_1 e^{-\gamma i^{1/\alpha}}
\end{align*}
where $C_1 = \frac{|S^{d-2}|\Gamma((d-1)/2)}{2}   \frac{2^{\frac{d-1}{2}}c_1}{1-r^2}$.
Therefore $\mathcal{G}_{\omega,\beta}\subset $
$\mathcal{F}_{H_N,\alpha,\beta}$ and by applying theorem \ref{thm:upper-rate}, we obtain the results for  $C=2*\text{max}(B,128*V\text{max}(5*Q,K))$ and $A= \text{max}(256KQ,16K,1)$ where $Q=\gamma^{-\alpha} \left[1+\omega C_1\int_{1}^{\infty} \frac{(\log(u)+1)^{\alpha-1}}{\omega C_1 u+u^2}du\right]$,  $V=\text{max}(L^2,\sigma^2,2BK+ 2B_{\infty})$, $K=  \sup_{x\in\mathcal{X}}k(x,x)$.
\end{proof}

The following theorem investigates the optimality of our learning rates, from a nonparametric learning viewpoint~\cite{steinwart2008support}.
\begin{thm}
\label{thm:lower-geo}
Let us assume that there exists $0<c_2<c_1$ such that for all $m\geq 0$:
\begin{align*}
  c_2 r^m \leq b_m \leq c_1 r^m
\end{align*}
Then for any $\omega\geq 1 > h >0$ such that $\mathcal{W}_{\omega,h}$ is not empty it holds 
\begin{align*}
 \lim_{\tau\rightarrow 0^{+}}\lim\inf_{\ell\rightarrow\infty}\inf_{f_{\mathbf{z}}}\sup_{\rho\in\mathcal{G}_{\omega,h,\beta}} \rho^{\ell}\left(\mathbf{z}:\Vert f_{\mathbf{z}}-f_{\rho}\Vert_{\rho}^2>\tau b_{\ell}\right)=1
\end{align*}
where $b_{\ell}=\frac{\log(\ell)^{d-1}}{\ell}$. The infimum is taken over all measurable learning methods with respect to $\mathcal{G}_{\omega,h,\beta}$.
\end{thm}
Therefore for such networks, when $\beta>1$ the learning rates of the regularized least-squares estimator stated in theorem  \ref{thm:rls-geo} coincide with the minimax lower
bounds from theorem \ref{thm:lower-geo} and therefore are optimal in the minimax sense.

\begin{proof}
Let $0<h<1\leq \omega$ and let us denote $q=Q_2\log(\frac{4}{r})$. Thanks to the left-hand-side of Eq. (\ref{eq:geo-control-eigen-rho}) we have that for any $\rho\in\mathcal{G}_{\omega,h,\beta}$, the eigenvalues, $(\mu_i)_{i\geq 0}$ of the integral operator $T_{\rho}$ associated with $K_N$ fulfill the following lower bound for all $i$
\begin{align*}
\mu_i \geq hC_2 e^{-q i^{1/\alpha}}
\end{align*}
where $C_2=|S^{d-2}|\Gamma((d-1)/2)\Gamma(1/2) L \frac{c_2}{2}$. Therefore  $\mathcal{G}_{\omega,h,\beta}\subset$ 
$\mathcal{F}_{H_N,\alpha,q,\beta}$ and we can apply Theorem \ref{thm:lower-rate}.
\end{proof}


\textbf{Example.} Consider the case where $\sigma_1=...=\sigma_N=\tanh$. Indeed recall that $\tanh$ admits a Taylor decomposition on $[-1,1]$ with coefficients satisfying assumption (\ref{eq:assump_geometric}) and that $\tanh([-1,1])\subset [-1,1]$. Therefore the functions $(f_i)_{i=1}^N$ associated, even if we may have to renormalize $(f_i)_{i=1}^N$ by their largest values on $[-1,1]$, admit a Taylor decomposition on $[-1,1]$ and the coefficients $(b_m)_{m\geq 0}$ in the Taylor series about 0 of $f_N\circ...\circ f_1$ satisfy assumption (\ref{eq:assump_geometric}). Thus Theorem \ref{thm:rls-geo} can be applied. This case corresponds to the nonlinear function used in \textit{LeNet5}. Note also that the sigmoid function defined as $\sigma:=(1+\exp(-x))^{-1}$ is just a rescaled and shifted version of $\tanh$ which therefore can be used here.



\subsection{Super-geometric Case: Learning rates}
\label{proof:rls-super-geo}
Another regime of interest is the one where the composition of nonlinear functions involved in the network admits a Taylor decomposition with coefficients decreasing super-geometrically. As in the geometric case, the goal is to obtain a control the of the eigenvalues associated with the integral operator $T_{K_N}$. See Appendix~\ref{proof:rls-super-geo}.
\begin{thm}
%\label{thm:super-geo}
Assume that there exists $1 > \delta>0$ such that
\begin{align}
\label{eq:b_n-final}
\left|\frac{b_{m}}{b_{m-1}}\right|\in O(m^{-\delta}) \; .
\end{align}
Let also $0<\beta\leq 2$ and $\omega>0$.
Then there exist a constant $C$ independent of $\beta$ such that
for any $\rho\in \mathcal{G}_{\omega,\beta}$ and $\tau\geq 1$ we have:
\begin{itemize}
\item  If $\beta> 1$, then there exists $\ell_{\tau}>0$ such that for all $\ell\geq \ell_{\tau}$ and $\lambda_{\ell}=\frac{1}{\ell^{1/\beta}}$, with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
    \begin{align*}
    \Vert f_{H_N,\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{d-1}}{[\log(\log(\ell))]^{d-1}\ell}
    \end{align*}
    \item  If $\beta = 1$, then there exists $\ell_{\tau}>0$ such that for all $\ell\geq \ell_{\tau}$, $\lambda_{\ell}=\frac{\log(\ell)^{\mu}}{[\log(\log(\ell))]^{\mu}\ell}$ and $\mu\geq d-1$, with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
    \begin{align*}
    \Vert f_{H_N,\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{\mu}}{[\log(\log(\ell))]^{\mu}\ell}
    \end{align*}
    \item If $\beta < 1$, then there exists $\ell_{\tau}>0$ such that for all $\ell\geq \ell_{\tau}$ and $\lambda_{\ell}=\frac{\log(\ell)^{\frac{d-1}{\beta}}}{[\log(\log(\ell))]^{\frac{d-1}{\beta}}\ell}$ with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
    \begin{align*}
    \Vert f_{H_N,\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{d-1}}{[\log(\log(\ell))]^{d-1}\ell^{\beta}}
    \end{align*}
\end{itemize}
\end{thm}
As expected, in that regime, we obtain faster rates compared to the geometric case as the eigenvalues decrease faster. 



\begin{proof}
Our first goal is to obtain a control of $\text{df}(\lambda)$ associated with $T_{\rho}$ in the super-geometric regime. 
\begin{prop}
\label{prop:df-super-exp}
Let $\omega>0$ and $\nu\in\mathcal{W}_{\omega}$. Let also $(\mu_i)_{i\in I}$, where $I$ is at most countable, be the sequence of eigenvalues with their multiplicities associated with $T_{\rho}$ ranked in the non decreasing order. If there exist $1>\delta>0$ such that
\begin{align*}
%\label{eq:b_n-final}
\left|\frac{b_{m}}{b_{m-1}}\right|\in O(m^{-\delta})
\end{align*}
Then we have:
\begin{align*}
    \degreef(\lambda)\in\mathcal{O}\left(\frac{\log(\lambda^{-1})^{d-1}}{\left(\log(\log(\lambda^{-1}))\right)^{d-1}} \right)
\end{align*}
\end{prop}

\begin{proof}
From Proposition \ref{prop:spectrum_anal_gene}, there exists $0<G\leq 1$ such that
\begin{align*}
\eta_m&\in O\left(m^{-\frac{\delta}{s} m^{\frac{1}{d-1}}}\right) \; ,
\end{align*}
where $s:=\frac{4(d-1)}{G}$. 
Moreover as $S^{d-1}$ is compact and $K_N$ continuous, the Mercer theorem guarantees that $H_N$ and $\mathcal{L}_2^{d\nu}(S^{d-1})$ are isomorphic, and $I=\mathbb{N}$. Therefore, as in the proof of Proposition \ref{thm:rls-geo} the Courant–Fischer–Weyl theorem~\cite{HirschF.Francis1999Eofa} allows us to obtain that for all $m\geq 0$:
\begin{align*}
\mu_m \leq \omega \eta_m \in  O\left(m^{-\frac{\delta}{s} m^{\frac{1}{d-1}}}\right)
\end{align*}

Let $\lambda>0$ and let us now compute $\text{df}(\lambda)$. There exist $\gamma>0$ such that
\begin{align*}
\text{df}(\lambda)=\sum_{i\in I}\frac{\mu_i}{\mu_i+\lambda}\leq \sum_{m\geq 1}\frac{\gamma}{\gamma+\lambda e^{\frac{\delta}{s}\log(m)  m^{\frac{1}{d-1}}}}
\end{align*}
Moreover as the application $x\in[1,+\infty[\rightarrow \frac{\gamma}{\gamma+\lambda e^{\frac{\delta}{s} \log(x) x^{\frac{1}{d-1}}}}$ is positive and decreasing, therefore we have
\begin{align*}
\textsl{df}(\lambda)\leq \int_{1}^{+\infty}\frac{\gamma}{\gamma+\lambda e^{\frac{\delta}{s} \log(x) x^{\frac{1}{d-1}}}} dx
\end{align*}
Let us denote $\alpha= \left(\frac{s}{\delta}\right)^{d-1}$, $g:x\in]1,+\infty[\rightarrow \log(x)^{d-1} x$ and let us consider the following substitution
\begin{align*}
v=\lambda e^{\frac{\delta}{s} \log(x) x^{\frac{1}{d-1}}}
\end{align*}
Therefore we have
\begin{align*}
\int_{1}^{+\infty}\frac{\gamma}{\gamma+\lambda e^{\frac{\delta}{s} \log(x) x^{\frac{1}{d-1}}}} dx = \int_{\lambda}^{+\infty}\frac{\gamma\left[\alpha \frac{d-1}{v}\log(v\lambda^{-1}) \right](g^{-1})'(\alpha \log(v\lambda^{-1})^{d-1})
}{\gamma+v} dv
\end{align*}
Moreover we have for any $\lambda\leq 1$ and $v\geq e^{\alpha^{-\frac{1}{d-1}}}$
\begin{align*}
g\left(\alpha^{\frac{1}{d}}\log(v\lambda^{-1})^{\frac{d-1}{d}}\right)&=\log(\alpha^{\frac{1}{d}}\log(v\lambda^{-1})^{\frac{d-1}{d}})^{d-1} \alpha^{\frac{1}{d}}\log(v\lambda^{-1})^{\frac{d-1}{d}}\\
&\leq \alpha \log(v\lambda^{-1})^{d-1}
\end{align*}
Indeed the latter inequality comes from the fact that $0\leq \log(x)\leq x$ for $x\geq 1$. Therefore by monotonicity of $g$ we obtain that
\begin{align*}
g^{-1}(\alpha \log(v\lambda^{-1})^{d-1})\geq \alpha^{\frac{1}{d}}\log(v\lambda^{-1})^{\frac{d-1}{d}}
\end{align*}
Moreover as $g'(x)=\log(x)^{d-1}+ (d-1)\log(x)^{d-2}$ and it is an increasing function, we obtain that
\begin{align*}
g'\circ g^{-1}(\alpha \log(v\lambda^{-1})^{d-1})&\geq g'(\alpha^{\frac{1}{d}}\log(v\lambda^{-1})^{\frac{d-1}{d}})\\
&\geq \log(\alpha^{\frac{1}{d}}\log(v\lambda^{-1})^{\frac{d-1}{d}})^{d-1}
\end{align*}
where the last inequality comes from
\begin{align*}
\alpha^{\frac{1}{d}}\log(v\lambda^{-1})^{\frac{d-1}{d}}\geq 1 \; .
\end{align*}
Finally we obtain that
\begin{align*}
(g^{-1})^{'}\left(\alpha \log(v\lambda^{-1})^{d-1} \right)\leq \frac{1}{\log(\alpha^{\frac{1}{d}}\log(v\lambda^{-1})^{\frac{d-1}{d}})^{d-1}} \; .
\end{align*}
Therefore we have
\begin{align*}
\text{df}(\lambda)&\leq  \int_{\lambda}^{+\infty}\frac{\gamma\left[\alpha \frac{d-1}{v}\log(v\lambda^{-1}) \right](g^{-1})'(\alpha \log(v\lambda^{-1})^{d-1})
}{\gamma+v} dv   \\
& \leq \int_{\lambda}^{e^{\alpha^{\frac{-1}{d-1}}}}\left[\alpha \frac{d-1}{v}\log(v\lambda^{-1}) \right](g^{-1})'(\alpha \log(v\lambda^{-1})^{d-1})dv  + \int_{e^{\alpha^{\frac{-1}{d-1}}}}^{+\infty}\frac{\gamma\left[\alpha \frac{d-1}{v}\log(v\lambda^{-1}) \right]
}{\left(\gamma+v\right)\left[\log(\alpha^{\frac{1}{d}}\log(v\lambda^{-1})^{\frac{d-1}{d}})^{d-1}  \right]} dv \\
&\leq g^{-1}\left(\alpha \log(e^{\frac{1}{d-1}}\lambda^{-1})^{d-1}\right) + \int_{e^{\alpha^{\frac{-1}{d-1}}}}^{+\infty}\frac{\gamma\left[\alpha \frac{d-1}{v}\log(v\lambda^{-1}) \right]
}{\left(\gamma+v\right)\left[\log(\alpha^{\frac{1}{d}}\log(v\lambda^{-1})^{\frac{d-1}{d}})^{d-1}  \right]} dv
\end{align*}
But by considering $\lambda\leq e^{-1}$, we obtain that
\begin{align*}
\log(v\lambda^{-1})^{d-1}\leq (\log(v)+1)^{d-1}\log(\lambda^{-1})^{d-1}
\end{align*}
Moreover we have for all $v\geq e^{\alpha^{\frac{-1}{d-1}}}\geq 1$
\begin{align*}
\log(\alpha^{\frac{1}{d}}\log(v\lambda^{-1})^{\frac{d-1}{d}})^{d-1} &= \left[\frac{1}{d}\log(\alpha)+\frac{d-1}{d}\log(\log(v\lambda^{-1}))  \right]^{d-1}\\
&\geq  \left[\frac{1}{d}\log(\alpha)+\frac{d-1}{d}\log(\log(\lambda^{-1}))  \right]^{d-1}
\end{align*}
And as soon as 
\begin{align*}
\lambda \leq \text{min}\left(e^{-1}, \exp(\exp(\frac{d}{d-1}\log(\alpha^{\frac{1}{d}})))\right)
\end{align*}
We have that
\begin{align*}
  \log(\alpha^{\frac{1}{d}}\log(v\lambda^{-1})^{\frac{d-1}{d}})^{d-1}\geq 
 \left(\frac{d-1}{d}\right)^{d-1} \left(\log(\log(\lambda^{-1}))\right)^{d-1}
\end{align*}
Finally we obtain that
\begin{align*}
\int_{e^{\alpha^{\frac{-1}{d-1}}}}^{+\infty}\frac{\gamma\left[\alpha \frac{d-1}{v}\log(v\lambda^{-1}) \right]
}{\left(\gamma+v\right)\left[\log(\alpha^{\frac{1}{d}}\log(v\lambda^{-1})^{\frac{d-1}{d}})^{d-1}  \right]} dv \leq \frac{\log(\lambda^{-1})^{d-1}}{\left(\log(\log(\lambda^{-1}))\right)^{d-1}}\frac{\gamma\alpha(d-1)d^{d-1}}{(d-1)^{d-1}}\int_{e^{\alpha^{\frac{-1}{d-1}}}}^{+\infty}
\frac{(\log(v)+1)^{d-1}}{(\gamma v+v^2)}dv
\end{align*}
Moreover we have
\begin{align*}
g\left(\frac{\log(\lambda^{-1})^{d-1}}{\left(\log(\log(\lambda^{-1}))\right)^{d-1}} \right)=\frac{\log(\lambda^{-1})^{d-1}}{\left(\log(\log(\lambda^{-1}))\right)^{d-1}} \log\left(\frac{\log(\lambda^{-1})^{d-1}}{\left(\log(\log(\lambda^{-1}))\right)^{d-1}} \right)^{d-1}
\end{align*}
And we have:
\begin{align*}
\log\left(\frac{\log(\lambda^{-1})^{d-1}}{\left(\log(\log(\lambda^{-1}))\right)^{d-1}} \right)^{d-1}=\left[(d-1)\log(\log(\lambda^{-1}))-(d-1)\log(\log(\log(\lambda^{-1}))) \right]^{d-1}
\end{align*}
But as $y:\rightarrow \frac{d-2}{d-1}y-\log(y)$ is positive on $\mathbb{R}_{+}$, we obtain that:
\begin{align*}
  \log\left(\frac{\log(\lambda^{-1})^{d-1}}{\left(\log(\log(\lambda^{-1}))\right)^{d-1}} \right)^{d-1}\geq  \left(\log(\log(\lambda^{-1}))\right)^{d-1} 
\end{align*}
And finally we have that:
\begin{align}
\label{eq:g^-1}
\frac{\log(\lambda^{-1})^{d-1}}{\left(\log(\log(\lambda^{-1}))\right)^{d-1}}\geq g^{-1}(\log(\lambda^{-1})^{d-1})
\end{align}
Therefore we obtain that:
\begin{align*}
\text{df}({\lambda})&\leq g^{-1}\left(\alpha \log(e^{\frac{1}{d-1}}\lambda^{-1})^{d-1}\right) + \frac{\log(\lambda^{-1})^{d-1}}{\left(\log(\log(\lambda^{-1}))\right)^{d-1}}\frac{\gamma\alpha(d-1)d^{d-1}}{(d-1)^{d-1}}\int_{e^{\alpha^{\frac{-1}{d-1}}}}^{+\infty}
\frac{(\log(v)+1)^{d-1}}{(\gamma v+v^2)}dv\\
\end{align*}
And thanks to the Eq. (\ref{eq:g^-1}), we obtain that:
\begin{align*}
    \text{df}(\lambda)\in\mathcal{O}\left(\frac{\log(\lambda^{-1})^{d-1}}{\left(\log(\log(\lambda^{-1}))\right)^{d-1}} \right)
\end{align*}
\end{proof}
% \begin{thm}
% Let $\tau\geq 1$ $0<\beta\leq 2$, $\omega>0$, $0<\beta\leq 2$ and $\rho\in \mathcal{G}_{\omega,\beta}$. If there exist $1 > \delta>0$ such that:
% \begin{align*}
% %\label{eq:b_n-final}
% \left|\frac{b_{m}}{b_{m-1}}\right|\in O(m^{-\delta})
% \end{align*}
% There exists a constant $Q>0$ such that:
% \begin{itemize}
% \item  If $\beta> 1$, then there exists $\ell_{\tau}>0$ such that for all $\ell\geq \ell_{\tau}$ and $\lambda_{\ell}=\frac{1}{\ell^{1/\beta}}$, with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
%     \begin{align*}
%     \Vert f_{\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{d-1}}{[\log(\log(\ell))]^{d-1}\ell}
%     \end{align*}
    
%     \item  If $\beta = 1$, then there exists $\ell_{\tau}>0$ such that for all $\ell\geq \ell_{\tau}$, $\lambda_{\ell}=\frac{\log(\ell)^{\mu}}{[\log(\log(\ell))]^{\mu}\ell}$ and $\mu\geq d-1$, with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
%     \begin{align*}
%     \Vert f_{\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{\mu}}{[\log(\log(\ell))]^{\mu}\ell}\\
%     \end{align*}
%     \item If $\beta < 1$, then there exists $\ell_{\tau}>0$ such that for all $\ell\geq \ell_{\tau}$ and $\lambda_{\ell}=\frac{\log(\ell)^{\frac{d-1}{\beta}}}{[\log(\log(\ell))]^{\frac{d-1}{\beta}}\ell}$ with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ it holds
%     \begin{align*}
%     \Vert f_{\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2 &\leq 3C\tau^2\frac{\log(\ell)^{d-1}}{[\log(\log(\ell))]^{d-1}\ell^{\beta}}
%     \end{align*}
% \end{itemize}
% where $N=\text{max}(256KQ,16K,1)$,  $C=2*\text{max}(B,128*V\text{max}(5*Q,K))$, $K=\sup_{x\in S^{d-1}} K_N(x,x)$ and $V=\text{max}(L^2,\sigma^2,2BK+ 2B_{\infty})$.
% \end{thm}
Let us now prove the theorem. Thanks to Proposition \ref{prop:df-super-exp}, we have an explicit control of $\text{df}(\lambda)$, which allows us to derive a proof analogous to the one of Theorem \ref{thm:upper-rate}. Indeed there exists a constant $Q>0$ such that for any $\lambda>0$ we have:
\begin{align*}
\text{df}(\lambda)\leq Q \frac{\log(\lambda^{-1})^{d-1}}{\lambda \left(\log(\log(\lambda^{-1}))\right)^{d-1}}
\end{align*}

The only changes required are the ones related to the new formulation of the the $\text{df}(\lambda)$, that is to say,  $N_{\lambda,\tau}$ and the RHS term of the inequality in Eq.\ref{eq:main-upper-inequality}. Indeed in that case by the exact same arguments of the proof of Lemma \ref{lem:control-const}, we have for $\tau\geq 1$ and $\lambda>0$:
\begin{align*}
N_{\lambda,\tau}&\leq N\tau^2
\frac{\log(\lambda^{-1})^{d-1}}{\lambda \left(\log(\log(\lambda^{-1}))\right)^{d-1}}\\
\text{where\quad} N&=\text{max}(256KQ,16K,1)
\end{align*}
Moreover if $\ell\geq N_{\lambda,\tau}$, a similar proof as in Theorem \ref{thm:upper-rate} gives
\begin{align*}
\Vert f_{H_N,\mathbf{z},\lambda}-f_{\rho,\lambda}\Vert_{\rho}^2&\leq
C_1\left[\frac{\tau^2}{\ell \lambda^{\text{max}(0,1-\beta)}}\left(\frac{\log(\lambda^{-1})^{d-1}}{\left(\log(\log(\lambda^{-1}))\right)^{d-1}}+\frac{1}{\ell \lambda}\right)\right]\\
\text{where\quad } C_1&=128*V\text{max}(5*Q,K)
\end{align*}
with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$. Moreover from Lemma \ref{lem:approx-error} we finally have:
\begin{align*}
\Vert f_{H_N,\mathbf{z},\lambda}-f_{\rho}\Vert_{\rho}^2&\leq
C\left[\lambda^{\beta}+\frac{\tau^2}{\ell \lambda^{\text{max}(0,1-\beta)}}\left(\frac{\log(\lambda^{-1})^{d-1}}{\left(\log(\log(\lambda^{-1}))\right)^{d-1}}+\frac{1}{\ell \lambda}\right)\right]\\
\text{where\quad } C&=2*\text{max}(B,128*V\text{max}(5*Q,K))
\end{align*}
with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$. Now if we assume that $\beta>1$ and $\lambda_{\ell} = \frac{1}{\ell^{1/\beta}}$, we obtain that:
\begin{align*}
\Vert f_{H_N,\mathbf{z},\lambda}-f_{\rho}\Vert_{\rho}^2&\leq
C\left[\frac{1}{\ell}+\frac{\tau^2}{\ell}\left(\frac{1}{\beta^{d-1}}\frac{\log(\ell)^{d-1}}{[\log(\log(\ell))]^{d-1}}+\frac{1}{\ell^{1-\frac{1}{\beta}}}\right)\right]\\
&\leq 3C\tau^2\frac{\log(\ell)^{d-1}}{[\log(\log(\ell))]^{d-1}\ell}
\end{align*}
with a $\rho^{\ell}$-probability $\geq 1-e^{-4\tau}$ provided that 
\begin{align*}
\ell\geq  \left(\frac{ N}{\beta^{\frac{d-1}{\delta}}}\right)^{{\frac{\beta}{\beta-1}}} \tau^{{\frac{2\beta}{\beta-1}}}
\left(\frac{\log(\ell)}{[\log(\log(\ell))]}\right)^{\frac{(d-1)\beta}{\beta-1}}:=\ell_{\tau}
\end{align*}

A similar reasoning leads to the results in the cases where $\beta=1$ and $0<\beta<1$.
\end{proof}

\begin{coro}
\label{coro:exp-rate}
Under the exact same assumptions of theorem \ref{thm:super-geo}, it holds:
\begin{equation*}
\lim_{\tau\rightarrow +\infty}\lim \sup_{\ell\rightarrow\infty}\sup_{\rho\in \mathcal{F}_{H,\alpha,\beta}} \rho^{\ell}\left(\mathbf{z}:\Vert f_{\mathbf{z},\lambda_{\ell}}-f_{\rho}\Vert_{\rho}^2>\tau a_{\ell}\right)=0
\end{equation*}
if one of the following conditions hold:
\begin{itemize}
    \item $\beta> 1$, $\lambda_{\ell}=\frac{1}{\ell^{1/\beta}}$ and $a_{\ell} = \frac{\log(\ell)^{d-1}}{[\log(\log(\ell))]^{d-1}\ell}$
    \item $\beta = 1$, $\lambda_{\ell}=\frac{\log(\ell)^{\mu}}{[\log(\log(\ell))]^{\mu}\ell}$ and $a_{\ell} = \frac{\log(\ell)^{\mu}}{[\log(\log(\ell))]^{\mu}\ell}$ for $\mu>d-1>0$
    \item $\beta < 1$, $\lambda_{\ell}=\frac{\log(\ell)^{\frac{d-1}{\beta}}}{[\log(\log(\ell))]^{\frac{d-1}{\beta}}\ell}$ and $a_{\ell} = \frac{\log(\ell)^{d-1}}{[\log(\log(\ell))]^{d-1}\ell^{\beta}}$
\end{itemize}
\end{coro}

% \begin{proof}{Sketch of proof}
% To prove the non asymptotic results obtained, we just need to show that the existence of such an $\ell_0>0$. Let $\beta>1$ and we denote $\lambda_\ell=\frac{\tau^2}{\ell^{\frac{1}{\beta}}}$. First we remarks that:
% \begin{align*}
% \frac{\ell\lambda^{\ell}}{\log(\lambda_{\ell})^{\frac{d-1}{\delta}}}\geq \tau^2 \beta^{\frac{d-1}{\delta}}\frac{\ell^{\frac{\beta-1}{\beta}}}{\log(\ell)^{\frac{d-1}{\beta}}}
% \end{align*}
% Therefore as $\frac{\ell^{\frac{\beta-1}{\beta}}}{\log(\ell)^{\frac{d-1}{\beta}}}\rightarrow \infty$ as $\ell\rightarrow\infty$, there exists $\ell_0>0$ (independent of $\tau$) such that for all $\ell\geq \ell_0$, 
% \begin{align*}
% \frac{\ell^{\frac{\beta-1}{\beta}}}{\log(\ell)^{\frac{d-1}{\beta}}}\geq\frac{N}{\beta^{\frac{d-1}{\delta}}}
% \end{align*}
% Finally we obtain that for such $\ell\geq \ell_0$:
% \begin{align*}
% \Vert f_{\mathbf{z},\lambda}-f_{\rho}\Vert_{\rho}^2&\leq
% C\left[\frac{\tau^{2\beta}}{\ell}+\frac{\tau^2}{\ell}\left(1+\frac{1}{\beta^{\frac{d-1}{\delta}}}\log(\ell)^{\frac{d-1}{\delta}}+\frac{1}{\ell^{1-\frac{1}{\beta}}}\right)\right]\\
% &\leq  4C\tau^{2\beta}\frac{\log(\ell)^{\frac{d-1}{\delta}}}{\ell}
% \end{align*}
% A similar proof hold for $\beta=1$ and $\beta<1$.
% \end{proof}


\subsection{Proof of Proposition~\ref{prop:effect_depth_geo}}
\label{proof:effect_depth_geo}
\begin{proof}
In the following let us denote $$f (x) = f_N\circ...\circ f_1(x)$$ and $(b_m)_{_m\geq 0}$ its non negative coefficients. Let us now introduce the following lemma.
\begin{lemma}
\label{lem:upp-alpha-coeff}
If there exists $1>r>0$ and $c_1\geq c_2>0$ there for all $m\geq 0$:
\begin{align}
\label{assumption-coeff-2}
    b_m \leq c_1 r^m
\end{align}
Then we have that for all $\alpha\geq 1$ and $m\geq 0$:
\begin{align*}
\frac{d^{m}}{dt^{m}}|_{t=0} \frac{f^{\alpha}}{m!} \leq  c_1^{\alpha} (m+1)^{\alpha-1} r^m
\end{align*}
\end{lemma}
\begin{proof}
Recall that for all $m\geq 0$, $b_m:= \frac{d^{m}}{dt^{m}}|_{t=0} \frac{f}{m!}$. Let us now show the result by induction on $\alpha$. For $\alpha=1$, the result comes directly from Eq. \ref{assumption-coeff-2}. Let now $\alpha \geq 1$ and $m\geq 0$, then we have:
\begin{align*}
\frac{d^{m}}{dt^{m}}|_{t=0} \frac{f^{\alpha+1}}{m!}&=\frac{1}{m!}\sum_{k=0}^m \binom{m}{k}\frac{d^{k}}{dt^{k}}|_{t=0} f^{\alpha}\frac{d^{k}}{dt^{k}}|_{t=0} f_1\\
&= \sum_{k=0}^m \frac{d^{k}}{dt^{k}}|_{t=0} \frac{f^{\alpha}}{k!}\times \frac{d^{m-k}}{dt^{m-k}}|_{t=0} \frac{f}{(m-k)!}
\end{align*}

Moreover by induction we have for all $1\leq q\leq \alpha$ and $k\geq 0$:
\begin{align*}
    c_2^{q}  r^k   \leq \frac{d^{k}}{dt^{k}}|_{t=0} \frac{f^{q}}{k!}\leq 2 c_1^{q} (k+1)^{q-1} r^k 
\end{align*}
Therefore we have:
\begin{align*}
\sum_{k=0}^m c_2^{\alpha}  r^k \times c_2 r^{m-k}  &\leq \frac{d^{m}}{dt^{m}}|_{t=0} \frac{f^{\alpha+1}}{m!}\leq  \sum_{k=0}^m  c_1^{\alpha} (k+1)^{\alpha-1} r^k \times c_1 r^{m-k}\\
c_2^{\alpha+1} r^m   &\leq \frac{d^{m}}{dt^{m}}|_{t=0} \frac{f^{\alpha+1}}{m!}  \leq  c_1^{\alpha+1} r^m \sum_{k=0}^m  (k+1)^{\alpha-1} \leq c_1^{\alpha+1} r^m \sum_{k=1}^{m+1}  k^{\alpha-1}
\end{align*}
Moreover a clear induction give us for all $m\geq 1$ and $\alpha\geq 1$
\begin{align*}
\sum_{k=1}^m  k^{\alpha-1} \leq m^{\alpha}
\end{align*}
Indeed for $\alpha=1$ the result is clear and for all $m\geq 1$ and $\alpha\geq 1$ we have
\begin{align*}
\sum_{k=1}^m  k^{\alpha}&\leq m\times \sum_{k=1}^m  k^{\alpha-1}\\
&\leq m^{\alpha+1}
\end{align*}
The last inequality is obtained by induction on $\alpha\geq 1$. Therefore we have for all $m\geq 0$
\begin{align*}
c_2^{\alpha+1} r^m   &\leq \frac{d^{m}}{dt^{m}}|_{t=0} \frac{f^{\alpha+1}}{m!}  \leq  c_1^{\alpha+1} (m+1)^{\alpha} r^m 
\end{align*}
and the result follows.
\end{proof}


Recall that $f_{N+1},...,f_{N+q}$ are polynomial functions, therefore there exists $\alpha\geq 1$ such that:
\begin{align*}
    f_{N+1}\circ...\circ f_{N+q}(x)=\sum_{k=0}^\alpha d_k x^k
\end{align*}
Therefore we obtain that:
\begin{align*}
    f_{N+q}\circ...\circ f_{1}(x)&=\sum_{k=0}^\alpha d_k [f(x)]^k\\
    &= \sum_{k=0}^\alpha c_k \left[\sum_{m\geq 0} \frac{d^{m}}{dt^{m}}|_{t=0} \frac{f^k}{m!}  \right] x^m\\
    &=\sum_{m\geq 0} \left[\sum_{k=0}^\alpha d_k \frac{d^{m}}{dt^{m}}|_{t=0} \frac{f^k}{m!}\right]  x^m.
\end{align*}
And thanks to Lemma \ref{lem:upp-alpha-coeff} we obtain that:
\begin{align*}
    a_m = \left[\sum_{k=0}^\alpha d_k \frac{d^{m}}{dt^{m}}|_{t=0} \frac{f^{k}}{m!}\right] \leq \sum_{k=1}^\alpha d_k c_1^{k} (m+1)^{k-1} r^m 
\end{align*}
Therefore by considering $1>r'>r>0$, we obtain that:
\begin{align*}
    a_m \leq c_1' r'^m
\end{align*}
for a constant $c_1'$ depending on $q$ and $(d_k)_{k=1}^\alpha$.
\end{proof}

\begin{prop}
Let $N\geq 1$, $d\geq 2$ and $(f_i)_{i=1}^N$ be a sequence of N real value functions such that
\begin{align*}
 f_N\circ...\circ f_1(x):=\sum_{m\geq 0} b_m x^m.
\end{align*}
where $(b_m)_{_m\geq 0}$ are non negative coefficients. Let also $q\geq 1$ and $f_{N+1},...f_{N+q}$ polynomial functions of arbitrary degree with non negative coefficients. Assume that there exists $0<c_1$ and $\delta>0$ some constants such that the sequence $(b_m)_{m\geq 0}$ satisfies for all $m\geq 0$:
\begin{align*}
b_m \leq c_1 (m!)^{-\delta}
\end{align*}
Then  $f_{N+q}\circ...\circ f_1(x)$ admits a Taylor decomposition with non negative coefficients and by denoting $(a_m)_{m\geq 0}$ those coefficients, we obtain that there exists $\delta>\delta'>0$ and $0<c_1'$ such that for all $m\geq 0$
\begin{align*}
 a_m \leq c_1' (m!)^{-\delta'}
\end{align*}
\end{prop}

\begin{proof}
We first start by introducing the following lemma.
\begin{lemma}
\label{lem:upp-alpha-coeff-super-geo}
If there exists $\delta>0$ and $c_1>0$ such that there for all $m\geq 0$:
\begin{align}
\label{assumption-coeff}
    b_m \leq c_1 (m!)^{-\delta}
\end{align}
Then we have that for all $\alpha\geq 1$ and $m\geq 0$:
\begin{align*}
\frac{d^{m}}{dt^{m}}|_{t=0} \frac{f^{\alpha}}{m!} \leq  c_1^{\alpha} (2)^{(\alpha-1)m}  b_m \leq c_1 (m!)^{-\delta}
\end{align*}
\end{lemma}
\begin{proof}
A similar induction as in the proof of Lemma \ref{lem:upp-alpha-coeff} leads to the results.
\end{proof}
Therefore we have
\begin{align*}
    a_m = \left[\sum_{k=1}^\alpha d_k \frac{d^{m}}{dt^{m}}|_{t=0} \frac{f^{k}}{m!}\right] \leq \sum_{k=1}^\alpha d_k c_1^{k} 2^{(k-1)m}  b_m \leq c_1 (m!)^{-\delta}
\end{align*}
and by considering $\delta>\delta'>0$ the result follows.
\end{proof}

Adding layer to the network when it has already reached a geometric or super-geometric regime does not change the regime, and therefore the results of Theorem \ref{thm:rls-geo} can be applied. Therefore as soon as the network reaches the geometric regime, adding layers to the network does not affect the learning rate of convergence. However adding layers to the network allows the function space of target function to grow. Indeed observe that the eigenvalue decay decreases slower when the number of layers increases. Therefore, the RKHS obtained become larger. The eigenvalue decay gives a concrete notion of the complexity of the function space considered. Given an eigensystem  $(\mu_m)_{m\geq 0}$ and $(e_m)_{m\geq 0}$ of positive eigenvalues and eigenfunctions respectively of the integral operator $T_{K_N}$, associated with the Kernel $K_N$, defined on $L_2(S^{d-1})$, the RKHS $H_N$ associated is defined as:
$$ H_N=\left\{f\in L_2(\mathcal{I})\text{:\quad} f = \sum_{m\geq 0} a_m e_m \text{\quad with\quad } \left( \frac{a_m}{\sqrt{\mu_m}} \right)\in\ell_2\right\}$$
endowed with the following inner product:
\begin{align*}
\langle f,g \rangle=\sum_{m\geq 0} \frac{a_m b_m}{\mu_m}
\end{align*}
From this definition, we see immediately that as the eigenvalues of the integral operator decreases slower, the RKHS becomes larger. Therefore composing layers allows the function space generated by the network to grow and therefore allows the function space of the target function to grow, while the learning rates remain the same.

\section{Example}
\begin{figure}[ht!]
\centering
\includegraphics[width=0.5\textwidth]{figures/b_n_decay.pdf}
    \caption{Decay of $(|b_m/b_{m-1}|)_{m\geq 1}$. \label{fig:decay_bn}}
\end{figure}


\label{proof:example}
\begin{lemma}
\label{lemma:coeff-rec}
Let $N\geq 2$. If $f_N$ is the exponential function we have the following relation for all $m\geq 0$
\begin{align*}
b_{m+1}=\frac{1}{m+1}\sum_{k=0}^m b_{k} b_{m+1-k}(m+1-k)
\end{align*}
Moreover if $f_1(t)=...=f_N(t)=\exp(t)$ the result above hold for all $n\in[|2,N|]$.
\end{lemma}


\begin{proof}
We remarks that:
\begin{align*}
f_{N}'(t)&=(f_N\circ(f_{N-1}))'(t)\\
&= f_{N-1}'(t)\times f_{N}(t)
\end{align*}
Therefore by applying the Leibniz formula we obtained that:
\begin{align*}
f_{N}^{m+1}(t)= \sum_{k=0}^m \dbinom{m}{k}  f_{N}^{k}(t) 
f_{N-1}^{m+1-k}(t)
\end{align*}
Therefore we obtain:
\begin{align*}
\frac{f_{N}^{m+1}(0)}{(m+1)!}&=\sum_{k=0}^m \dbinom{m}{k} \frac{k!}{(m+1)!} \frac{ f_{N}^{k}(0)}{k!}f_{N-1}^{m+1-k}(0)\\
&= \frac{1}{m+1}\sum_{k=0}^m \frac{ f_{N}^{k}(0)}{k!}\frac{f_{N-1}^{m+1-k}(0)}{(m+1-k)!}(m+1-k)
\end{align*}
The results follows.
\end{proof}


\section{Background}
\label{sec:background}
\begin{defn}(\textbf{Positive semi-definite kernel})
A positive semi-definite kernel on $\mathcal{X}$ is an application $k:\mathcal{X}\times\mathcal{X}\rightarrow\mathbb{R}$ symmetric, such that for all finite families of points in $\mathcal{X}$, the matrix of pairwise kernel evaluations is positive semi-definite.
\end{defn}
\begin{defn}(\textbf{Positive definite kernel} \cite{pinkus2004strictly})
A positive definite kernel on $\mathcal{X}$ is an application $k:\mathcal{X}\times\mathcal{X}\rightarrow\mathbb{R}$ symmetric, such that for all finite families of \textbf{distinct} points in $\mathcal{X}$, the matrix of pairwise kernel evaluations is positive definite.
\end{defn}
\begin{defn}(\textbf{$c$-universal} \cite{sriperumbudur2011universality})
A continuous positive semi-definite kernel k on a compact Hausdorff space $\mathcal{X}$ is called $c$-universal if the RKHS, H induced by k is dense in $\mathcal{C}(\mathcal{X})$ w.r.t. the uniform norm, i.e., for every function $g\in\mathcal{C}(\mathcal{X})$ and all $\epsilon > 0$, there exists an $f \in H$ such that $\Vert f-g\Vert_{u}\leq \epsilon$.
\end{defn}
\begin{defn}(\textbf{$cc$-universal} \cite{sriperumbudur2011universality})
%\label{def:cc-universal}
A continuous positive semi-definite  kernel k on a Hausdorff space $\mathcal{X}$ is said to be $cc$-universal if the RKHS, H induced by k is dense in $\mathcal{C}(\mathcal{X})$ endowed with the topology of compact convergence, i.e., for any compact set $Z \subset \mathcal{X}$, for any $g\in \mathcal{C}(Z)$ and all $\epsilon > 0$, there exists an $f\in H|_{Z}$ such that $\Vert f- g \Vert_u\leq \epsilon$.
\end{defn}
\begin{rmq}
It is important to notice that a $c$- or $cc$- universal kernel is necessarily a positive definite kernel.
\end{rmq}
\begin{defn}(\textbf{Dot product kernel on the sphere}  \cite{smola2001regularization})
Let  consider a function $f:[-1,1]\rightarrow\mathbb{R}$ that can be expended into its Taylor series in 0, i.e. for all $t\in[-1,1]$:
\begin{align*}
\label{def:dev}
f(t)=\sum_{n\geq 0}\frac{f^{(n)}(0)}{n!} t^{n}
\end{align*}
Let us now define the general dot product kernel $k$ associated with $f$ on the unit sphere $S^{d-1}\subset\mathbb{R}^d$ by:
\begin{align*}
k(x,y):=f(\langle x,y\rangle_{\mathbb{R}^d}).
\end{align*}
\end{defn}
\begin{rmq} 
If $f^{(n)}(0)\geq 0$  for every $n\geq 0$ then k is a continuous positive semi-definite kernel on $S^{d-1}$.
\end{rmq} 


\section{Useful Theorems}
\label{sec:useful-thm}
\begin{thm}{\cite{fischer2017sobolev}}
\label{thm:stein-oracle-1}
Let $0<\beta\leq 2$ and $H$ a separable RKHS on $\mathcal{X}$ with respect to a bounded and measurable kernel $k$ and $\rho$ a probability measure on $\mathcal{X}\times\mathcal{Y}$ with $\int_{\mathcal{X}\times\mathcal{Y}}y^2d\rho(x,y) < \infty$. We assume that $\Vert f_{\rho}\Vert_{L_{\infty}^{d\rho_{\mathcal{X}}}} < \infty$ and that there exist $g\in L_2^{d\rho_{\mathcal{X}}}(\mathcal{X})$ such that $f_\rho=T_{\rho}^{\beta/2}g$.
Furthermore, we assume that there exist $\sigma>0$ and $L>0$ such that
\begin{equation}
 \int_{\mathcal{Y}} |y-f_{\rho}(x)|^m d\rho(y|x)\leq \frac{1}{2}m!L^{m-2} 
\end{equation}
for $\rho_{X}$-almost all $x\in\mathcal{X}$ and all $m\geq 2$.
Then for $\tau \geq 1$, $\lambda>0$ and $\ell\geq N_{\lambda,\tau}$
 we have with $\rho^{\ell}$-probability $\geq 1-4e^{-\tau}$,
\begin{equation}
\Vert f_{\mathbf{z},\lambda}-f_{\rho,\lambda}\Vert_{\rho}^2\leq 128\frac{\tau^2}{\ell}\left(5\text{df}(\lambda)\sigma_{\lambda}^2+ K \frac{L_{\lambda}}{\ell\lambda}   \right)
\end{equation}
where $K = sup_{x\in\mathcal{X}}k(x,x)$
\begin{align*}
N_{\lambda,\tau}&= \max\left(\frac{256\tau^2 K\text{df}(\lambda)}{\lambda},\frac{16\tau K}{\lambda}, \tau \right)\\
\sigma_{\lambda}&=\max(\sigma,\Vert f_{\rho}- f_{\rho,\lambda}\Vert_{L_\infty^{d\rho_{\mathcal{X}}}})\\
L_{\lambda}&=\max(L,\Vert f_{\rho}-f_{\rho,\lambda}\Vert_{L_\infty^{d\rho_{\mathcal{X}}}})
\end{align*}
\end{thm}

\begin{thm}{\cite{caponnetto2007optimal}}
\label{prop:number_of_func}
For every $m > 16$ there exist $N\in\mathbb{N}$ and $\omega^1,...,\omega^N\in \{-1,+1\}^m$
such that
\begin{align*}
 \sum_{i=1}^m(\omega^k_i-\omega^{j}_i)^2 &\geq m \text{\quad} k\neq j=1,...,N\\
 N&\geq e^{m/24}
\end{align*}
\end{thm}

\begin{thm}\cite{saitoh1997integral}
\label{thm:RKHS-Inclusion}
Let $\phi:\mathcal{X}\rightarrow H$ be a feature map to a Hilbert space $H$, and let $K(z,z'):=\langle \phi(z),\phi(z')\rangle_{H}$ a positive semi-definite kernel on $\mathcal{X}$.
Then $\mathcal{H}:=\{f_{\alpha}:z\in\mathcal{X}\rightarrow\langle \alpha,\phi(z)\rangle_{H}\text{,\quad} \alpha\in H\}$ endowed with the following norm:
\begin{align*}
\Vert f_{\alpha}\Vert^2:=\inf_{\alpha'\in\mathcal{H}}\{ \Vert \alpha' \Vert_{H}^2\text{\quad s.t \quad } f_{\alpha'}=f_{\alpha}\}
\end{align*}
is the RKHS associated to K.
\end{thm}

\begin{thm}{\cite{steinwart2001influence}}
\label{thm:univ_classic}
Let $0<r\leq +\infty$ and $f: (-r,r)\rightarrow\mathbb{R}$ be a $C^{\infty}$-function that can be expanded
into its Taylor series in 0, i.e.
\begin{align*}
\label{function}
f(x)=\sum_{m=0}^{\infty}a_m x^{m}\text{.}
\end{align*}
Let $X:=\{x\in \mathbb{R}^d: \Vert x\Vert_2 <\sqrt{r}\}$. If we have $a_n>0$ for all $n\geq 0$ then $k(x,y):=f(\langle x,y\rangle)$ defines a $c$-universal kernel on every compact subset of X.
\end{thm}


\begin{thm}\citep{azevedo2014sharp}
\label{thm:eigenval}
Each spherical harmonics of degree m, $Y_{m}\in H_{m}(S^{d-1})$, is an eigenfunction of $T_{K_N}$ with associated eigenvalue given by the formula:
\begin{equation*}
\label{def:formula_eigen}
\lambda_{m}=\frac{|S^{d-2}|\Gamma((d-1)/2)}{2^{m+1}}\sum_{s\geq 0}b_{2s+m}\frac{(2s+m)!}{(2s)!}\frac{\Gamma(s+1/2)}{\Gamma(s+m+d/2)}
\end{equation*}
\end{thm}




\section{Technical Lemmas}
\label{sec:tech-lem}
\begin{lemma}{\cite{fischer2017sobolev}}
\label{lem:KL-div}
For $f,f'\in L_2^{d\nu}(\mathcal{X})$ and $\ell \geq  1$ it holds $\rho_f^{\ell} \ll \rho_{f'}^{\ell}$ and $\rho_f^{\ell} \gg \rho_{f'}^{\ell}$ . Furthermore, the KL
divergence fulfills
\begin{align*}
\text{KL}(\rho_f^{\ell},\rho_{f'}^{\ell})=\frac{\ell}{2\hat{\sigma}^2}\Vert f-f'\Vert_{L_2^{d\nu}(\mathcal{X})}^2
\end{align*}
\end{lemma}

\begin{lemma}\cite{devore2006approximation}
\label{lem:devore-approx} 
 Let $\mathcal{A}$ be a sigma algebra on the space $\Omega$. Let $A_i\in \mathcal{A}$, $i \in \{0,1,...,n\}$ such that $\forall i\neq j$, $A_i\bigcap A_j =\emptyset$. Let $P_i$, $i\in\{0,1,...,n\}$ be $n+1$ probability measures on
$(\Omega, \mathcal{A})$. If
\begin{align*}
p:=\sup_{i=1,...,n} P_i(\Omega \setminus A_i)
\end{align*}
then either $p>\frac{n}{n+1}$ or 
\begin{align*}
\min_{j=1,...,n} \frac{1}{n}\sum_{i\neq j}\text{KL}(P_i,P_j)\geq \psi_n(p)
\end{align*}
where 
\begin{align*}
\psi_n(p):=\log(n) + (1-p) \log \left(\frac{( 1-p )}{p}\right)- p \log \left(\frac{ n-p}{p}\right)
\end{align*}
\end{lemma}
\subsection{Proof of Lemma \ref{lem:explicitcoeffcomp}}
\label{lem-proof-explicitcoeffcomp}
\begin{proof}
Let us show the result by induction on $N$.
For $N=1$ the result is clear as $f_1$  can be expand in its Taylor series in 0 on $\mathbb{R}$ with positive coefficients. Let $N\geq 2$, therefore we have:
\begin{align*}
g(t)=(f_N\circ\text{...}\circ f_2)\circ ( f_{1}(t))
\end{align*}
By induction, we have that for all $t\in\mathbb{R}$:
\begin{align*}
f_N\circ\text{...}\circ f_2(t)=\sum_{l_2,...,l_{N}\geq 0}\frac{f_N^{(l_N)}(0)}{l_{N}!}\times 
\phi_{N-1}(l_N,l_{N-1}) \text{...}\times \phi_{2}(l_3,l_2) t^{l_2}
\end{align*}
Therefore we have that:
\begin{align*}
g(t)&=\sum_{l_2,...,l_{N}\geq 0}\frac{f_N^{(l_N)}(0)}{l_{N}!}\times 
\phi_{N-1}(l_N,l_{N-1}) \text{...}\times \phi_{2}(l_3,l_2) (f_1(t))^{l_2}\\
\end{align*}
Moreover, for all $l_2\geq 0$, $f_{1}^{l_2}$ can be expand in its Taylor series in 0 on $\mathbb{R}$ with non negative coefficients, and we have that for all $l_2\geq 0$ and  $t\in\mathbb{R}$:
\begin{align*}
(f_1(t))^{l_2}=\sum_{l_1\geq 0} \phi_{1}(l_2,l_1) t^{l_1}
\end{align*}
And we obtain that:
\begin{align*}
g(t)=\sum_{l_1,...,l_{N}\geq 0}\frac{f_N^{(l_N)}(0)}{l_{N}!}\times 
\phi_{N-1}(l_N,l_{N-1}) \text{...}\times \phi_{1}(l_2,l_1)t^{l_1}
\end{align*}
Finally we have by unicity of the decomposition that for all $l_1\geq 0$:
\begin{align*}
\frac{g^{(l_1)}(0)}{l_1!}=\sum_{l_2,...,l_{N}\geq 0}\frac{f_N^{(l_N)}(0)}{l_{N}!}\times 
\phi_{N-1}(l_N,l_{N-1}) \text{...}\times \phi_{1}(l_2,l_1)
\end{align*}
Moreover let $k\in[|1,N-1|]$, $l\geq 1$ and let us denote $(a^k_i)_{i\geq 0}$ the coefficients in the Taylor decomposition of $f_k$. Then we have:
\begin{align*}
f_k^{l}(t)&=\sum_{n_1,...,n_l\geq 0}\prod_{i=1}^l \left(a^{k}_{n_i}\right) x^{n_1+...+n_l}\\
&=\sum_{q\geq 0} \left[\sum_{\substack{n_1,...,n_l\geq 0\\ \sum\limits_{i=1}^n n_i=q}} \prod_{i=1}^l \left(a^{k}_{n_i}\right)\right] x^{q}  
\end{align*}
But as $a^k_i>0$ for all $i\geq 0$, we obtain that by unicity of the decompoisition that for all $m\geq 0$:
\begin{align*}
\phi_{k}(l,m)=\frac{d^m}{dt^m}|_{t=0}\frac{f_{k}^{l}(t)}{m!}>0
\end{align*}
and the result follows.
\end{proof}

\section{Experiments}
\label{sec:experiments}


% \begin{figure}[ht]
%   \centering
%   \subfigure[Accuracy vs Depth.\label{fig:accuracy}]{\includegraphics[scale=0.3]{mlp/figures/MLP-depth.pdf}}\quad \quad
%   \subfigure[Decay vs. Depth.\label{fig:spectrum-512}]{\includegraphics[scale=0.3]{mlp/figures/MLP-spect-512.pdf}}
% \end{figure}

% \begin{wrapfigure}{r}{0.3\textwidth}\vspace*{-4.5ex}
%         \includegraphics[width=0.7\linewidth]{mlp/figures/MLP-depth.pdf}
%     \caption{Accuracy vs Depth.\label{fig:accuracy}}
% \end{wrapfigure}


\begin{figure}[ht!]
\centering
\includegraphics[width=0.4\linewidth]{figures/MLP-depth.pdf}
\caption{Accuracy vs Depth\label{fig:accuracy}.} 
\end{figure}



First, we investigate the relations between network depth and prediction accuracy on MNIST~\footnote{ http://yann.lecun.com/exdb/mnist/}. We construct fully connected neural networks from 1 to 3 layers. We model large-width networks by setting number of weights per layer to be constant and sufficiently large. The number of weights can be either 128, 256 or 512 at each layer. Moreover we normalize the input data so that the input datapoints lie on a subspace of the unit sphere. 
We see in Figure~\ref{fig:accuracy} that, in each situation, as the number of layers increases, the prediction accuracy gets better. This means that the networks get better at approximating the target function as the network depth increases.
\medbreak


% \begin{wrapfigure}{r}{0.3\textwidth}\vspace*{-4.5ex}
%         \includegraphics[width=0.7\linewidth]{mlp/figures/MLP-spect-512.pdf}
%     \caption{Decay vs. Depth.\label{fig:spectrum-512}}
% \end{wrapfigure}


\begin{figure}[ht!]
\centering
\includegraphics[width=0.4\linewidth]{figures/MLP-spect-512.pdf}
\caption{Decay vs. Depth.\label{fig:spectrum-512}} 
\end{figure}



Second, we investigate the relation between the network depth and the eigenvalue decay, in the super-geometric setting. We proceed similarly, including regarding input normalization. The first nonlinear activation is the exponential function, while the others are quadratic activation functions for which assumption (\ref{eq:b_n-final}) is indeed satisfied. We obtain the spectral decomposition of the kernel associated with the network by computing the eigenvalues associated with the last hidden layer as a feature map of the kernel. Figure~\ref{fig:spectrum-512} shows the result after 15 epochs and for a number of weights per layer equal to 512. See Figures~\ref{fig:spectrum-128},\ref{fig:spectrum-256} for 128 and 256 respectively. We observe that, as the number of layers increases, the eigenvalue decay is slower, which means that the function space generated by such structures is larger. Therefore, as the number of layers increases, the network gets better at approximating the target function in the asymptotic regime. 




% The MNIST dataset is a dateset of handwritten digits from 0 to 9 which has a training set of 60,000 examples, and a test set of 10,000 examples. In order to train networks on this classification task, we consider the Cross-Entropy loss. Figures \ref{fig:spectrum-256},\ref{fig:spectrum-128} show the eigenvalue decay of the kernel associated with MLPs where the number of weight at each layer is fixed to be 128 and 256 respectively. We observe that, as the number of layers increases, the eigenvalue decay is slower. 
The eigenvalue decay gives a concrete notion of the complexity of the function space considered. Indeed, given an eigensystem  $(\mu_m)_{m\geq 0}$ and $(e_m)_{m\geq 0}$ of positive eigenvalues and eigenfunctions respectively of the integral operator $T_{\rho}$, associated with the Kernel $K_N$, defined on $L_2^{d\rho_{S^{d-1}}}(S^{d-1})$, the RKHS $H_N$ associated is defined as:
$$ H_N=\left\{f\in L_2^{d\rho_{S^{d-1}}}(S^{d-1})\text{:\quad} f = \sum_{m\geq 0} a_m e_m \text{\quad with\quad } \left( \frac{a_m}{\sqrt{\mu_m}} \right)\in\ell_2\right\}$$
endowed with the following inner product:
\begin{align*}
\langle f,g \rangle=\sum_{m\geq 0} \frac{a_m b_m}{\mu_m}
\end{align*}
From this definition, we see immediately that as the eigenvalues of the integral operator decreases slower, the RKHS becomes larger. Therefore composing layers allows the function space generated by the network to grow. Moreover the source condition on the target function $f_{\rho}$ assumes that that there exists $g\in L_2^{d\rho_{S^{d-1}}}(S^{d-1})$ such that $f_\rho=T_{\rho}^{\beta/2}g$ and we have an explicit formulation of the space where the target function is allowed to live:
$$H_{\beta}:=\left\{f\in L_2^{d\rho_{S^{d-1}}}(S^{d-1})\text{:\quad} f = \sum_{m\geq 0} a_m e_m \text{\quad with\quad } \left( \frac{a_m}{\mu_m^{\beta/2}} \right)\in\ell_2\right\}$$
Therefore as soon as the eigenvalues of the integral operator decrease slower, the space where the target function $f_{\rho}$ is allowed to live grows and the network gets better at approximating the target function $f_{\rho}$.


\begin{figure}[ht!]
\centering
\includegraphics[width=0.4\linewidth]{figures/MLP-spect-128.pdf}
\caption{Rate of eigenvalue decay for different depths in semi-log scale. The number of weights is fixed to 128 at each layer \label{fig:spectrum-128}.}
\end{figure}


\begin{figure}[ht!]
\centering
\includegraphics[width=0.4\linewidth]{figures/MLP-spect-256.pdf}
\caption{Rate of eigenvalue decay for different depths in semi-log scale. The number of weights is fixed to 256 at each layer \label{fig:spectrum-256}.} 
\end{figure}


==> sections/zaid_sections.tex <==
\section{Introduction}
%Cutting 1 paragraph approx.
Multi-layer perceptrons have been an important family of machine learning methods, whose history alternates between periods of wide popularity and periods of fading interest \cite{rosenblatt1958perceptron, Minsky:Papert:1987, duda1973pattern}. Described in a mathematical language, a multi-layer perceptron is the iterated composition of parameterized affine maps and nonlinear maps, ultimately composed with a prediction map either for the purpose of predicting a scalar value as in curve fitting or regression, or a binary label as in supervised classification. As the number of layers or network depth grows, the parameterized map resulting from this iterated composition may change in terms of smoothness properties. 

However the impact of network depth on the regularity of the resulting deep network function is, quite surprisingly, still not fully understood, in particular for multi-layer perceptrons. Consider the setting, where the number of datapoints is finite, the number of hidden layers is finite, and the number of weights per layers is finite. We would like to understand, in the case of least-squares regression through with regularized empirical risk minimization for instance \cite{Lin_2020,marteau2019beyond,blanchard2018optimal,steinwart2008support,caponnetto2007optimal,smale2007learning}, how fast does the learned function converge to the target function as the network depth grows and the sample size grows. 

Understanding the relative scaling of the sample size and the network depth can be related to the detailed study of the spectrum of the integral operator associated with a reproducing kernel related to the network architecture. This reproducing kernel may or may not be universal, hence Bayes-consistency may or may not be satisfied. Yet, as we show in this paper, the universality and Bayes-consistency is guaranteed for wide array of situations.


The integral operator is compact, self-adjoint and admits a spectral decomposition. The rate of eigenvalue decay directly controls the convergence rate of the learned function. In this work, we obtain a tight control of the rate of eigenvalue decay for several regimes depending on the nonlinear maps involved in the construction of the network. From this control, we establish high-probability bounds on the learned function and provide guidance on the effect of the depth for such networks, depending on the sample size. Moreover the results obtained extends previous results related to the Mercer decomposition of dot product kernels on spheres \cite{azevedo2014sharp}.

Reproducing kernels are powerful tools which have been used to analyze deep networks in various ways. Recent works used reproducing kernels to build equivalent instantaneous approximations of deep networks during the training process, blending algorithmic and statistical considerations in the analysis. Although remarkable progress has been made in recent years, the understanding of training processes of deep networks is still limited. Many results are qualitative in spirit and various seemingly incompatible interpretations have been proposed and subject to discussion \cite{jacot2018neural,song2018mean,chizat2019lazy}.

We adopt here a nonparametric learning approach~\cite{gkkw:2002,steinwart2008support}, with the modest goal to uncover the interplay of regularity controlled by the network depth and the sample size, with the expectation to obtain high-probability bounds on the learned function explicitly involving the eigenvalue decay of the integral operator. We shall not assume that the target function belongs to the function spaces used for learning. We believe such results are important steps to shed light on the role of network depth on statistical performance. We present here results of this kind for multi-layer perceptrons.
\medbreak
This work makes the following contributions.


Explain that the main purpose of this work is to obtain a control of the eigenvalue decay of the spectrum of the kernel associated to a MLP.
\medbreak
From this control we deduce two important statistical proprietes: first ther rates of MLPs and the effect of the depth


\begin{itemize}
    \item In Sections 3, we present general convergence rates for regularized least-squares regression with kernel-based methods, improving upon known convergence rates in the near geometric regime of eigenvalue decay of integral operators. 
    \item In Section 4, we consider deep networks of multi-layer perceptron type and show how to approach them through reproducing kernel Hilbert spaces and associated integral operators. We obtain tight controls of the eigenvalue decay of the integral operator in two regimes, geometric and super-geometric. 
    
    \item In section 5 we obtain the learning rates assocaited to multi-layer perceptrons in two regimes of eigenvalue decay of the integral operators, geometric and super-geometric, matching known minimax optimal rates in nonparametric least-squares regression. We show increasing the network depth allows to increase the target function space without sacrificing the convergence rate. 
\end{itemize}
We round off the paper with  illustrations of the relationship between the eigenvalue decay and the network depth.



\section{Related work}

\begin{itemize}

    \item Caponetto: Explain the difference with classical results on statistical rates: Polynomial different from geo and super geo. Precise also that we show in appendix the general case for an abitrary RKHS under the assumption of a geometric decay of the spectrum: This is also new. Same for super geo. Finally Thanks to the spectral anlyisis no assumption needed on the spectrum and therefore we obtain learning rates on a non trivial set of distributions.

    \item Zhang: The kernel defined here is a generalisation of Zhang and Mairal as it is adapative to the non linear activation chosen. Therefore the generalization bounds obtained that one may obtained by deriving the RKHS norm of neural networks is tighter than the one presented in Zhang. See Apendix for an upper bound of the RKHS norm of neural networks.
    
    \item Bach: exponential in the dimension. Because we consider this space of distributions. Consider a smaller space allows us to withdraw the dimension.
    
    \item Susuki: 2 major differences: the first one is that the estimators used here is different from the one there and the second is that Susuki  does not provide a control of the eigenvalue decay and other estimator. Note that here we consider RLS which reach optimal learning rates therefore at least as good as MLP estimator.
    
    Recht: \cite{shankar2020neural}: The kernel impletended by Recht and co when considering the index set of size 1 is exactly the same implementation as our MLP. 
    
     Srebro: \cite{ongie2019function}: Fourrier not so bad.

    
\end{itemize}







\section{Framework}

\paragraph{Multi-layer perceptron.}
\paragraph{Deep networks and compositional chains.}
A deep network of depth $k$ is a transformation of an input $x$ into an output  through the composition of $k$ modules; see Fig.~\ref{fig:deep-net} (left). 
 In classical deep networks, such as multi-layer perceptrons or convolutional networks, each module is called a \textit{layer} and corresponds to an affine map followed by a non-linear map. 
 
 We are going to assume that the data consists of $n$ points from $\mathbb{R}^d$ and the number of ``neurons'' is $N$. That is, at the $\ell$-th layer there are $N$ many vector of weights $w_\ell=(w_{\ell,1}, \ldots, w_{\ell,N})$. The layer takes an input vector $z_{\ell-1}$ and returns another  vector $z_{\ell}$ as $z_{\ell} = \left(\sigma_\ell(g_{\ell}(w_{\ell, i}, z_{\ell-1}))\right)_{i=1, \ldots, N}$,
where $g_\ell$ can be linear in $w_\ell$ and affine in $z_{\ell-1}$ and $\sigma_\ell$ is a nonlinear function such as a sigmoid or a rectifier linear unit function, called an \textit{activation function}. Each layer can be seen as a function of the input parameterized by the weight, i.e., $z_\ell = h_\ell(z_{\ell-1}) =\sigma_\ell(g_{\ell}(w_\ell, z_{\ell-1}))$ and the output is a function of the input $x=z_0$, i.e., $z_k = h(x)$. see Fig.~\ref{fig:deep-net} (right). 

\paragraph{The sum of all fears.}
%need figure here
\begin{itemize}
\item describe the many terms for a comprehensive analysis of mlps
\item synchronize notations with Schmidthieber
\item explain that we focus on one term
\item explain why it is hard already
\end{itemize}

\newpage
\paragraph{Embedding into RKHS.}
%need figure here
\begin{itemize}
\item describe how we embed the function space of mlp into rkhs
\item can we say something on the size of the corresponding sets?
\item explain that this is different from other uses of kernels in the literature (tangent kernels, compositional kernels, etc.)
\item draw a figure with the two sets
\end{itemize}

\paragraph{Kernel on sphere.}
%need figure here
\begin{itemize}
\item describe the spherical harmonic decomposition (figure?)
\item state result that we do better than Gepetto
\end{itemize}








\paragraph{Necessary Notations to introduce in this section:}
\todo{I add this because I need these notations after except for the spherical harmonics}
\medbreak
\textbf{Multi-layer Perceptrons.} Let us first introduce the network of interest. Here we consider a fully-connected deep neural network. We shall refer to it as a multi-layer perceptron (MLP).
Let $\mathcal{X}$ be a subset of ${R}^d$, $N$ be the number of hidden layers, $\sigma_1,...,\sigma_N$ real-valued functions defined on $\mathbb{R}$ be the activation functions at each layer and $m_1,...,m_N$ be the width of each layer. Set $m_0:=d$ and $m_{N+1}:=1$. Then, any function defined by an MLP is parameterized by weight matrices $(W^k)_{k=1}^{N+1}$ where each $W^k\in\mathbb{R}^{m_{k-1}m_{k}}$ and can be recovered as follows. Let $x\in\mathcal{X}$, define $\mathcal{N}^0(x):=x$ and for $k\in\{1,\dots,N\}$,  denote
$W^k:=(w_1^k,...,w_{m_{k}}^k)$ where for all  $j\in[|1,m_k|]$ $w_j^k\in\mathbb{R}^{m_{k-1}}$. Then, for all $k\in\{1,...,N\}$, define the $k^{\text{th}}$ layer as
$$\mathcal{N}^{k}(x):=(\sigma_k(\langle \mathcal{N}^{k-1}(x),w_1^k \rangle), ...,\sigma_k(\langle \mathcal{N}^{k-1}(x),w_{m_k}^k \rangle))$$
We obtain $\mathcal{N}(x)=\langle \mathcal{N}^N(x),W^{N+1}\rangle_{\mathbb{R}^{m_N}}$.
We shall denote $\mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N,(m_i)_{i=1}^N}$ the function space defined by all functions $\mathcal{N}$ defined as above on $\mathcal{X}$ for any choice of $(W^k)_{k=1}^{N+1}$. We shall also consider the union space
$$\mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N}:=\bigcup_{(m_1,...,m_N)\in\mathbb{N_{*}}^N} \mathcal{F}_{\mathcal{X},(\sigma_i)_{i=1}^N,(m_i)_{i=1}^N}$$


\textbf{From MLPs to RKHSs.} \todo{not necessary} In the following we show that functions generated by a multi-layer perceptron can be embed into an adaptative RKHS with respect to the nonlinear activations involved in the construction of the network. Moreover we show that kernels induced by MLPs are dot product kernels of the form
\begin{align}
\label{eq:dot-product-kernel}
    K(x,y)= \sum_{m\geq 0}  b_m (\langle x,y\rangle)^{m}\text{,\quad} x,y\in \mathcal{X}
\end{align}
where $(b_m)_{m\geq 0}$ is completely determined by the non linear activation functions $(\sigma_i)_{i=1}^N$ involved in the network. When $\mathcal{X}$ happens to be the unit sphere $S^{d-1}$ of $\mathbb{R}^d$ with $d\geq 2$, we even have access to the eigenspectrum of the integral operator associated.

\textbf{Spherical Harmonics.} Let $d\geq 2$ and $S^{d-1}$ be the unit sphere of $\mathbb{R}^d$. Let $P_{m}(d)$ be the space of homogeneous polynomials of degree $m$ in $d$ variables with real coefficients and $\mathcal{H}_{m}(d)$ be the space of harmonics polynomials defined by
\begin{align}
\mathcal{H}_m(d):=\{P\in P_{m}(d)| \Delta P=0\}
\end{align}
where $\Delta \cdot = \sum\limits_{i=1}^d\frac{\partial^2\cdot}{\partial x_i^2} $ is the Laplace operator on $\mathbb{R}^d$. Moreover let us define
$H_{m}(S^{d-1})$ the space of real spherical harmonics of degree $m$ defined as the set of restrictions of harmonic polynomials in $\mathcal{H}_{m}(d)$ to $S^{d-1}$. Let also $L_2^{d\sigma_{d-1}}(S^{d-1})$ be the space of (real) square-integrable functions on the sphere $S^{d-1}$ endowed with its induced Lebesgue measure $d\sigma_{d-1}$ and $|S^{d-1}|$ the surface area of $S^{d-1}$. $L_2^{d\sigma_{d-1}}(S^{d-1})$  endowed with its natural inner product is a separable Hilbert space and the family of spaces $(H_m(S^{d-1}))_{m\geq 0}$, yields a direct sum decomposition \cite{frye2012spherical}
\begin{align}
L_2^{d\sigma_{d-1}}(S^{d-1})=\bigoplus_{m\geq 0}H_m(S^{d-1})
\end{align}
which means that the summands are closed and pairwise orthogonal.
Moreover, each $H_m(S^{d-1})$ has a finite dimension $\alpha_{m,d}$ with $\alpha_{0,d}=1$, $\alpha_{1,d}=d$ and for $m\geq 2$
\begin{align*}
\alpha_{m,d}=\dbinom{d-1+m}{m}-\dbinom{d-1+m-2}{m-2}
\end{align*}
Therefore for all $m\geq 0$, given any orthonormal basis of $H_m(S^{d-1})$, $(Y_{m}^1,...,Y_{m}^{\alpha_{m,d}})$, we can build an Hilbertian basis of $L_2^{d\sigma_{d-1}}(S^{d-1})$ by concatenating these orthonormal basis. Let us denote in the following $(Y_{m}^{l_m})_{m,l_m}$ such an Hilbertian basis of $L_2^{d\sigma_{d-1}}(S^{d-1})$.
\medbreak
\textbf{Integral Operator.} Given a positive semi-definite kernel $K$ on $S^{d-1}$, we define the integral operator on $L_2^{d\sigma_{d-1}}(S^{d-1})$ associated 
$$\begin{array}{ccccc}
T_{K} & : &  L_2^{ d\sigma_{d-1}}(S^{d-1}) & \to &  L_2^{ d\sigma_{d-1}}(S^{d-1})\\
 & & f &\to & \int_{S^{d-1}} K(x,\cdot)f(x)d\sigma_{d-1}(x).
\end{array}$$
As soon as $\int_{S^{d-1}} K(x,x)d\sigma_{d-1}(x)$ is finite, $T_K$ is well defined, self-adjoint, positive semi-definite and trace-class \cite{smale2007learning}. Denote $H$ the Reproducing Kernel Hilbert Space (RKHS) associated to $K$. The spectral theorem for compact operators tells us for an for at most countable index set $I$, we have a positive, decreasing sequence $(\lambda_i)_{i\in I} \in \ell_1(I)$ and a family $(e_i)_{i\in I} \subset H$, such that $(\lambda_i^{1/2} e_i)_{i\in I}$ is an orthonormal system in $H$ while $(e_i)_{i\in I}$ is an orthonormal system in $L_2^{d\sigma_{d-1}}(S^{d-1})$ with
\begin{align*}
T_{K} &=\sum_{i\in I}\lambda_i\langle ., e_i\rangle_{L_2^{d\sigma_{d-1}}(S^{d-1})} e_i
\end{align*}
In fact for some kernels, one may have access to an explicit formulation of the eigensystem of $T_{K}$.
\medbreak
\textbf{Kernels on Sphere.} Kernels of the form 
\begin{align*}
    K(x,y)=\sum_{m\geq 0}  b_m (\langle x,y\rangle)^{m}\text{,\quad} x,y\in S^{d-1}
\end{align*}
in which $(b_m)_{m\geq 0}$ is an absolutely summable sequence of real numbers are called dot product kernels on $S^{d-1}$ \cite{zwicknagl2009power}. Moreover, If $b_m\geq 0$ for every $m\geq 0$ then $K$ is a continuous positive semi-definite kernel on $S^{d-1}$ \cite{pinkus2004strictly}. In fact for those specific kernels, \cite{azevedo2014sharp} obtain an explicit Mercer decomposition.  More precisely,  each spherical harmonics of degree $m$, $Y_{m}\in H_{m}(S^{d-1})$, is an eigenfunction of $T_{K}$ with associated eigenvalue $\lambda_m$ given by the formula
\begin{align}
\label{eq:formula_eigen-notions}
&\lambda_{m}=\frac{|S^{d-2}|\Gamma((d-1)/2)}{2^{m+1}}\sum_{s\geq 0}b_{2s+m}\frac{(2s+m)!}{(2s)!}\frac{\Gamma(s+1/2)}{\Gamma(s+m+d/2)}.
\end{align}
The main challenge here is to control the eigenvalues decay with their multiplicities of the kernels related to MLPs from the expression given in eq.(\ref{eq:formula_eigen-notions}). Such controls are obtained only for very specific kernels defined on very specific domains. In Table \ref{table:1} we introduce the control obtained for kernels related to MLPs in this paper and give some examples of such controls for other kernels available in the literature \citep{bach2017breaking,bach2017equivalence,blanchard2008finite}.  

\todo{uncomment table}
% \begin{table}[h!]
% \centering
% \begin{tabular}{lcc}
% Kernel & Space & Rate \\ 
% \hline
% \vspace{0.25cm}
% $K(x,x'):=\exp(-b(x-x')^2)$ & $[0,1]$  & $(b/(a+b))^{m}$,$\quad a,b>0$ \\
% \vspace{0.25cm}
% $K(x,x'):=\nu_0+\sum_{m>0}\nu_m \cos(2\pi m(x-x'))$ & $[0,1]$&  $m^{-2s}$,$\quad s\in\mathbb{N}^{*}$\\
% \vspace{0.25cm}
% $K(x,x'):=\mathbb{E}_{v\sim\sigma_{d-1}}(v^T x)^s_{+}(v^T x)^s_{+}$ &$S^{d-1}$  & $m^{-1-1/(d-1)-2s/(d-1)}$, $\quad s\in\mathbb{N}$\\
% \vspace{0.25cm}
% $K_1$ & $S^{d-1}$ &  $m^{- \gamma m^{1/(d-1)}}$, $\quad\gamma>0$ \\
% \vspace{0.25cm}
% $K_2$ & $S^{d-1}$  & $e^{-\gamma m^{\frac{1}{d-1}}}$,$\quad\gamma>0$ 
% \end{tabular}
% \caption{Comparison of eigenvalue decay rates for different kernels. $K_1$ and $K_2$ are the kernels associated respectively to MLPs in the super-geometric and geomtric regime.\label{table:1}}
% \end{table}

\textbf{Notations} Let $(u_n)_{n\geq 0}$ and $(v_n)_{n\geq 0}$ two real-valued sequences. In the following we denote $u_n\in O(v_n)$ if there exists a universal constant $C$ such that for all $n\geq 0$, $u_n\leq C v_n$ and we denote $u_n\in \mathcal{O}(v_n)$ if there exists a constant $C_d$ depending on $d$ such that for all $n\geq 0$ $u_n\leq C_d v_n$.

\newpage

